Understanding Human Intervention in the Platform Economy: A case study of an indie food delivery service

This paper examines the sociotechnical infrastructure of an "indie" food delivery platform. The platform, Nosh, provides an alternative to mainstream services, such as Doordash and Uber Eats, in several communities in the Western United States. We interviewed 28 stakeholders including restauranteurs, couriers, consumers, and platform administrators. Drawing on infrastructure literature, we learned that the platform is a patchwork of disparate technical systems held together by human intervention. Participants join this platform because they receive greater agency, financial security, and local support. We identify human intervention's key role in making food delivery platform users feel respected. This study provides insights into the affordances, limitations, and possibilities of food delivery platforms designed to prioritize local contexts over transnational scales.

==> ChiRevisionsVersion/0_Introduction.tex <==
%NOTE NEED TO ADD IN TRACKED CHANGES
\section{Introduction}
%what is the topic? Indie platforms
%replace users with stakeholders and define stakeholders in paragraph 1
\chdeleted{Mainstream food delivery platforms, such as \textit{UberEats}, \textit{DoorDash}, and \textit{Grubhub}, more than doubled in  popularity in the United States during the COVID-19 pandemic \cite{OrderingRapidEvolution}. This growth helped them further cement themselves as an essential element of most restaurants' business models, and allowed them to charge commission rates of up to 30\% in exchange for access to their large customer base~\cite{DeliveryAppsGrubhub2021, thompsonHiddenCostFood2020}. Restauranteurs \cite{atkinsonMoreJobFood2021}, couriers \cite{dziezaRevoltDeliveryWorkers2021}, and local governments \cite{bomeyDoorDashGrubHubUber} have resisted these mainstream platforms because  platforms' near-monopolistic power often forces restaurants to decide whether to pass on these higher costs and risk losing price-conscious customers or to subsume the costs themselves, reducing already-thin profit margins. This discontent, coupled with the availability of white label software}\chdeleted{White label software is software that an organization pays for to brands as its own. This software is often sold under a subscription or transaction fee. Users usually do not know the software maker.}\chdeleted{, facilitated the rise of ``indie''}\chdeleted{We borrow both the term and meanings associated with ``indie'' from music, film, games, and other industries where indie was used to identify small, independent artists supported by an enthusiastic local fanbase who operated separately from the mainstream.}\chdeleted{platforms. Indie platforms are localized, community-centric, independent businesses that rely on white-label software to offer an alternative to mainstream services.} 
\chadded{Evidence about the negative impacts of gig work---digital platforms that coordinate short-term, on-demand work--- has grown in recent years. Scholars and journalists alike have documented the precarity~\cite{ravenelleSideHustleSafety2021,ma2022brush,dziezaRevoltDeliveryWorkers2021}, the invasive surveillance~\cite{ravenelle2019we}, and the psychological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a} of mainstream gig work platforms, such as Uber, DoorDash, and Deliveroo. In response to these negative impacts, stakeholders of mainstream gig work platforms have begun to explore alternative, ``indie'' platforms. We borrow the meaning and associations of ``indie'' from music, film, games, and other industries where indie was used to identify small, independent artists supported by an enthusiastic local fanbase who operated separately from the mainstream platforms. Indie platforms are localized,
independent businesses that offer an alternative to mainstream services. These indie platforms claim to offer stakeholders more favorable terms of participation and better treatment. Despite their growing popularity, there is very little empirical HCI research exploring stakeholders' motivations for joining and their experiences within these alternative platforms.}

%what is the context? Food delivery 
%replace doubling with the specific number 
\chadded{In this paper, we are interested in indie food delivery platforms. In this context, the stakeholders we are concerned with are restaurants, couriers, and consumers. During the COVID-19 pandemic, the revenue of mainstream food delivery platforms, like DoorDash and GrubHub, more than doubled~\cite{mckinsey}. However, the increased use of these platforms was accompanied by increased dissatisfaction due to high commissions rates and fees~\cite{popper2020diners}, untenable pacing~\cite{dziezaRevoltDeliveryWorkers2021}, and one-sided communication~\cite{thompsonHiddenCostFood2020, DeliveryAppsGrubhub2021,lord2022critical,ma2022brush}. Moreover, restaurants and couriers felt that mainstream food delivery platforms did not support the human intervention needed to make a complex process like food delivery possible~\cite{figueroaEssentialUnprotectedAppbased,dziezaRevoltDeliveryWorkers2021,griswoldAreFoodDelivery2022}. Discontent with the unfavorable terms offered by mainstream platforms, coupled with the availability of white-label software}\footnote{White label software is software that an organization pays for to brand as its own. This software is often sold under a subscription or transaction fee. Users usually do not know the software maker.}, \chadded{facilitated the rise of indie food delivery platforms as an alternative. Despite their growing popularity, indie food delivery platforms remain understudied.} 

%what did we do about the problem
%adjust the language in line 12 to just ask why would people try something other than what they know already works - explain to 2AC that the idea about increased financial risk is really more of a finding
\chdeleted{While some restaurants and drivers have turned to indie platforms as a result of their negative experience with mainstream platforms, this model has downsides too: Indie platforms are financially riskier because they lack the established customer base and technology capabilities to build and maintain a polished food ordering and distribution service~\cite{DeliveryAppsGrubhub2021}. Nonetheless, the stakeholders we talked to, which included restauranteurs, couriers, customers, and platform staff, have been willing to take on these risks to have access to a platform that is embedded within their local community. }
\chdeleted{In this paper, we investigate how indie food delivery platforms operate and what motivates people to join them. We do this by interviewing 28 stakeholders---\textit{restauranteurs}, \textit{couriers}, \textit{customers}, and \textit{administrators}---of an indie platform called \textit{Nosh}, which operates in the northern region of a state in the Western United StatesThe state name has been anonymized for review. While previous HCI research has thoroughly documented the detrimental effects that mainstream platforms have on users (e.g., financial precarity~\cite{ravenelleSideHustleSafety2021}, invasive surveillance~\cite{ravenelle2019we}, and psychological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a}), few studies have explored how users seek out alternatives, such as indie platforms, that could offer them more favorable terms of participation. In this paper we explore what motivates restaurants, customers, and couriers to seek out alternative avenues for participation in the food delivery industry through joining an indie platform \textbf{and} how this indie platform functions, fails, and is repaired. }
\chdeleted{We are guided by two main research questions:
 \textit{What \textbf{motivates} stakeholders to join an indie platform?} We were interested in learning why stakeholders would take the risks associated with a newer indie platform that has a smaller customer base and less technological sophistiation.
\textit{What are the capabilities and limitations of the sociotechnical \textbf{infrastructure} that powers an indie platform?} We were interested in learning how users navigate the comparatively lower-fidelity technology used by indie platforms and if they engaged in additional work to compensate for failures in the technology. }


\chadded{While some restaurants, couriers, and consumers have turned to indie platforms as a result of their negative experience with mainstream platforms, this model has downsides too. Unlike mainstream platforms, indie platforms\chadded{ are relatively small and lack a well-established customer base which makes them a risky venture for restaurants and couriers.} To understand why stakeholders would take on the risks associated with joining an indie platform and how they navigate the socio-technological ecosystem of an indie platform, we ask:}

\begin{description}
\item [RQ1:] \textit{What \textbf{motivates} stakeholders to join an indie platform?} 
\item [RQ2:] \textit{What are the capabilities and limitations of the socio-technical \textbf{infrastructure} that powers an indie platform?} 
\end{description}


%what did we do?
To answer our research questions, we interviewed 28 stakeholders---\textit{restauranteurs}, \textit{couriers}, \textit{customers}, and \textit{administrators}---of an indie platform called \textit{Nosh}, operating in the northern region of a state in the Western United States\footnote{The state name has been anonymized for review}. We asked what motivates restaurants, customers, and couriers to seek out alternative avenues for participation in the food delivery industry through joining an indie platform \textbf{and} how this indie platform functions, fails, and is repaired. We utilized thematic analysis to qualitatively code our data. 
%Using thematic analysis we identified two key themes: (1) all stakeholders highly value human intervention in the process of food delivery (2) human intervention is crucial to making platform-mediated food delivery function.

%what was our contribution?
%we contribute a situated understanding of the role of human intervention in supporting platfomr mediated food delivery 

\chdeleted{We provide three design recommendations for routing, customer support, and dispute resolution processes within food delivery platforms that promote stakeholder well-being. Specifically, our work makes two primary contributions: 
We highlight the role of human intervention. For example, we identify the crucial role of platform administrators as intermediaries between stakeholders and the technical systems when breakdowns occur. We illustrate how human intervention is crucial to repair work  to address infrastructural breakdowns and integral to perceptions of agency and respect that stakeholders seek. 
We demonstrate the need for HCI scholarship to consider the role of business models when making design recommendations for the platform economy.} %We do this through illustrating how the design of systems is constrained by the business models and economic incentives structures in which they operate. 


\chadded{Drawing on a conceptual lens that brings together the platform economy and infrastructure studies from science and technology studies, \textbf{we find that human intervention is a commonplace and necessary part of platform-mediated food delivery}. We found that human intervention plays a crucial role in the process of food delivery: users are willing to leave platforms that penalize interventions for alternative platforms that support them.} \chadded{In this context, human intervention refers to when individuals make an autonomous, ad-hoc decision that goes against algorithmically prescribed instructions, such as modifying an algorithmically recommended driving route for delivery based on road closures. Mainstream platforms tend to punish human intervention, despite its essential role in mediating a complex process such as food delivery.} However, human intervention is essential to the repair work that addresses infrastructural breakdowns and is integral to the perceptions of agency and respect that stakeholders seek. This paper contributes \chadded{a grounded understanding of the role that human intervention plays in making gig work platforms viable and in supporting stakeholders' perceptions of agency. Additionally, \textbf{we reflect on how business models play a vital role in dictating whether socio-technical systems will support human intervention}. Drawing on our findings, we call attention to }the role of business models in shaping the socio-technical systems of digital labor platforms. In particular, we highlight the need to consider the role of business models as an analytical frame when making design recommendations for the platform economy. We conclude by calling for HCI scholars seeking to improve conditions for participants in the platform economy to consider how a platform’s business model enables and constrains the intent of their design recommendations. 




% \chdeleted{While some restaurants and drivers have turned to indie platforms as a result of their negative experience with mainstream platforms, this model has downsides too: Indie platforms are financially riskier because they lack the established customer base and technology capabilities to build and maintain a polished food ordering and distribution service~\cite{DeliveryAppsGrubhub2021}. Nonetheless, the stakeholders we talked to, which included restauranteurs, couriers, customers, and platform staff, have been willing to take on these risks to have access to a platform that is embedded within their local community. }

% \chdeleted{In this paper, we investigate how indie food delivery platforms operate and what motivates people to join them. We do this by interviewing 28 stakeholders---\textit{restauranteurs}, \textit{couriers}, \textit{customers}, and \textit{administrators}---of an indie platform called \textit{Nosh}, which operates in the northern region of a state in the Western United States\footnote{The state name has been anonymized for review}. While previous HCI research has thoroughly documented the detrimental effects that mainstream platforms have on users (e.g., financial precarity~\cite{ravenelleSideHustleSafety2021}, invasive surveillance~\cite{ravenelle2019we}, and psychological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a}), few studies have explored how users seek out alternatives, such as indie platforms, that could offer them more favorable terms of participation. In this paper we explore what motivates restaurants, customers, and couriers to seek out alternative avenues for participation in the food delivery industry through joining an indie platform \textbf{and} how this indie platform functions, fails, and is repaired.} 


% \chdeleted{We are guided by two main research questions:
% \begin{description}
% \item [RQ1:] \textit{What \textbf{motivates} stakeholders to join an indie platform?} We were interested in learning why stakeholders would take the risks associated with a newer indie platform that has a smaller customer base and less technological sophistiation.
% \item [RQ2:] \textit{What are the capabilities and limitations of the sociotechnical \textbf{infrastructure} that powers an indie platform?} We were interested in learning how users navigate the comparatively lower-fidelity technology used by indie platforms and if they engaged in additional work to compensate for failures in the technology. 
% \end{description}}

% \chdeleted{We provide three design recommendations for routing, customer support, and dispute resolution processes within food delivery platforms that promote stakeholder well-being. Specifically, our work makes two primary contributions: 
% \begin{enumerate}
%     \item We highlight the role of human intervention. For example, we identify the crucial role of platform administrators as intermediaries between stakeholders and the technical systems when breakdowns occur. We illustrate how human intervention is crucial to repair work  to address infrastructural breakdowns and integral to perceptions of agency and respect that stakeholders seek. 
%     \item We demonstrate the need for HCI scholarship to consider the role of business models when making design recommendations for the platform economy. %We do this through illustrating how the design of systems is constrained by the business models and economic incentives structures in which they operate. 
% \end{enumerate}}


% % (1) what is topic? (
% In this paper, we set to study \textit{indie}\footnote{We borrow both the term and meanings associated with ``indie'' from music, film, games, and other industries where indie was used to identify small, independent artists supported by an enthusiastic local fanbase who operated separately from the mainstream.} food delivery platforms to better understand why people join them and how they operate. Although scholars have studied the platform economy extensively, they have not focused enough on indie platforms. Scholars have extensively documented the precarity~\cite{ravenelleSideHustleSafety2021}, the invasive surveillance~\cite{ravenelle2019we}, and the psychological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a} of mainstream gig work platforms, especially ride-sharing platforms. In addition to the same problematic labor practices of ride-sharing platforms, mainstream food delivery platforms also grapple with local restaurants' discontent. Indie food delivery platforms have emerged as more localized and community-centric alternatives, but researchers have yet to examine how they function across stakeholders.

% ADD ANOTHER PARAGRAPH THAT SUMMARIZES OUR RELATED WORK 

% Motivated by a desire to design a more just and equitable platform economy, we must understand why people choose to join, engage in, and are impacted by indie food delivery platforms. We set to explore this by answering these two research questions: 
%what is the topic? Indie platforms
%In this paper, we set to study \textit{indie}\footnote{We borrow both the term and meanings associated with ``indie'' from music, film, games, and other industries where indie was used to identify small, independent artists supported by an enthusiastic local fanbase who operated separately from the mainstream.}food delivery platforms to better understand why and how they operate.  Scholars have  studied the platform economy extensively; however, most of their work has focused on the problems of \textit{mainstream} gig work platforms, such as Uber \cite{} and %DoorDash \cite{}, and not much on smaller indieplatforms. Scholars have documented  the financial precarity~\cite{ravenelleSideHustleSafety2021}, the invasive surveillance~\cite{ravenelle2019we}, and the pyschological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a}) of mainstream  platforms.
%negatively impact workers' well-being due to opaque algorithmic management \cite{}, hidden costs of participation \cite{}, and suppression of individual agency ~\cite{}.
%what is the context? Food delivery 
%Furthermore, a lot of research on has focused on \textit{ride-sharing}, without paying enough attention to food delivery. Although mainstream food delivery platforms grapple with labor practices issues too, they also have disenfranchised local restauranteurs \cite{}. 
%Within the food delivery sector of the gig economy, discontent with mainstream platforms has grown since the start of the COVID-19 pandemic. 
%Food delivery platforms coordinate the provision of food from restaurants, directly to consumers via couriers. %Mainstream food delivery platforms charge commission rates to restaurants of up to 30\% in exchange for access to their large customer base~\cite{DeliveryAppsGrubhub2021, thompsonHiddenCostFood2020}. %During COVID-19, restaurants were dependent on access to mainstream food delivery platforms to continue their business and thus had to decide whether to pass on these higher costs and risk losing price-conscious customers or to subsume the costs themselves, reducing already-thin profit margins. 
%Indie platforms, on the other hand, have emerged as alternatives that are more localized and community-centric, but researchers have yet to examine how these platforms operate across stakeholders. 
%Indie food delivery platforms have capitalized on stakeholders' discontent %with the unfavorable terms offered by mainstream platforms, coupled with 
%and leveraged the availability of white label software
%\footnote{White label software is software that an organization pays for to brand as its own. This software is often sold under a subscription or transaction fee. Users usually do not know the software maker.} to operate.
%, facilitated the rise of indie food delivery platforms.
%While indie platforms, beyond the sector of food delivery, have grown in prominence over recent years, there has been little research examining the sociotechnical infrastructure of these alternative systems. 

% what we set to investigate
%To design a more just and equitable platform economy, we need to better understand of how people choose to join, engage in, and are impacted by indie food delivery platforms.% has implications for the design of a more just and equitable platform economy.\par  
%what did we do about the problem
%Although some couriers and restaurateurs have turned to indie platforms as a result of their negative experience with mainstream platforms, switching can have some risks too. %this indie model could have downsides too.%: Indie platforms are financially riskier because they lack the established customer base and technology capabilities to build and maintain a polished food ordering and distribution service~\cite{DeliveryAppsGrubhub2021}. Given the financial risk, why would stakeholders join an indie food delivery platform?  How do stakeholders negotiate the technological capabilities of indie platforms which are less sophisticated than mainstream options? 
%To understand why stakeholders would take on the risks associated with joining an indie platform and how they navigate the socio-technological ecosystem of an indie platform we ask the following research questions:

% \begin{description}
% \item [RQ1:] \textit{What \textbf{motivates} stakeholders to join an indie platform?} 
% \item [RQ2:] \textit{What are the capabilities and limitations of the socio-technical \textbf{infrastructure} that powers an indie platform?} 
% \end{description}


% %what did we do?
% To answer our research questions, we interviewed 28 stakeholders---\textit{restauranteurs}, \textit{couriers}, \textit{customers}, and \textit{administrators}---of an indie platform called \textit{Nosh}, which operates in the northern region of a state in the Western United States\footnote{The state name has been anonymized for review}. We analyzed our data by drawing on a conceptual lens that brings together the platform economy and infrastructure studies from Science and Technology Studies. 
% %While previous research has thoroughly documented the detrimental effects that mainstream platforms have on users (e.g., financial precarity~\cite{ravenelleSideHustleSafety2021}, invasive surveillance~\cite{ravenelle2019we}, and pyschological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a}), few studies have explored how alternatives, such as indie platforms, could offer users more favorable terms of participation. In this paper we explore what motivates restaurants, customers, and couriers to seek out alternative avenues for participation in the food delivery industry through joining an indie platform \textbf{and} how this indie platform functions, fails, and is repaired. 

%what was our contribution?
 
% We found that human intervention plays such a crucial role in the process of food delivery that users are willing to leave platforms that penalize this intervention for alternative platforms that support it. 
% We found that human intervention is an inherent and necessary part of platform-mediated food delivery. Specifically, we find that human intervention is crucial to the repair work that addresses infrastructural breakdowns and integral to perceptions of agency and respect that stakeholders seek. Additionally, we find that the platform's underlying \texit{business values} play a vital role in shaping whether sociotechnical systems will support human intervention. This paper contributes an analytical framework for understanding the role of business values in shaping sociotechnical systems of digital labor platforms. In particular, we bring attention to the need to consider the role of business models as an analytical frame when making design recommendations for the platform economy. HCI scholars seeking to improve conditions for participants in the platform economy must consider how a platform’s business model enables and constrains the intent of their design recommendations.

%Given the financial risk, why would stakeholders, specifically restaurants, couriers, and consumers, join an indie food delivery platform?  How do stakeholders negotiate the technological capabilities of indie platforms which are less sophisticated than mainstream options? 

% While previous HCI research has thoroughly documented the detrimental effects that mainstream platforms have on users (e.g., financial precarity~\cite{ravenelleSideHustleSafety2021}, invasive surveillance~\cite{ravenelle2019we}, and psychological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a}), few studies have explored how alternatives, such as indie platforms, could offer users more favorable terms of participation.  

==> ChiRevisionsVersion/1_Literature_Review.tex <==
\section{Literature Review}
Food delivery platforms create a two-sided market: they match the supply of food from restaurants to the demand for food from consumers and coordinate the delivery of food through a fleet of couriers~\cite{parwezCOVID19PandemicWork2022}. During the lockdown phase of the COVID-19 pandemic, food delivery platforms provided a means for local restaurants to continue their business despite shutting down brick-and-mortar locations. Since then, food delivery platforms have cemented themselves as a permanent fixture in the restaurant industry as they generate record sales and volume~\cite{pewresearch, mckinsey}. 

Despite the usefulness of food delivery platforms, they present challenges to both the restauranteurs and the couriers who rely upon them. Restaurants experience financial precarity as a result of high commission rates and drivers are subject to intrusive surveillance, both of which were exacerbated during the pandemic ~\cite{thorbecke2020impact}. Researchers and journalists have identified structural flaws in food delivery and ride-hailing platforms, ranging from exploitation~\cite{van2017platform,ravenelle2019we,moore2021augmented} to algorithmic control~\cite{woodcock2020algorithmic} to discrimination~\cite{beerepoot,adermon2022gig}. While previous research has documented the harms caused by mainstream food delivery platforms, little work has been done to examine \textbf{how workers and communities have sought to address these harms by supporting local, independent platforms}. In this literature review, we explore the role that food delivery platforms play in supporting the restaurant industry, problems endemic to food delivery platforms, and emergent solutions to those problems. We \chreplaced{utilize infrastructure as a lens}{draw upon infrastructure theory} to add context to our findings of how these platforms function, break down, and are repaired.  

\subsection{What is Infrastructure?}
\chadded{Infrastructure refers to the foundation that underpins any-large scale system; society is dependent upon these systems to conduct everyday activities~\cite{rice2006handbook}. While infrastructure is typically conceived as physical (\textit{e.g.}, roads), information communication technologies are also infrastructures~\cite{hanseth2010design}. These information infrastructures are comprised of digital platforms that allow users and communities to engage with the information systems~\cite{hanseth2010design}.
Information infrastructures have become integral to how people communicate with each other and obtain goods and services in the modern economy. Infrastructures are socio-technical systems that shape and are shaped by social practices ~\cite{edwards2003infrastructure,rice2006handbook}. In other words, infrastructure \emph{``never stands apart from the people who design, maintain and use it,''}~\cite{rice2006handbook}. Thus, infrastructures are value-laden -- they are imbued with the values of their designers~\cite{star1996steps,rice2006handbook}. When the values of designers do not align with the values of users, friction occurs which can result in breakdowns. Breakdowns occur when users encounter ``insurmountable incongruence between the expected infrastructure service and its actual or perceived behavior.''~\cite{pipek2009infrastructuring}. For example, couriers working for food delivery apps can experience breakdowns when the routing instructions given by the platform tell them to take a road that is closed due to poor weather conditions. Examining when infrastructural breakdowns occur allows us to surface the values of designers and users~\cite{dye2019if}.}

\chadded{To mitigate breakdowns, infrastructures should be designed in tandem with users and integrated into existing structures~\cite{rice2006handbook,lee2006human,pipek2009infrastructuring}. However, this requires the acknowledgment of local, end-user expertise~\cite{bowker2009toward}. In the context of the platform economy, where designers are building to achieve scale and universality of their product, the development of flexible systems that incorporate end-user expertise is complicated~\cite{qadri2022seeing}. Qadri and D'Iganazio posit that platforms have a fundamentally different ``vision''~\cite{qadri2022seeing} of the landscape of work from drivers which makes it difficult for them to see and account for end-user expertise~\cite{qadri2022seeing}. The infrastructure of the platform economy ``mediates between the local and global''~\cite{lee2006human}: UberEats is an infrastructure that translates between the global concern for on-demand food delivery and the local concern of how traffic-snarled streets can be navigated as efficiently as possible to complete a delivery order. However, as Qadri demonstrates in her ethnography of delivery drivers in Indonesia~\cite{qadriPlatformWorkersInfrastructures2021}, the translations from local to global in the context of the platform economy are slipshod at best. End-users often develop their own human infrastructures---\emph{``arrangements of organizations and actors that must be brought into alignment in order for work to be accomplished''}~\cite{lee2006human}---to make up for the gaps in translation~\cite{chandra2017market,gray2019ghost,lee2006human}. Human infrastructures play a crucial role in supporting information infrastructures~\cite{lee2006human}. For example, communities come together to maintain and care for networked infrastructures~\cite{dye2019if}, geographically isolated gig workers develop communication networks to make micro-task work tenable~\cite{gray2019ghost}, and delivery drivers build coalitions to maintain rest stops for other drivers~\cite{qadri2022seeing}. Infrastructure literature has thoroughly documented the importance of human infrastructure in supporting large-scale systems~\cite{lee2006human,pipek2009infrastructuring,rice2006handbook}. Despite their importance, human infrastructures are often invisible by nature~\cite{lee2006human}.}

\chadded{In this paper, we use infrastructure as a lens to look beyond the surface-level system functioning to see the power relations embedded in the values which motivate the labor of people on these platforms. We specifically focus on the interaction between human infrastructures and the infrastructures of the platforms they support. In doing so, we are able to better understand the entanglement between local practices and global technologies and why, despite their importance, these local practices remain invisible to some platforms. We adopt Jackson and colleagues' ``broken-world''~\cite{jackson2012repair} thinking to center the ongoing labor involved in maintaining gig work platforms, the values imbued within the platform economy, and the underlying power structures. In the following sections, we examine the infrastructure of platform-mediated food delivery to understand the values imbued within mainstream food delivery platforms, how those values create friction that leads to infrastructural breakdowns, and how end-users engage in repair work to make platforms viable.}

\subsection{What are Food Delivery Platforms?}
GrubHub, founded in 2004, was one of the first food delivery platforms in the United States~\cite{OnlineFoodOrdering2022}. Food delivery platforms coordinate the request, preparation, and delivery of food by connecting restaurants, drivers, and customers through their applications. In other words, they are a platform aggregator: they aggregate supply and demand~\cite{kenneyRisePlatformEconomy2016,zwickWelcomeGigEconomy2018}. These platforms have become a fixture in the restaurant industry, with sales and volume skyrocketing for the largest delivery platforms in recent years~\cite{pewresearch,mckinsey}. %Food delivery platforms such as DoorDash, UberEats, and GrubHub  enable consumers to obtain food, drivers to find work, and restaurants to sell their goods. Users rely on networked online interfaces to conduct an exchange of goods and services. 
While food delivery platforms were popular before 2020, they became an integral part of restaurants' revenue streams after consumers became accustomed to ordering take-out online during the lockdown phase of the COVID-19 pandemic~\cite{mckinsey,pewresearch,smithPeopleHaveEat}. These platforms can be thought of as infrastructure---they are the foundation that underpins the large-scale systems of the food delivery industry~\cite{hanseth2010design}. Like all infrastructures, food delivery platforms are socio-technical systems that are imbued with the values of their designers: They shape and are shaped by social practices~\cite{star1996steps,friedmanValueSensitiveDesign2013a}. \chadded{Moreover, the digital nature of food delivery platforms is inextricable from the social contexts in which they traffic~\cite{van2018platform}. Food delivery platforms re-organize existing social and labor relations of food delivery but are embedded within the same physical institutions (\textit{e.g.} restaurants, delivery drivers, homes in neighborhoods). Thus, tensions arise when the re-organized design of food delivery fails to align with end-user expectations and values.}  

\subsubsection{Value Misalignment Between Designers and Users of Food Delivery Platforms}
Food delivery platforms are designed by software engineers and funded by venture capitalists and are thus imbued with their values~\cite{zuboff2015big}. Food delivery platforms, like DoorDash, are designed by software engineering teams who prioritize high-speed, low-cost delivery by assigning orders to gig workers available nearby regardless of gig workers' preferences~\cite{weinsteinUsingMLOptimization2021}. Couriers are constantly pushed to deliver more, faster: the expected speed of their next delivery is determined by the speed they were able to achieve with past deliveries ~\cite{dziezaRevoltDeliveryWorkers2021}. In some cases, this has led to couriers getting into fatal traffic accidents as they speedily navigate roads on electric bicycles~\cite{figueroaEssentialUnprotectedAppbased}. Platform interfaces are artifacts that reveal the underlying values of their designers; there are few, if any, features on the couriers' mobile application interface that allow for them to articulate their preferences to the platform~\cite{liBottomUp}. \chadded{Numerous infrastructure scholars have pointed to the importance of integrating user input into the design process to ``manage issues of complexity and standardized interfaces between new and existing work infrastructure''~\cite{pipek2009infrastructuring}, yet in most food delivery platforms there are few avenues for this communication to take place.} When the values of designers fail to align with and account for the values of users, such as couriers, problems arise which can result in users being harmed~\cite{Semaan2019,friedmanValueSensitiveDesign2013a}. 

\subsection{What are the Problems with Food Delivery Platforms?}
During the COVID-19 pandemic, demand for the largest food delivery services like Grubhub and UberEats grew as delivery became an integral part of restaurants' business models~\cite{smithPeopleHaveEat}. However, researchers have identified several harms specific to food delivery platforms, including exacerbating workers’ and restaurants’ economic insecurity and pervasive algorithmic control~\cite{parwezCOVID19PandemicWork2022,frankeConnectingEdgeCycles2021,huangRidersStormAmplified2022,woodcock2020algorithmic}. Gig platform scholars assert that these harms are endemic to gig work which functions on the basis of predatory inclusion---the inclusion of marginalized populations into seemingly democratizing arrangements on extractive terms~\cite{mcmillancottomWherePlatformCapitalism2020}. This model of predatory inclusion coupled with opaque algorithmic management creates precarious working conditions~\cite{mcmillancottomWherePlatformCapitalism2020, woodcockGigEconomyCritical2020, van2017platform, popanEmbodiedPrecariatDigital2021, ravenelleSideHustleSafety2021}. While gig platforms market themselves as a novel way for workers to be their own bosses, they often fail to disclose the emotional, physical, and financial costs workers incur by doing so. 

\subsubsection{Problems that couriers experience in the food delivery economy}
Unlike traditional food delivery services (\textit{e.g.}, Pizza Hut phone order delivery), platform delivery services heavily incorporate algorithms into their operations to not only convey logistical information to couriers about their tasks, but also to track their performance~\cite{goods2019your}. This omnipresent surveillance allows companies like UberEats to track the rate at which food couriers accept or deny delivery requests as well as their customer ratings to compile a performance rating of each worker~\cite{veenPlatformCapitalAppetiteControl2020}. Constant surveillance and uncertainty about how they are being managed causes emotional and psychological stress for couriers~\cite{caloTAKINGECONOMYUBER2017,woodcock2020algorithmic,rosenblatAlgorithmicLaborInformation2016a}. Opacity around algorithmically-determined payments creates additional precarity for workers~\cite{goods2019your,calacciBargainingBlackBox2022}. 

Couriers participating in the platform food delivery industry take on financial risk as part of their work. For example, shifting consumer demands, poor weather conditions, and irregular unpaid wait times for restaurant food preparations are common occurrences that can bring couriers’ earnings to below minimum wage~\cite{goods2019your}. Opaque algorithmic management also causes wage insecurity. Platforms will often update their interfaces and algorithms without warning couriers beforehand about how changes will impact their earnings~\cite{calacciBargainingBlackBox2022}. For instance, when the delivery platform Postmates updated their interface to include customizable tipping amounts, couriers feared earning less because consumers may not always be aware that they should tip their delivery driver~\cite{shapiro2018between}. \chdeleted{The economic toll of using delivery platforms also extends to restaurants.}

\chadded{While platform designers are not intentionally trying to develop technologies that harm couriers, the intentional \textit{design choices} they make result in harm regardless. Platform designers value scale and thus embrace abstraction of local contexts: they embrace ``scale-thinking''~\cite{hanna2020against}. This can lead to a failure to consider how their algorithms, such as those that continually increase the expected speed of deliveries, function on the ground where couriers encounter physical barriers and must slow down to be safe~\cite{dziezaRevoltDeliveryWorkers2021}. Business values play a crucial role in dictating what types of interactions are supported by the infrastructure~\cite{shestakofsky2020making}. Value misalignment between designers and users of food delivery platforms extends to restaurants as well.}

\subsubsection{Problems that restaurants experience in the food delivery economy}
After indoor dining was restricted during the pandemic, many restaurants signed up for food delivery services as an alternative revenue stream. However, the mainstream platforms’ high commission rates cut into the earnings of already struggling local businesses~\cite{saxenaDeliveryAppsAre2019}. Restaurants were hesitant to raise prices because doing so may drive away price-sensitive consumers~\cite{DeliveryAppsGrubhub2021, thompsonHiddenCostFood2020}. This put participating restaurants in a situation where they had to take a hit on their already thin profit margins to avoid driving away consumers. These negative impacts have driven some restaurants and couriers to explore alternative options, such as indie platforms, for participating in the food delivery platform economy.  

\begin{figure}[h]
\caption{Software and Services in the Unbundling Economy as described by the founder of a tech company in the food delivery industry}
\label{fig:unbundling}
\includegraphics[width=5cm,height=10cm]{images/unbundling.png}
\end{figure}

\subsection{The Emergence of ``Indie'' Platforms as a Response to Infrastructural Breakdowns}
Small, localized, and community-centric alternative gig platforms have surfaced to fill the gaps left by mainstream services~\cite{atkinsonMoreJobFood2021}. These ``indie'' platforms claim to offer restaurants, drivers, and customers a service that charges lower commissions, cares about the stakeholders involved, and is on the side of the community ~\cite{atkinsonMoreJobFood2021, schneiderExitCommunityStrategies2020,WhyAreRestaurants2021,DeliveryCoopsProvide}. However, there are also drawbacks to indie platforms. They usually do not have as large of a customer base or as sophisticated of technology as mainstream platforms~\cite{DeliveryAppsGrubhub2021}. Research into these new models has been limited, often only focusing on one subset that function as co-operatives~\cite{bundersFeasibilityPlatformCooperatives2022a,scholz2016and,schor2021after}. Our research seeks to expand the conversation around these alternative designs by applying the CSCW and HCI infrastructure literature to understand why these platforms emerge, how they function, and their limitations and advantages. 

\subsubsection{Indie platforms rely on the ``unbundling'' economy for technical infrastructure}
Indie platforms draw upon the ``unbundling'' economy to build their own services from the bottom up. This economy provides software and services for individual elements of the food delivery process: point of sales systems, order aggregation services, and last mile delivery fleets (see Figure~\ref{fig:unbundling} above)~\cite{wangCommissionfreeOnlineOrders2020,wangArmingRebelsFood2021}. These piecemeal systems that attempt to integrate disparate software and services often break down due to incompatibility and difficulty of use. However, prior literature in HCI provides guidance on how users engage in \textit{bricolage} to make piecemeal systems work when mainstream offerings breakdown~\cite{vallgaarda2015interaction,jackson2014RethinkingRepair}. Through the process of bricolage, users extend and repair existing systems through human labor to build an infrastructure that better meets their needs~\cite{vallgaarda2015interaction,jackson2014RethinkingRepair}. \chadded{Firms recombine existing resources (such as those available through the ``unbundling economy'') to create something out of nothing~\cite{baker2005creating}. In doing so, indie food delivery platforms refuse to accept the limitations of the dominant definitions of resources required to compete in the platform economy. Whereas typical firms in the platform economy are well-funded technology firms staffed with engineers, indie food delivery platforms are small, grassroots-funded operations with some technical expertise. Indie platforms are able to operate in the same markets as mainstream platforms because they engage in the creative practice of bricolage~\cite{baker2005creating}. However, the practice of bricolage necessitates human labor and creativity~\cite{baker2005creating,jackson2014RethinkingRepair,vallgaarda2015interaction}.}

\subsubsection{Human labor plays a key role in supporting indie platforms}
Indie platforms build their services by integrating disparate pieces of software into one technology stack, usually without having a fully-staffed software engineer team on hand~\cite{DeliveryCoopsProvide}. In this low-resource environment, technological breakdowns are inevitable~\cite{DeliveryCoopsProvide}. Despite this, indie platforms have continued to survive and grow in prominence because of their small-scale, localized nature and human-centric design~\cite{atkinsonMoreJobFood2021,DeliveryCoopsProvide,holtzCanCoOpsFix2022}. However, little empirical work has been done to understand how indie platforms manage to overcome technological shortcomings. We draw upon the concept of bricolage to better understand how users of indie platforms overcome failures in their technology stack to create a cohesive food delivery service all within a low-resource environment~\cite{baker2005creating}.   

This paper draws upon infrastructure literature and applies it to the context of the food delivery platform economy to develop a better understanding of why users join indie platforms and how these platforms continue to survive despite their lower levels of technological sophistication. We identify how stakeholders surface the values embedded in the infrastructures of mainstream platforms, which become evident during breakdowns, and how value misalignment motivates them to join indie platforms. We examine how top-down construction of infrastructures fails to account for local contexts and highlight the importance of designing to incentivize human intervention in the face of breakdowns. This work expands on design literature in the platform economy by providing guidance for how HCI scholars can develop systems that align with local communities' needs and mesh with the economic incentives of the business model at hand. 




==> ChiRevisionsVersion/2_Methods.tex <==
\section{Background on mainstream and indie food delivery platforms}
In this paper, we differentiate between mainstream and indie food delivery platforms. Here we describe the characteristics of each to highlight the key differences between the two models. We then provide additional details about the empirical setting where we conducted the research.

\subsection{Mainstream food delivery platforms}
% Here's what GrubHub, DoorDash, Uber Eats do operationally and how they describe their business strategy
Mainstream platforms have business models predicated on \textit{market capture}, or the monopolization of a given market. Mainstream platforms have access to large pools of venture capital funding that enables them to operate at a loss ~\cite{DoorDashSharesSink, GrubHubOrdersKeep}. Thus, mainstream platforms are not solely reliant on commissions from orders for profit; rather, they simply need to demonstrate growth or the potential for growth to continue to receive funding. This means that mainstream platforms' success is not strictly predicated on the success of the restaurants and drivers participating in them. This business strategy informs both the technical design of their systems and therefore shapes the nature of interactions that stakeholders have with each other and the platform. 

\begin{figure}[t]
\caption{Difference in financial flows between mainstream platforms and Nosh}
\label{fig:financialflows}
\includegraphics[width=\textwidth]{images/fig1.jpg}
\end{figure}

\subsection{Nosh: an indie food delivery platform}
\subsubsection{Organizational and financial structure} 
In contrast to mainstream platforms, Nosh's business model is rooted in the local communities in which it operates. 
Nosh operates as a ``hub and spoke'' business model. This means that the parent company, Nosh, provides the technology, brand, and initial seed capital for the smaller, local Nosh ``hubs.'' When Nosh comes to a new community, they establish a local Nosh delivery service (\textit{e.g.}, \chreplaced{similar to} how franchises of McDonald's operate). \chadded{Restaurants that join Nosh tend to be locally owned and operated. At the time of our study, no national chains, like McDonalds or Chipotle, were on the Nosh platform. }Each local Nosh delivery service is funded by a coalition of local restaurants that invest seed money into their hub. These "investor" restaurants get voting power over operational decisions in their locale. \chadded{Investor restaurants pay a buy-in fee of approximately \$5,000 which entitles them to a say over operational decisions and a fixed commission rate of 15\%. Restaurants that want to join Nosh but do not want to be investors can join the platform without paying a buy-in fee. However, these \textit {member} restaurants do not get a direct say over operational decisions for their locale and pay a slightly higher commission rate, typically around 20\%.}

The parent company helps each local hub get started by hiring dispatchers and drivers from the community. The parent company also provides the instruction and technical infrastructure needed to run the application. In return, each local Nosh hub shares a percentage of its profit with the parent company. Once dispatchers and drivers have been hired, the investor restaurants begin delivering through the Nosh application. Because Nosh does not have access to venture capital, the platform relies on commissions from their orders and investment from local restaurants. In other words, Nosh's success as a business model is predicated on its stakeholders' success. In Figure~\ref{fig:financialflows} we illustrate how the economic structure of Nosh differs from that of mainstream platforms, particularly how monetary incentives shape relationships between stakeholders and the platform.

Mainstream models rely upon investments from venture capitalists and individual shareholders to finance their operations. This makes mainstream platforms less dependent upon patronage from customers and restaurants as they have access to alternative cash flows. Nosh's model differs from mainstream platforms in terms of economic incentives because the primary investors in the platform are the restaurants themselves. As investors/owners of each local Nosh hub, restaurants contribute to operational decisions and are the platform's primary source of cash flow. The platform's viability is thus tied to stakeholders’ fiscal well-being. Through this model, Nosh is \textbf{beholden} to its stakeholders in ways that mainstream platforms are not. This impacts how the Nosh platform operates, especially in times of breakdown.

%\subsubsection{Nosh the Platform} 
\subsubsection{Nosh relies on a patchwork of technical systems to function}
Food delivery relies upon multiple parties and disparate pieces of software being able to communicate with each other. Nosh uses a suite of proprietary and software-as-a-service technologies to run their business that include:
\begin{itemize}
\item \textit{DataDreamers} for delivery logistics. Although Nosh reported moving to another company's software.
\item \textit{WhenIWork} for courier scheduling and chatting with couriers.  
\item \textit{Zendesk} for customer support.
\item \textit{Slack} for internal communications between dispatchers. 
\item \textit{Google Suite} for generating earning reports for restaurants.
\end{itemize}

While these pieces of software are more affordable than a vertical integration model, breakdowns and confusion often occur, which can frustrate stakeholders.

\subsection{Empirical Setting} %take out methods & put in background section
We conducted an interview study with four stakeholder groups participating in Nosh: restauranteurs, couriers, platform administrators, and customers, to understand what motivates people to join an indie platform. At the time of our interviews, Nosh was operating in two regions. One region encompassed multiple mid-sized cities. The other contained only one major metropolitan area. We have anonymized the region and city names for peer review. We conducted interviews from August to December of 2021. The region is also served by mainstream platforms such as GrubHub, UberEats, DoorDash, and Postmates. %Below we detail our approach for understanding why people joined Nosh and the work they performed within the platform to sustain it. 

\section{Methods}
%Samantha to describe recruitment method
Our study aims to better understand the workings of an indie food delivery operation. We conducted 28 interviews with four stakeholder groups participating in Nosh: restaurants, couriers, customers, and platform administrators. Before conducting the interviews, our protocol and procedures were certified by our institutional review boards. The interview protocols differed for each stakeholder group, but all sought to surface why the subject chose to use Nosh and how they participated in Nosh. We include the interview protocols for each stakeholder group in the appendix. Below we provide more detail on \chdeleted{our positionality as researchers,} the participants, interview protocol, \chreplaced{and data analysis}{data analysis, and limitations}.

%COMMENTING OUT WHILE WE WRITE IT
%\subsection{Positionality Statement}
%Before we continue, we think it would be helpful present the positionality of the (five?) authors of this paper, as it may effect how we view the data. 

%Nikoo: 
%- (Nationality, gender, ethnicity: U.S. born woman of Middle-Eastern 5descent)
%- Age and Education: undergraduate student at an Ivy League institution in her early 20's

% Andrés: Mexican-born and raised, now US-based, male, 42, Ivy league professor, former tech worker <-- i feel like this might deanonymize us easily :)
% Andrés: 
    % no experience a courier or restauranteur 
    % customer: have used several mainstream FDPs, including Uber Eats, Doordash, Postmates. Have not used an indie platform
    % admin: former tech worker, and  platform administrator (but not FDP)

\subsection{Participant Recruitment}
%Our participant pool comprises individuals from four stakeholder groups within Nosh: delivery drivers, restaurateurs, customers, and platform dispatchers or administrators of Nosh. In total, 28 participants across these four stakeholder groups sat for interviews. We selected these stakeholder groups because they played key roles in the food delivery industry. Additional detail about stakeholders is included  in Table~\ref{table:stakeholderlist}.


%\subsubsection{Recruitment Strategy}
%We recruited participants through Nosh via an email list. 
We contacted the founder of Nosh who helped us distribute a call for participation to an email list that was sent out to all restaurants, drivers, platform administrators, and customers that used Nosh. %Once we established contact with participants, we scheduled them for one-hour interviews conducted via Zoom. We read a consent script to participants and received verbal consent to have their interviews recorded and used for this study. We transcribed and removed personally identifiable information from the interviews.  We compensated participants for their time with a \$20 Amazon gift card. 

%\subsubsection{Participant Summary}
In total, we conducted 28 interviews across four stakeholder groups: restauranteurs (n=7), couriers (n=6), customers (n=10), and platform administrators (n=5). %We had seven restauranteurs, six drivers, ten customers, and five platform administrators.
The majority of restauranteurs worked for or owned fast-casual businesses (R1, R2, R4, R5, R6, R7). We spoke to platform administrators who did back-end work (P2), customer-facing work (P1, P5), and managerial work (P3, P4). The drivers we spoke to were evenly split among part-time (D1, D2, D4) and full-time drivers (D3, D5, D6). We  break down our participant demographics in Table~\ref{table:stakeholderlist}.
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}\\

\begin{table}[]
\caption{List of participants broken down by the four stakeholder categories: restauranteurs, platform administrators, couriers, and customers}
\label{table:stakeholderlist}
\begin{tabular}{ll}
\toprule
\textbf{Participant} & \textbf{Occupation Description}    \\
\midrule
\multicolumn{2}{c}{\textit{Restauranteurs}} \\
\hline
R1                   & COO - Chicken Wing Restaurant\\

R2                   & Owner - Tea Shop                \\

R3                   & Owner - Seafood Fine Dining     \\

R4                   & Owner - Wood Fired Pizza        \\

R5                   & Owner - Fast-Casual Take Out    \\

R6                   & Owner - Chicken Wing Restaurant \\

R7                   & Owner - Burger Restaurant       \\
\hline
\multicolumn{2}{c}{\textit{Platform Administrators}}                       \\
\hline

P1                   & Dispatcher                                    \\

P2                   & Data Analyst                                  \\

P3                   & Co-Director of Operations                     \\

P4                   & Co-Director of Operations                     \\

P5                   & Dispatcher                                    \\
\hline
\multicolumn{2}{c}{\textit{Couriers}}                       \\
\hline

D1                   & Driver - Part Time                                    \\

D2                   & Driver - Part Time                                  \\

D3                   & Driver - Full Time                     \\

D4                   & Driver - Part Time                     \\

D5                   & Driver - Full Time                                    \\

D6                   & Driver - Full Time                                    \\
\hline
\multicolumn{2}{c}{\textit{Customers}}                       \\
\hline

C1                   & Health Care Professional                                    \\

C2                   & Office Worker                                  \\

C3                   & Office Worker                     \\

C4                   & Homemaker                     \\

C5                   & Office Worker                                    \\

C6                   & Office Worker                                    \\

C7                   & Office Worker                                    \\

C8                   & Undisclosed                                  \\

C9                   & Office Worker                     \\

C10                   & Undisclosed                    \\
\bottomrule

\end{tabular}
\end{table}

\subsection{Interview Protocol}
The first, second, and third authors conducted one-hour interviews via Zoom. We informed participants of their right to skip  questions or stop the process at any time. We obtained their verbal consent for recording the interview and gave them the option to sign up for a follow-up survey for future research. We transcribed the interviews and anonymized the transcripts. We compensated participants for their time with a \$20 Amazon gift card. 


Our interviews followed semi-structured scripts based on the participant's group affiliation\footnote{see the Appendix for interview protocols}. These scripts focused on surfacing key motivations for participating in Nosh and understanding how participants interacted with the platform. For example, depending on their role, we discussed the pros and cons of delivering for Nosh (drivers), collaborating with Nosh (restaurateurs), ordering from Nosh (customers), and working for Nosh (dispatchers). \chadded{Specifically, for restaurants, couriers, and customers we first asked them about what food delivery platforms they use regularly and why they chose to use Nosh. We then explored how these stakeholders interacted with both Nosh's digital interface and other stakeholders involved in the food delivery process, paying special attention to how they handled breakdowns in the food delivery process both within the context of mainstream platforms and Nosh. The goal of this set of questions was to better understand how these stakeholders handled and repaired infrastructural breakdowns. We concluded interviews with these stakeholders by asking them to describe what a co-op is---because Nosh describes itself as a co-op, even though it is not legally incorporated as one---and what the differences were between this business model and mainstream platform business models. For the platform administrators, we started by asking them to describe their roles and the suite of tools they used to do their jobs. We concluded interviews with the platform administrators by asking them about their interactions with other stakeholders and the community in which they operated to gain a better understanding of the social interactions necessary to make platform-mediated food delivery functional. }The first, second, and third authors manually corrected the automatically-generated transcriptions provided by Zoom by cross-referencing them with the audio recordings. %We then moved on to analyze the corrected transcripts.
%%need to include transition sentence 
\subsection{Data Analysis}
After transcribing each interview, the first, second, and third authors coded the contents using thematic analysis. To standardize the analysis between three people, we conducted preliminary coding where the researchers independently analyzed the same batch of interviews. We then convened afterward to compare and discuss our findings. We also conducted card-sorting exercises to arrive at the final codes. Later, we compiled repeating themes in a centralized codebook, which we then used to code the remainder of the interviews.

\chadded{We frame our findings around two key themes: \textbf{(1) Users' motivations for participating in indie platforms and (2) How users and technology come together to make indie platforms work}. In Section~\ref{sec:motivations} we first identify the essential roles of agency and financial security in motivating restaurants, couriers, and customers to join Nosh. We highlight how the presence of human intervention in the face of breakdowns is a differentiating factor between mainstream platforms and Nosh. In Section~\ref{sec:patchwork} we then examine how users interact with Nosh's technical systems, paying special attention to the key role of platform administrators in serving as buffers between users and the technical systems.}
%Our work reveals two major sets of findings. In Section~\ref{sec:motivations}, we present two primary reasons why restaurants, couriers, and customers were motivated to join Nosh: they achieved a greater level of agency and a greater degree of financial security when participating in Nosh compared to mainstream platforms. In the Table 2~\ref{tab:Table 2} we break down the motivations of restaurants, couriers, and customers for using Nosh. Then in Section~\ref{sec:patchwork}, we present how all stakeholders and technology functioned in tandem to make Nosh work. In Table 3 we break down the pieces of technology each stakeholder group interacted with and the type of repair work they engaged in when using the Nosh platform. 




==> ChiRevisionsVersion/3_Findings.tex <==


\chdeleted{We frame our findings around two key themes: 
Users' motivations for participating in indie platforms and 
How users and technology come together to make indie platforms work
We first identify the essential roles of agency and financial security in motivating restaurants, couriers, and customers to join Nosh. We highlight how the presence of human intervention in the face of breakdowns is a differentiating factor between mainstream platforms and Nosh. Then we examine how users interact with Nosh's technical systems, paying special attention to the key role of platform administrators in serving as buffers between users and the technical systems.}

\section{Why do stakeholders join an indie platform? More agency and financial security}
\chdeleted{Why do stakeholders join an indie platform? More agency and financial security}\label{sec:motivations}



Restaurateurs and couriers joined the indie platform because of a desire for more agency and financial security. Similarly, customers joined because they perceived the indie platform as more ethical, precisely for the same reasons: more agency and financial security for restaurateurs and couriers. See Table~\ref{tab:motivations} for a synthesis of these motivations.


%\subsubsection{Stakeholders Preserve A Greater Degree of Agency in Nosh Compared to Mainstream Platforms}
\subsection{More agency motivates stakeholders to join}
\chdeleted{More agency motivates stakeholders to join}
When participating in mainstream platforms, stakeholders (couriers, restauranteurs, and customers) noted that they are required to fit themselves into the logics of the platforms with little room for negotiation. Processes for participation, operation, and dispute resolution were predetermined by mainstream platforms. This limited stakeholders' ability to exert meaningful control over their participation, advocate for themselves, and come to resolutions they perceived to be fair. In contrast, stakeholders felt that their agency was preserved when using Nosh, which motivated their adoption of the service. Stakeholders’ perception of agency was closely aligned with the presence of human intervention: the ability to interact, reason, and negotiate with a human representative from Nosh gave them a sense of agency that they lacked when participating in mainstream platforms. We demonstrate how agency was defined and identified by restaurants, couriers, and customers below.

\subsubsection{Restauranteurs' agency through transparency and operational input}
Negative experiences with mainstream platforms, such as encounters with dark patterns, drove restauranteurs to seek out alternatives. For example, restauranteurs pointed to non-consensual listings of their business on mainstream platforms as a violation of their agency: 
\begin{quote}\textit{
     ``Grubhub will find our menu put it online without telling us...and then so you'll get a phone call from somebody and then they'll place an online order to pick up. And when they pick up it's it's a Grubhub driver. What they do later is contact you and say hey look you had X amount of deliveries [through] Grubhub, and you know, do you want to sign up for Grubhub?'' (R5)
}\end{quote}

In contrast, because each local hub of Nosh operates as a cooperative run by local restauranteurs, restauranteurs had a direct role in influencing business operations: 
\begin{quote}\textit{
    ``there's a lot of people, giving input and their thoughts, [Nosh] is truly a cooperative where you know matters of importance are voted on and discussed openly. It's very transparent operation from Nosh, the other services, you know no transparency [is] there you know it's just a plug and play... I don't have any say on what happens once I sign up.'' (R6)
}\end{quote}
Having a say over and transparency into operations meant that, in Nosh, restaurants were partners with agency to negotiate their participation. Restauranteurs felt that their ability to negotiate terms of participation with Nosh led to a more equitable relationship than the one they had with mainstream platforms.

\subsubsection{Courier's agency through respect for discretionary decisions}
In mainstream platforms, couriers get their work allocated through an algorithmic system. Also, mainstream platforms tend to punish couriers for deviating from the prescribed instructions even if they had good reason to do so. \begin{quote}\textit{
     ``One thing I also like with Nosh versus DoorDash – Nosh does not track my movements and my location in a way that... If I'm not heading to the restaurant and if I'm biding my own time, it's not going to tell me to turn around or else I'll lose the order. That's something that I remember with DoorDash, that even if there was a large wait time and I didn't head in the direction of the restaurant first, the app would track that and say, 'Are you heading to the restaurant? Looks like you're not heading in the direction of the  restaurant, if you're not going to be heading there in the next couple minutes, we're going to reassign your order to somebody else'.'' (D2)
}\end{quote}
When couriers worked for Nosh, they were able to exercise their best judgment, even if it went against what the dispatching algorithm prescribed, and not be punished for it. The ability to exert control over their work without fear of retribution meant that couriers had a higher degree of agency when working with Nosh.  Several of them pointed out that they felt comfortable deviating from the instructions of the dispatching algorithm because they knew there was always a human dispatcher supervising the system. 
\begin{quote}\textit{
    ``overall, our system is much more fair than other services that I worked for because you have that human aspect of problem solving.'' (D5)
}\end{quote}

Platform administrators could be spoken to and rationalized with, unlike an algorithm. 

\subsubsection{Customers agency through an ability to get a human for support}
Customers discussed their dispute resolution experience with mainstream platforms, emphasizing the one-sided nature of the process with mainstream platforms. \begin{quote}\textit{''One of the times I ordered formula, [Postmates]...delivered the wrong kind. So I reached out and they told me I could return the item. I mean, I get in my car, go return the item, and get what I wanted, and then they gave me a credit. Which I was, like all right fine whatever like that's very irritating that like you should really just send somebody out with the correct thing. And then they refunded my account, but it was a credit on Postmates and then, when I went to use it had been...a while my credit expired...I ended up...not getting that money at all.'' (C2)
 }\end{quote}Here C2 details the frustration that many customers felt with mainstream platforms: they weren't given an option to negotiate what kind of resolution they wanted. In contrast, with Nosh, customers were able to contact a real, local person, for help. Customers feel like they had agency over the situation because they were able to speak with a human and have a say in resolving problems. Customers pointed to the fact that platform administrators always asked them ``what can we do to make this right'' as evidence of their ability to negotiate the outcome. 

 In sum, stakeholders' sense of agency was intimately linked to the presence of human intervention during the course of food delivery. Platform administrators acted as intermediaries between stakeholders and the technical infrastructure of Nosh. Stakeholders could interact and negotiate with platform administrators in a way that they could not with the automated interfaces of mainstream platforms. The ability to engage in two-sided interactions was critical to stakeholders’ agency.
\subsection{Greater financial security motivates stakeholders to join}
\chdeleted{Greater financial security motivates stakeholders to join}

Mainstream platforms dictate the financial costs and benefits of participation. Stakeholders reported that this one-sided negotiation infringed on their ability to achieve financial security in the already low-margin business. With Nosh, restauranteurs reported having lower commission rates and peace of mind knowing that the platform's financial success was tied to theirs. Couriers reported that they had transparency into the fees Nosh extracted from each order, plus the satisfaction of guaranteed floor-pay\footnote{Floor pay is a minimum payment per shift regardless of the number of orders based on the local minimum wage. If couriers did not meet local hourly minimum wages while working, and were not ``gaming'' the system by simply rejecting orders assigned to them, their wage was supplemented by Nosh so that it was equal to the local hourly minimum wage.}, reducing the precarity endemic to independent contractor jobs. Below, we demonstrate how restaurants and couriers were able to attain higher degrees of financial security with Nosh and how customers perceived this as an indicator that Nosh was a more ethical option for food delivery. 

\subsubsection{Restauranteurs' financial security through lower fees and co-ownership}
\chadded{
Restauranteurs reported being too small to negotiate the on average 30\% commission that mainstream platforms charged them. Thus, restauranteurs with already thin profit margins had to raise menu prices to make up for the high commissions charged by mainstream platforms, which they worried would affect their customer base: }
\begin{quote}\textit{
    ``Commission rates are important... and we do raise our prices significantly on delivery platforms to recover a portion of that commission'' (R7). 
}\end{quote}
\chadded{Nosh offered a more financially sound alternative because they charged a 15-20\% commission rate, according to conversations the research team had with Nosh administrators.}

\chadded{Additionally, since each Nosh hub is owned and operated by local restauranteurs, the financial success of the platform is tied to that of the restaurant owners. Thus, restauranteurs had the added security knowing that,  \textit{``...it's not just Nosh's financial success. They're also looking out for each individual  restauranteur's success because \textit{\textbf{[Nosh is]}} those individual restauranteurs``} (R2, emphasis added).}

\subsubsection{Couriers' financial security through floor pay and guaranteed shifts}

\chadded{Couriers reported that, in mainstream platforms, the work was not as flexible as platforms claim because they cannot actually \textit{get} work when they log onto the platform.} 
\begin{quote}\textit{
     ``One of the things with the scheduling and the shifts that they [Nosh] offer is there as a preventative measure to not over-saturate the market with drivers because when you sign on for like DoorDash or like Grubhub, or any of those, there could be hundreds and hundreds of drivers... with Nosh, you know, you can kind of be the big fish in a small pond. If you work hard, and you're efficient and fast, you can make all the money. So there's less saturation I guess is probably the main thing I like about it.'' (D3)
}\end{quote}
\chadded{This courier explicitly calls out Nosh's scheduling system as a key element in promoting financial security. Couriers we interviewed characterized Nosh's hybrid scheduling-open shift system as being \textit{both} more flexible and secure than the "log on and drive" model of mainstream platforms. Nosh's hybrid scheduling-open shift system allows couriers to submit their preferred schedules a week in advance and then assigns couriers shifts based on their availability and preferences. For example, a courier who wanted to work on Tuesday evenings might be assigned the Tuesday dinner rush shift. Couriers could drop shifts, without penalty, after they were assigned by notifying Nosh dispatchers and these shifts would become available in the open shifts tab of the courier's mobile application. This scheduling model combined with Nosh's guaranteed floor-pay provided couriers with a sense of financial security that motivated their participation in Nosh.}

\chadded{Increased agency and financial security made stakeholders feel respected by Nosh: the platform centered food delivery and the stakeholders upholding it. As one restaurant put it:\textit{ “DoorDash and Grubhub are fantastic technology companies that deliver food. Nosh is a fantastic food delivery company that has some technology.”} (R6). This restauranteur  highlights the primary trade-off that stakeholders who participate in Nosh make: access to top-of-the-line technology to facilitate food delivery versus access to more human-centered services that promote agency and respect. Nosh's respect for agency and financial security of restaurants and couriers motivated customers to join as they sought more ethical alternatives for food delivery platforms. }

\subsubsection{Perception of ethicality motivates customers}
 Customers felt that the way Nosh handled the financial aspect of food delivery was more ethical than mainstream platforms.
 Nosh gave couriers and restauranteurs a degree of financial security that they were not able to achieve when working for mainstream platforms. For customers, this motivated them to patronize Nosh because they felt this made the platform a more ethical alternative for food delivery.

Customers articulated feeling strongly about how both restauranteurs and couriers were treated financially by food delivery companies: 
\begin{quote}\textit{
    ``I mean I read the news article, you know, in the Times about how Grubhub and DoorDash are just ripping off restaurants like it's not okay take advantage of people during a pandemic, so I prefer not to use companies that do that.'' (C3)
}\end{quote}

The majority of customers we interviewed described being avid supporters of local restaurants before the COVID-19 pandemic. When the pandemic began, customers sought out ways to patronize local restaurants in an effort to support their community: \textit{``I love that [Nosh] is local so that's my biggest thing...it has a lot of like my favorite local restauranteurs''} (C4). 

Customers noted that even though other food delivery platforms, like DoorDash and UberEats, also had some local restaurants listed, they preferred ordering from Nosh because it was \textit{``just a little bit more ethical''} (C1). For customers, ethical meant that the platform treated both couriers and restauranteurs with respect by not engaging in exploitative financial practices.
 
\begin{table}[]
\centering
\begin{minipage}{1\textwidth}
  \centering
    \begin{tabular}{ll}
        \toprule \textbf{Stakeholder Group} & \textbf{Motivations for Participating In Nosh}  \\ \midrule
        Restaurants & Lower commissions, Increased operational oversight, Dislike of mainstream platforms  \\
        Couriers & Floor pay, Guaranteed shifts, Increased autonomy \\
        Customers  & Support local, Dislike of mainstream platforms, Better customer service \\ \bottomrule
    \end{tabular}
    \caption{Restaurant, Courier, and Customer Motivations for Participating in Nosh}
    \label{tab:motivations}
\end{minipage}
\end{table}

\chdeleted{ \textbf{Restauranteurs' financial security through lower fees and co-ownership.} Restauranteurs reported being too small to negotiate the, on average, 30\% commission that mainstream platforms charged them. Thus, restauranteurs with already thin profit margins had to raise menu prices to make up for the high commissions charged by mainstream platforms, which they worried would affect their customer base: 
    ``Commission rates are important... and we do raise our prices significantly on delivery platforms to recover a portion of that commission'' (R7). 
Nosh offered a more financially sound alternative because they charged a 15-20\% commission rate, according to conversations the research team had with Nosh administrators. } 

\chdeleted{Additionally, since each Nosh hub is owned and operated by local restauranteurs, the financial success of the platform is tied to that of the restaurant owners. Thus, restauranteurs had the added security of knowing that,  \textit{``...it's not just Nosh's financial success. They're also looking out for each individual  restauranteur's success, because \textit{\textbf{[Nosh is]}} those individual restauranteurs``} (R2, emphasis added).}

\chdeleted{\textbf{Couriers' financial security through floor pay and guaranteed shifts.} 
Couriers reported that, in mainstream platforms, the work was not as flexible as platforms claim because they cannot actually \textit{get} work when they log onto the platform. 
     ``One of the things with the scheduling and the shifts that they [Nosh] offer is there as a preventative measure to not over-saturate the market with drivers because when you sign on for like DoorDash or like Grubhub, or any of those, there could be hundreds and hundreds of drivers... with Nosh, you know, you can kind of be the big fish in a small pond. If you work hard, and you're efficient and fast, you can make all the money. So there's less saturation I guess is probably the main thing I like about it.'' (D3)}

\chdeleted{This courier explicitly calls out Nosh's scheduling system as a key element in promoting financial security. Couriers we interviewed characterized Nosh's hybrid scheduling-open shift system as being \textit{both} more flexible and secure than the "log on and drive" model of mainstream platforms. Nosh's hybrid scheduling-open shift system allows couriers to submit their preferred schedules a week in advance and then assigns couriers shifts based on their availability and preferences. For example, a courier who wanted to work on Tuesday evenings might be assigned the Tuesday dinner rush shift. Couriers could drop shifts, without penalty, after they were assigned by notifying Nosh dispatchers and these shifts would become available in the open shifts tab of the courier's mobile application. This scheduling model combined with Nosh's guaranteed floor-pay provided couriers with a sense of financial security that motivated their participation in Nosh.} 


\chdeleted{Increased agency and financial security made stakeholders feel respected by Nosh: the platform centered food delivery and the stakeholders upholding it. As one restaurant put it:\textit{ “DoorDash and Grubhub are fantastic technology companies that deliver food. Nosh is a fantastic food delivery company that has some technology.”} (R6). This restauranteur  highlights the primary trade-off that stakeholders who choose to participate in Nosh make: access to top-of-the-line technology to facilitate food delivery versus access to more human-centred services that promote agency and respect. Nosh's respect for agency and financial security of restaurants and couriers motivated customers to join as they sought more ethical alternatives for food delivery platforms.} 

\chdeleted{Perception of ethicality motivate customers}
 Customers felt that the way Nosh handled the financial aspect of food delivery was more ethical than mainstream platforms.
 Nosh gave couriers and restauranteurs a degree of financial security that they were not able to achieve when working for mainstream platforms. For customers, this motivated them to patronize Nosh because they felt this made the platform a more ethical alternative for food delivery.

Customers articulated feeling strongly about how both restauranteurs and couriers were treated financially by food delivery companies: 
    ``I mean I read the news article, you know, in the Times about how Grubhub and DoorDash are just ripping off restaurants like it's not okay take advantage of people during a pandemic, so I prefer not to use companies that do that.'' (C3)
The majority of customers we interviewed described being avid supporters of local restaurants before the COVID-19 pandemic. When the pandemic began, customers sought out ways to patronize local restaurants in an effort to support their community: \textit{``I love that [Nosh] is local so that's my biggest thing...it has a lot of like my favorite local restauranteurs''} (C4). 

Customers noted that even though other food delivery platforms, like DoorDash and UberEats, also had some local restaurants listed, they preferred ordering from Nosh because it was \textit{``just a little bit more ethical''} (C1). For customers, ethical meant that the platform treated both couriers and restauranteurs with respect by not engaging in exploitative financial practices. %such as taking cuts of couriers tips or charging exorbitant commission fees for restauranteurs. While customers did not have first-hand knowledge about tip distribution or restaurant commissions, they put a lot of stock in popular narratives about mainstream platforms' mistreatment of couriers and restauranteurs. Customers perceived Nosh as respecting restaurateurs and couriers in the way Nosh handled the financial dimensions of food delivery.

%Restaurateurs, couriers, and customers participated in a relatively untested model of indie food delivery because doing so enabled them to exert agency in a way they were previously unable to with mainstream food delivery platforms. Restaurateurs and couriers benefited from a greater degree of financial security, which customers viewed favorably as an indicator that Nosh was a more ethical option for food delivery. A key factor to supporting agency among stakeholders and providing financial security was the presence of human intervention in the process of food delivery: platform administrators negotiated operations with restaurateurs and engaged in the extensive labor necessary to schedule shifts for couriers. How then does Nosh’s infrastructure differ from that of mainstream platforms \textbf{and} how do these difference lead to fundamentally different interactions that stakeholders have with the platform? 

\section{What Makes Nosh Work?: A patchwork of technical systems held together by human intervention}
\chdeleted{What Makes Nosh Work?: A patchwork of technical systems held together by human intervention}\label{sec:patchwork}

Nosh is a patchwork of technical systems held together by human intervention. Nosh relies upon multiple disparate pieces of software to operate. Breakdowns in their patchwork technology stack are commonplace and must be repaired through human intervention. This human intervention is what compels stakeholders to participate in Nosh. However, human intervention requires deep local knowledge, takes time, and \chreplaced{costs}{requires} money. In this section, we outline the contours of Nosh’s technology stack and identify how stakeholders engage in repair work to address gaps and breakdowns, paying special attention to the role of platform administrators. We provide a summary of what technologies each stakeholder interacts with and how they engage in repair work in Table~\ref{tab:repairwork}.

\subsection{Stakeholders struggle with Nosh's patchwork of technical systems}
\chdeleted{Stakeholders struggle with Nosh's patchwork of technical systems}
Restauranteurs we interviewed complained that Nosh's ordering system was clunky and required them to operate not only a separate order aggregation system, but also a tablet dedicated solely to Nosh orders. Mainstream food delivery platforms can integrate directly with most restaurants' point-of-sale software and order aggregation systems, reducing friction in the system. Couriers complained that as a result of the complicated order aggregation system, restaurants often forgot important steps such as starting a countdown timer that couriers relied on to estimate when the order would be ready for pickup: 
\begin{quote}\textit{
    ``it's hard you know because everybody wants to point fingers so it's hard...to say like if they're actually just like \textbf{not able to understand how the app works} or they just didn't start the order because they you know were lazy or busy or whatever. And they're just like oh like, it wasn't actually my fault, like \textbf{the App is bad}.'' (D3, emphasis added)
}\end{quote}

Nosh’s complex technical interface and the inability to integrate it into existing infrastructure resulted in frequent breakdowns that impacted restauranteurs and couriers. Platform administrators, despite their familiarity with the system, also articulated difficulty in navigating the patchwork technical stack Nosh used. 

During the course of a shift, platform administrators said they used, on average, four different platforms simultaneously. One platform administrator describes their shift as follows: \begin{quote}\textit{
    ``No it's an it's a nightmare, we need to...streamline it because my computer just wants to it's like about to  start on fire, because I've got so many things running yeah so so slow, because I always have a million things open''(P3)
}\end{quote} 
Having to jump back and forth between platforms introduced inefficiencies and confusion into their work. Administrators would actively monitor WhenIwork to manage their fleet of couriers, triage customer service requests that came through ZenDesk, answer phone calls from restauranteurs, and coordinate refunds with payroll administrators via Slack. One administrator who oversaw operations at one of the hubs said they wished they could purchase software from Salesforce to streamline their workflow better but it was prohibitively expensive. 

Administrators acted as the buffer between stakeholders and Nosh’s technical infrastructure. When couriers disagreed with delivery instructions or assigned tasks, administrators would be alerted to the situation. For example, couriers recounted times when they were assigned a delivery for a restaurant that was far away towards the end of their shift. In this situation, since the couriers wanted to stop working when their shift ended, they reached out to a platform administrator via chat and asked them to manually re-assign the order to someone else. Another example of human intervention by platform administrators occurs when restaurants ask them for the same detailed profit and loss reports they received from mainstream platforms. Because the DataDreamers software that Nosh used did not support report generation, backend administrators would manually compile these. The limitations of Nosh's technical infrastructure pushed stakeholders to engage in additional invisible labor to make up for shortcomings: 
\begin{quote}\textit{
    ``The point I'm  trying to make is the platform that we currently use is very limited. So there are many things that we can't access, although the  data is there, so we have to kind of find alternatives in order for us  to create visual reports so that we can analyze the data send it to  our couriers and our restauranteurs, etc.'' (P2)
}\end{quote}

Repair work and invisible labor were essential to making Nosh function properly. At all points in the food delivery process, the technical infrastructure of Nosh was subject to breakdowns. Stakeholders throughout the food delivery process intervened when the technical systems broke down, relying on human-intervention to rectify the situation.

\subsection{Human intervention was necessary to overcome breakdowns}
\chdeleted{Human intervention was necessary to overcome breakdowns}

Human operators in Nosh overcame breakdowns through invisible but essential labor. This labor is what the other stakeholders like because they want to interact with people and not machines when things go wrong. However, this requires deep local knowledge and money, and takes time. 

Human mediation plays a critical role in Nosh's operational logic. Platform administrators regularly intervene during the course of food delivery to provide emotional and informational support to restauranteurs, couriers, and customers. As restauranteurs started re-opening and became busier with dine-in traffic, couriers would often have to wait long periods of time to pick up their order. This wait time was compounded by the possibility that restauranteurs did not use the Nosh interface correctly to time the order preparation. To defuse potentially tense situations between restauranteurs and couriers, Nosh administrators 
\begin{quote}\textit{
    ``actually created these templates to send to our couriers that are acting out, getting frustrated with restauranteurs...say[ing] hey we know you're frustrated but we're all a team here let's work together,  here are some ways that you can you know, deal with those types of situations, you  can walk away, you can contact us, you can you know, take a deep  breath.'' (P3).
}\end{quote} 
The goal of these interactions was to show couriers that Nosh stood behind them and wanted to support their well-being on the job. Couriers appreciated these interactions, often explicitly calling out the unique degree of personal connection they had with administrators during our interviews.

A healthy skepticism of the capabilities of the technology used further motivated stakeholders to engage in and rely upon human mediation. Couriers developed rich mental models of what food delivery looked like from the restaurant perspective and anticipated where breakdowns might occur, then worked to address those failure points before problems arose. For example, couriers knew that the restaurant-facing UI was complicated and often led to mistakes with timing so they would call up restauranteurs directly and inquire about order status: \vspace{-1em}\begin{quote}\textit{
    ``So I would literally call every single time every restaurant like ‘I have this order. here's the order number/ here's the name. Anything else you need can you can you let me know if this food has been received by you and do you have any idea how long it's going to take and obviously you know whoever's answering, like the hostess or whoever they're just going to say it's going to take this long, and then you have to like multiply it by three you know, because they don't really know.'' (D3)
}\end{quote}
Many couriers we spoke to learned how to discern whether the person on the phone worked front or back of house and knew they had to speak with someone from the back of the house if they were to get an accurate estimate for their order.

Administrators were also aware that the algorithmic systems underlying the food delivery process were subject to breakdowns. They treated the algorithmic systems they used in a proactive manner; anticipating that \chreplaced{the systems}{it} would break down and require human intervention. As one administrator put it: \textit{``our job as dispatchers is to skim and identify issues.''}\chadded{ (P1). }Administrators played a vital role in manually checking and correcting the logic of the algorithmic system when complications common to food delivery occurred. This contrasts sharply with mainstream platforms, which have little flexibility built in for when situations deviate from what the algorithm prescribes. For example, a courier described a situation where they were delivering multiple orders, but a restaurant had forgotten to start the timer on their end, introducing delays in the process. The courier knew that waiting for the order to be completed would result in the order they had already picked up getting cold, potentially displeasing a customer. The courier reached out to Nosh's dispatchers and informed them of the situation. The dispatcher, understanding that these problems arise in food delivery manually changed the delivery routing system to allow the courier to make a single delivery without being penalized for not picking up the delayed order. Platform administrators are trained to manually intervene in the order dispatching system because they know that problems, such as the one described above, do occur.

Stakeholders act as the glue that holds the technical infrastructure of Nosh together. Platform administrators played a key role in maintaining the cohesiveness of the system: they engage in crucial repair work that takes the form of human-to-human interactions to mediate and patch over breakdowns. Restaurateurs, couriers, and customers point to these interactions as being integral to their perception of being respected and having agency during the process of food delivery. However, platform administrators articulate the limitations of their technology when it comes to supporting the business operating at a larger scale. As one administrator put it: \textit{``you will break the business because there's no way that you can  support the current infrastructure in a big city it's just not gonna work.''} (P2). This highlights a major tension in designing within the platform economy: at scale, human-to-human interactions that promote sentiments of respect and agency are often untenable.
%Brian pls help the table is compiled in the discussion and not the findings

\begin{table}[]
\begin{tabular}{lll}
\toprule
\multicolumn{1}{c}{\textbf{Stakeholder Group }} & \multicolumn{1}{c}{\textbf{Primary Technologies Used}} & \multicolumn{1}{c}{\textbf{Repair Work Performed}} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Restaurants \end{tabular} & \begin{tabular}[c]{@{}l@{}}Nosh Tablet\end{tabular} & \begin{tabular}[c]{@{}l@{}}NA \end{tabular}   \\ \midrule
\begin{tabular}[c]{@{}l@{}}Couriers\end{tabular} & \begin{tabular}[c]{@{}l@{}}DataDreamers App \\ WhenIWork \\ Cellphone\end{tabular}  &  \begin{tabular}[c]{@{}l@{}}Communicating with restaurants\\and customers\end{tabular}    \\ \midrule
\begin{tabular}[c]{@{}l@{}}Customers\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Nosh Mobile App\end{tabular}   & \begin{tabular}[c]{@{}l@{}}NA\end{tabular}  \\ \midrule
\begin{tabular}[c]{@{}l@{}}Platform Administrators\end{tabular} & \begin{tabular}[c]{@{}l@{}}DataDreamers app, WhenIWork,\\ZenDesk, GSuite, Slack, \\Cell Phone, Computer\end{tabular} & \begin{tabular}[c]{@{}l@{}}Dispute Resolution\end{tabular}\\ \bottomrule
\end{tabular}
\caption{Technologies Stakeholders Interact With and Repair Work Performed}
\label{tab:repairwork}
\end{table}




\chdeleted{Restauranteurs' agency through transparency and operational input.
Negative experiences with mainstream platforms, such as encounters with dark patterns, drove restauranteurs to seek out alternatives. For example, restauranteurs pointed to non-consensual listings of their business on mainstream platforms as a violation of their agency: 
     ``Grubhub will find our menu put it online without telling us...and then so you'll get a phone call from somebody and then they'll place an online order to pick up. And when they pick up it's it's a Grubhub driver. What they do later is contact you and say hey look you had X amount of deliveries [through] Grubhub, and you know, do you want to sign up for Grubhub?'' (R5)
In contrast, because each local hub of Nosh operates as a co-operative run by local restauranteurs, restauranteurs had a direct role in influencing business operations: 
    ``there's a lot of people, giving input and their thoughts, [Nosh] is truly a cooperative where you know matters of importance are voted on and discussed openly. It's very transparent operation from Nosh, the other services, you know no transparency [is] there you know it's just a plug and play... I don't have any say on what happens once I sign up.'' (R6)
Having a say over and transparency into operations meant that, in Nosh, restaurants were partners with agency to negotiate their participation. Restauranteurs felt that their ability to negotiate terms of participation with Nosh led to a more equitable relationship than the one they had with mainstream platforms.} 

\chdeleted{Courier's agency through respect for discretionary decisions.
In mainstream platforms, couriers get their work allocated through an algorithmic system. Also, mainstream platforms tend to punish couriers for deviating from the prescribed instructions even if they had good reason to do so. 
     ``One thing I also like with Nosh versus DoorDash – Nosh does not track my movements and my location in a way that... If I'm not heading to the restaurant and if I'm biding my own time, it's not going to tell me to turn around or else I'll lose the order. That's something that I remember with DoorDash, that even if there was a large wait time and I didn't head in the direction of the restaurant first, the app would track that and say, 'Are you heading to the restaurant? Looks like you're not heading in the direction of the  restaurant, if you're not going to be heading there in the next couple minutes, we're going to reassign your order to somebody else'.'' (D2)
When couriers worked for Nosh, they were able to exercise their best judgment, even if it went against what the dispatching algorithm prescribed, and not be punished for it. The ability to exert control over their work without fear of retribution meant that couriers had a higher degree of agency when working with Nosh.  Several of them pointed out that they felt comfortable deviating from the instructions of the dispatching algorithm because they knew there was always a human dispatcher supervising the system. 
    ``overall, our system is much more fair than other services that I worked for because you have that human aspect of problem solving.'' (D5)
Platform administrators could be spoken to and rationalized with, unlike an algorithm.} 

\chdeleted{Customers agency through an ability to get a human for support. Customers discussed their dispute resolution experience with mainstream platforms, emphasizing the one-sided nature of the process with mainstream platforms. ''One of the times I ordered formula, [Postmates]...delivered the wrong kind. So I reached out and I they told me I could return the item. I mean, I get in my car, go return the item, and get what I wanted, and then they gave me a credit. Which I was, like all right fine whatever like that's very irritating that like you should really just send somebody out with the correct thing. And then they refunded my account, but it was a credit on Postmates and then, when I went to use it had been...a while my credit expired...I ended up...not getting that money at all.'' (C2)
 Here C2 details the frustration that many customers felt with mainstream platforms: they weren't given the option to negotiate what kind of resolution they wanted. In contrast, with Nosh, customers were able to contact a real, local person, for help. Customers feel like they had agency over the situation because they were able to speak with a human and have a say in resolving problems. Customers pointed to the fact that platform administrators always asked them ``what can we do to make this right'' as evidence of their ability to negotiate the outcome.}





==> ChiRevisionsVersion/4_Discussion.tex <==
% \section{Discussion}
% \subsection{Breakdowns are inevitable in the platform economy}
% Broken world thinking, technologies perform “unexpectedly, otherwise than anticipated, or not at all” (Leszczynski, 2020) → why do things break? Platform economy is unpredictable and the design of algorithmic systems requires simplification. These simplifications can fail to capture the context at hand (Qadri). When designing a system the development of standards & simplification is required - these are value-ladden choices, what is noticed & what is ignored (Star, Pipek).

% However, when breakdowns occur, people fix them (or try to). People engage in unique problem solving, collaboration, and technical mastery (Jackson et. al). We see this in our findings. This intervention is undervalued by platforms (Qadri, Watkins, Chandra, Gray & Suri, Salehi). 

% \subsection{Human intervention remains undervalued and unseen in the platform economy}
% In the platform economy, design choices are guided by technosolutionist thinking that sidelines the importance of human interaction and intervention. → stems from scale thinking (Hanna & Park, Qadri) & captialism in general (Scott, Schnieder) 

% When designing systems of work, “user participation is a pragmatic approach to…manage issues of complexity and standardized interfaces between new and existing work infrastructure.” (Pipek). Why isn’t this done more? 

% \subsection{Business models and economic incentives enable and constrain design recommendations intended to support human intervention}
% Mainstream platforms prioritize massive growth in hopes of achieving monopolization over the market, at which point they can dictate the terms of participation (Graham 2012, Sullivan 2016). To achieve growth, platforms must operate at scale. At scale, the metis (local knowledge) is rejected in favor of standardized, low-context, low-resolution global knowledge (Qadri, Scott). In other words, business models built for scale are unable to support the interaction of deep situated human knowledge needed to make their infrastructures more flexible. 

% When making design recommendations intended to create a more just and equitable platform economy that supports human actors, researchers should consider the business they’re operating within. Some business models (e.g. subsidarity) can be better suited to supporting human intervention & local knowledge than scalability models. If researchers want to create a more just & equitable platform economy they should explore how subsidiarity models (like Nosh) can be supported through technological innovations. 

\section{Discussion}

\chreplaced{Our findings show that (1) infrastructural breakdowns are inevitable in platform-mediated food delivery, (2) human intervention is essential to address these breakdowns, and (3) stakeholders' perceptions of agency---the ability to interact, reason, and negotiate with a human representative---is intimately linked to the presence of human intervention. When breakdowns occur, human actors must intervene to repair the process of food delivery. However, these acts of human intervention are treated normatively differently depending on the platform \textit{type}. Under mainstream platforms such as DoorDash and UberEats, human intervention is viewed as extraneous to the algorithmically prescribed process and is punished. Indie platforms like Nosh, in contrast, view human intervention as an inherent part of the food delivery process and rely upon it. Human intervention allows for two-sided communication between the platform and stakeholders, which is integral to an increased sense of \textit{agency}. Restaurants, couriers, and customers highly value the ability to retain and exercise agency in an algorithmically mediated system. Stakeholders are willing to join a smaller, less well-known, and less technologically sophisticated indie platform that supports human intervention and offers them the ability to retain and exercise agency. }{Human intervention is both commonplace and necessary in the platform economy. Technical infrastructures underlying the platform economy sometimes break down in local contexts, requiring people to repair them. However, mainstream platforms and indie platforms handle breakdowns in vastly different ways. Nosh's processes for handling breakdowns demonstrate why human intervention should be incentivized rather than penalized, and we propose several mechanisms through which human intervention can be promoted. To explore the feasibility of these design recommendations, we call attention to the importance of business models and economic constraints of platforms seeking to incentivize human intervention.} 

\chreplaced{In this section, we discuss and extend our findings. In the first section, we demonstrate why breakdowns are inevitable in the platform economy and how humans intervene to engage in repair work. In the second section, we discuss several reasons why human intervention remains undervalued and unseen by mainstream platforms. We conclude by demonstrating how business models can be used as an analytical tool to help designers effectively assess whether their recommendations will work in practice to support human intervention in the platform economy. We show that the tension between scale and human-centered design is a navigable one by drawing attention to the role business models play in shaping infrastructures that support human intervention. However, we demonstrate that addressing this tension requires a shift in thinking about economic and organizational facets of the infrastructure underlying the platform economy.}{We first briefly restate our research questions and corresponding findings to provide a high-level overview of the implications for design. We then translate these implications for design into concrete recommendations with considerations for business models and economic constraints.}

\chdeleted{We first briefly restate our research questions and corresponding findings to provide a high-level overview of the implications for design. We then translate these implication for design into concrete recommendations with considerations for business model and economic constraints.}

\chdeleted{RQ1: What motivates stakeholders to join an indie platform?}
    \chdeleted{Findings: We find that restaurants, couriers, and customers join Nosh because they are afforded a higher degree of agency and financial security.}
        \chdeleted{Implications for Design: Design of automated systems in food delivery (\textit{e.g.} Routing systems, dispute resolution, etc,.) should not penalize human intervention and should instead accept that human intervention is necessary.} 
        \chdeleted{Explanation: The sentiments of agency and ability to attain a higher degree of financial security are inextricable from the presence of human intervention in the face of breakdowns. Having a platform administrator act as a buffer between users and technical systems enabled stakeholders to negotiate and build trust with an entity they felt understood and looked out for them.} 

    \chdeleted{RQ2: What are the capabilities and limitations of the sociotechnical infrastructure that powers an indie platform?}
    \chdeleted{Findings: The infrastructure of Nosh is made up of a patchwork of software systems that tend to breakdown and frustrate users. Users overcome these frustrations through human intervention, usually on the part of platform administrators. The current system works well enough at a local level, because there are local support staff, but would most likely fail if scaled up.} 
        \chdeleted{Implications for Design: Design of food delivery platform systems needs to take into account the business model and economic incentives at hand.}
        \chdeleted{Explanation: Nosh's model was able to continue operating with relatively unsophisticated technology infrastructure because their business model was set up to service local hubs. Each local hub had its own support staff that had rich knowledge of the stakeholders in that community and the ability to address their concerns effectively. Additionally, Nosh was able to rationalize its human labor costs because they were entirely reliant upon restaurants and customers for profits so they had extremely strong incentives to provide excellent support service.} 

\chdeleted{In sum, users joined Nosh because of the human intervention, thus design for systems to support food delivery should account for key role it plays. This level of human intervention would not be viable under mainstream business models that have differing economic incentive structures. However, it is worthwhile to explore how technical solutions can be developed to support alternative business models like Nosh because they offer a fundamentally different, more human-centric, organization of work in the food delivery platform economy that promotes agency, respect, and financial security. We expand on these claims below in more detail.}

% \subsection{Breakdowns are inevitable in the platform economy}
% Broken world thinking, technologies perform “unexpectedly, otherwise than anticipated, or not at all” (Leszczynski, 2020) → why do things break? Platform economy is unpredictable and the design of algorithmic systems requires simplification. These simplifications can fail to capture the context at hand (Qadri). When designing a system the development of standards & simplification is required - these are value-ladden choices, what is noticed & what is ignored (Star, Pipek).

% However, when breakdowns occur, people fix them (or try to). People engage in unique problem solving, collaboration, and technical mastery (Jackson et. al). We see this in our findings. This intervention is undervalued by platforms (Qadri, Watkins, Chandra, Gray & Suri, Salehi). 
\subsection{Breakdowns are inevitable in food delivery platforms}
\chdeleted{Breakdowns are inevitable in food delivery platforms}
\chadded{As our findings demonstrate, }during the course of platform-mediated food delivery, breakdowns are guaranteed to occur: unexpected traffic jams block routes, restaurants overlook details of orders during rush hour, and customers receive cold food. \chreplaced{S}{Previous work has highlighted that s}ystems of coordinated workflows fail due to a disparity between how they are designed and how they are actually used in practice, leading to inevitable breakdowns~\cite{grudinWHYCSCWAPPLICATIONS,leszczynski2020glitchy,lord2022critical}. \chadded{In the platform economy, algorithms are used to orchestrate work processes, such as matching the supply of couriers with demand from consumers. However, algorithmic systems require that work processes be simplified, standardized, and codified~\cite{qadri2022seeing}. When infrastructure designers simplify work processes, they make value-laden decisions about which features are extraneous to the design of their system~\cite{pipek2009infrastructuring}. Mismatches between users' and designers' values can result in breakdowns~\cite{rice2006handbook,pipek2009infrastructuring}. For example, an engineer working at DoorDash's San Francisco office may not anticipate that heavy snowfall in Denver occasionally causes road closures when they are designing routing algorithms. In the case of unexpected road closures, the couriers we spoke to improvised alternative delivery routes. However, as D2 noted, these deviations were punished by DoorDash. Despite the importance of human intervention in making platform-mediated work functional, designers often fail to consider \textit{human intervention} as a relevant factor in design process~\cite{chandra2017market,gray2019ghost,qadriPlatformWorkersInfrastructures2021,salehi2015we}. By examining breakdowns within the food delivery process, we were able to identify the invisible, but essential human labor that goes into repairing breakdowns.}

\chadded{Infrastructure scholarship shows us that the `re-conceptualization of breakdowns as normal'~\cite{dye2019if,jackson2012repair} can help surface and center the underlying labor, values, and power of systems. In Nosh, systems constantly broke down. However, rather than viewing these points of failure as abnormalities, platform administrators and couriers treated them as an inherent and expected feature of food delivery. In particular, platform administrators discussed how they constantly monitored the algorithmic systems for failure, and couriers discussed how they anticipated human error arising on behalf of the restaurants. These two stakeholder groups integrated acts of repair work into their everyday navigation of Nosh's infrastructure. In doing so, they not only maintained but also \textit{transformed} Nosh's infrastructure in a way that preserved humanistic values and gave it the flexibility to function in an unpredictable and idiosyncratic context~\cite{jackson2014RethinkingRepair}. Nosh recognized the \textit{value} of this repair work and relied upon it to make their platform functional. However, our stakeholders expressed that under mainstream food delivery platforms this repair work was not only unrecognized but also punished as a deviation from algorithmically prescribed instructions. Given the importance of repair work in the process of platform-mediated food delivery, why do mainstream platforms fail to recognize and value this process while indie platforms design for it? We argue that this failure can be traced back to the operational logic of mainstream platforms which prioritize automation and scalability.}

\subsection{Human intervention remains undervalued and unseen in the mainstream platform economy}
\chadded{The presence of human intervention played a significant role in addressing breakdowns during the course of food delivery. Despite the essential role human intervention plays in making the platform economy viable, it is often unseen and undervalued by mainstream platforms~\cite{elish2020repairing,gray2019ghost}. Drawing on critical labor and feminist critique, we hypothesize that human intervention remains unsupported in mainstream platforms because their `methods of seeing'~\cite{qadri2022seeing} preclude the inclusion of contextual and high-resolution data and their `scale thinking'~\cite{hanna2020against} over-simplifies complex work processes.}

\chadded{In Nosh, platform administrators proactively monitored the dispatching algorithm and communicated with couriers throughout their shifts. Nosh was able to \textit{see} the landscape of food delivery through the couriers' eyes, allowing the administrators to make manual adjustments to algorithmically prescribed instructions when reality didn't align with predictions. By incorporating couriers' vision into the operation of the platform, Nosh was able to not only foster couriers' sense of agency but also maintain the flexibility of their infrastructure. In contrast, mainstream platforms rely on ``large observational datasets, which are granular but low-context and low-resolution"~\cite{qadri2022seeing}. These datasets fail to capture the nuances of the landscape that couriers perceive and thus constrain the vision of the platform. Additionally, couriers have limited ways of communicating directly with administrators at mainstream platforms. Because mainstream platforms' methods of seeing overlooks the rich, local knowledge needed to support gig work, the human intervention that makes platforms functional often remains overlooked.}

\chadded{Mainstream platforms not only overlook the importance of human intervention, but they also undervalue it. Many mainstream platforms fall prey to `scale thinking'---the unwavering commitment to growth through scalability~\cite{hanna2020against,selbst2019fairness}. In the context of algorithmically mediated work, this type of thinking can result in the design of infrastructures that fail to account for local complexity~\cite{qadri2022seeing,hasinoff2022scalability}. Algorithmic code designed for scale makes simplifying assumptions that fail to account for the complexities of gig work, such as unexpected road closures and human error when preparing a complicated order. As we saw with D2, scale thinking can lead to breakdowns when edge cases that are unaccounted for arise. Unlike algorithmic code, platform administrators are able to respond to and address unforeseen edge cases. Despite its low-fidelity infrastructure, Nosh was able to effectively address breakdowns because it integrated human intervention and expertise into its infrastructure. Involving users in the design of infrastructure is ``a pragmatic approach to...manage issues of complexity and standardized interfaces between new and existing work infrastructure.''~\cite{pipek2009infrastructuring}. Yet, mainstream platforms often fail to account for, integrate, and value the local expertise of stakeholders.}

\chadded{Neglect of local expertise and human intervention in large-scale algorithmic systems can be traced back to computational disciplines that prioritize universal technology design~\cite{jacksonPolicyKnotReintegrating2014,qadri2022seeing}. In the context of gig work, mainstream platforms attempt to supplant local expertise with algorithmic systems: Human labor is seen as something to automate away, a hopefully fungible cost~\cite{iraniDifferenceDependenceDigital2015,doornPlatformCapitalismHidden2020}. However, the view that data-intensive algorithmic models can solve fundamentally human problems is misguided: the integration of human expertise into algorithmic systems makes them more robust in practice. Stakeholders identified how they relied upon their local expertise to navigate the food delivery process in both mainstream and indie platforms. Yet, the value placed on local expertise differed by type of platform. Within Nosh, human intervention was not only supported, but also heavily relied upon;  within mainstream platforms, human intervention was not only seen as an error but was also punished. By examining what types of interventions were supported, we can surface underlying value systems and the factors that inform them~\cite{shestakofsky2020making}.}

\subsection{Business models enable and constrain the design of infrastructures}
\chadded{Mainstream platforms do not ascribe value to the labor stakeholders perform in their acts of repair, despite the fact that these acts make the platform economy viable. We contend that platforms' business models inform their values which work to enable and constrain infrastructures that support human intervention~\cite{shestakofsky2020making,hasinoff2022scalability}. Mainstream platforms' business models prioritize scalability in order to secure funding from venture capitalists and subsequent valuation from shareholders~\cite{graham2012startup,sullivan2016blitzscaling}. The business imperative to scale drives the development of algorithms that can ``expand without having to change itself in substantial ways or rethinking its constitutive elements''~\cite{hanna2020against}. To demonstrate how business models inform value systems and subsequent infrastructure design, we discuss how three different design recommendations, while empirically informed by our findings, would fail in practice in the context of mainstream platforms. We then conclude with a call for researchers to examine the economic and organizational features of the platform economy when attempting to design to support human intervention.}

\subsubsection{Design recommendations intended to support human intervention  fail under mainstream business models.}
\chadded{\textbf{Making Room for Courier Discretion:}} \chadded{We found that couriers within Nosh rely upon their knowledge of local geography and familiarity with local restaurants to perform their jobs. Couriers highlighted that the ability to exercise agency during the course of food delivery without fear of retribution was a contributing factor to why they liked working for Nosh more than mainstream platforms. Therefore, food delivery platforms should avoid threatening drivers for reasonable deviations from the prescribed route. In mainstream platforms, allowing for driver discretion would introduce complexity into their fleet management systems which oversee thousands, not dozens, of couriers, and would obstruct their ability to prevent gaming behavior by couriers. Essentially, the scale at which mainstream platforms operate constrains the efficacy of this design recommendation. Additionally, each local Nosh hub hires couriers through an interview process, while mainstream platforms offer a ``log on and drive'' model, limiting the ability to verify courier expertise and capability which contributes to the defensive design of their algorithmic management systems~\cite{rahmanInvisibleCageWorkers2021a}.}

\chadded{\textbf{Promote Humans-in-the-Loop in Delivery Operations: }}\chadded{Restaurants, customers, and couriers valued the presence of human platform administrators who intervened when systems broke down. The human agents in Nosh were helpful to the other stakeholders because they were locally situated: each hub had its own staff of platform administrators that assisted customers, restaurants, and couriers operating within that hub. Thus, these platform administrators could provide relevant and responsive support that understood the contexts in which other stakeholders were operating. In contrast, mainstream food delivery platforms operate at a national scale and do not have regional hubs staffed with local support agents to support the commerce of each hub~\cite{beharBuildingUnifiedChat2022,GrubhubEasyCustomer}. Providing the localized support that restaurants, customers, and couriers value would necessitate that mainstream platforms decentralize their operations and establish regional hubs.}

\chadded{\textbf{Build Systems That Support Transparent Two-sided Dispute Resolution:}} \chadded{Restaurants we spoke to were appreciative of the support they received from Nosh when problems arose, characterizing Nosh as straightforward and transparent. In contrast, they characterized their experiences with mainstream platforms as frustrating and one-sided. For Nosh, it was extremely important to maintain restaurant satisfaction \textit{because Nosh was entirely dependent on restaurants for investment}. Mainstream platforms---as we depict in Figure~\ref{fig:financialflows}---do not have the same degree of financial obligation to restaurants \textit{because they have access to venture capital and shareholder investment}. These differences in financial dependence fundamentally shape how stakeholders are treated in both systems. It would be difficult to enforce the implementation of more nuanced dispute resolution processes without strong economic incentives. Reiterating what R2 said: \textit{``...it's not just Nosh's financial success, they're also looking out for each individual  restaurant's success because \textbf{[Nosh is]} those individual restaurants''} (emphasis added).}

\subsubsection{A path forward: Broadening the scope of design research to include policy and economic considerations}
\chadded{HCI scholars studying the platform economy often share the goal of trying to improve the conditions for participants by mitigating the negative impacts of technical systems through re-imagining their design. However, the technical interventions proposed often fail to consider the role of policy and economic incentives in shaping their feasibility~\cite{jacksonPolicyKnotReintegrating2014}. Attempting to improve conditions in the platform economy solely through technical interventions without considering the contexts in which those interventions would operate limits HCI scholars' ability to understand \textbf{\textit{what}} these interventions will fundamentally change: stopping at design leaves many questions unanswered. It is well established that the platform economy, despite its claims of offering liberatory access to on-demand work, further entrenches systems of oppression and marginalization (\textit{e.g.}~\cite{mcmillancottomWherePlatformCapitalism2020}); but what, realistically, are technical design recommendations doing to fundamentally reorganize the structure of the platform economy to avoid predatory inclusion and precarious conditions?} 

\chadded{We call for HCI researchers seeking to improve conditions in the platform economy to examine two paths forward:} 
\begin{enumerate}
    \item \textbf{Consider the ``Policy Knot'' that shapes the efficacy of design recommendations.} As Jackson and colleagues suggest, it is imperative for HCI scholars to think through how policy plays a key constitutive role in shaping the deployment and effects of technology~\cite{jacksonPolicyKnotReintegrating2014}. In the case of food delivery platforms, we call for HCI scholars to examine how policy, such as regulations of the types of funding mechanisms available to co-ops versus limited liability corporations, constrain the viability of alternative \textit{business models} that are necessary to support technical interventions that improve conditions of participation. HCI scholars do not need to be completely reliant on external domain expertise for guidance on how to study policy constraints on organizations. Rather, they can turn to early HCI and CSCW work, such as that done by Susan Leigh Star, Wanda Orlikowski, and Anselm Strauss for methodological guidance on conducting empirical research that incorporates policy and organizational factors as key elements of design investigations~\cite{orlikowskiInformationTechnologyStructuring1991,orlikowskiStudyingInformationTechnology1991,starLayersSilenceArenas1999,straussSocialOrganizationMedical1997}. 
    \item \textbf{Continue to examine alternative models within the platform economy.} As Glen Weyl suggests, it is essential for scholars to consider and contribute to the plurality of options in the marketplace~\cite{weylWhyAmPluralist2022}. In other words, it is important that scholars continue to investigate how we can further diversify the options available for participation rather than settle into the mindset that we must operate only within existing options. In the context of food delivery platforms, we call for HCI scholars to continue investigating how alternative models for food delivery can be viable \textit{and} simultaneously support participant well-being. \chadded{Specifically, HCI researchers should investigate how subsidiarity business models, like Nosh, function in comparison to scalability business models, like UberEats and DoorDash~\cite{hasinoff2022scalability}. }\chreplaced{HCI scholars could also explore how to support subsidiarity models through technical mechanisms for governance and coordination across multiple localized hubs to provide organizational knowledge and resources to their employees.}{This could look like HCI scholars exploring technical mechanisms for governance and coordination across multiple localized hubs that operate under one parent company that provides technical and knowledge resources.} 
\end{enumerate}

\chadded{Complicating design recommendations within the broader considerations of social, political, and economic contexts is not new to the fields of HCI and CSCW, especially in the context of systems of coordinated work ~\cite{starLayersSilenceArenas1999,straussSocialOrganizationMedical1997,grudinWHYCSCWAPPLICATIONS}. By presenting our design recommendations and complicating them by considering the constraints of business models and economic incentives, we draw attention to the need for HCI scholars to consider how proposed technical interventions will work to fundamentally reshape some of the root causes of negative impacts experienced by users. We urge HCI scholars to consider the role of policy in informing the impacts of design, however well-intentioned that design may be, and encourage them to continue exploring how a plurality of options for participation in the platform economy can be supported through technical design. In the words of Susan Leigh Star and Anslem Strauss, two eminent figures in the field of infrastructure studies within CSCW and HCI, we call for HCI researchers to \textit{``look in every circumstance at how the application affects relations of power and the nature of work.''}~\cite{starLayersSilenceArenas1999}.}
% % \chadded{Given that integration of user feedback and expertise is a well established approach to designing infrastructures that are robust in practice, why do mainstream platforms  fail to do so? Business models are a fruitful analytical framework for understanding \textit{why} certain platforms' infrastructures support human intervention.}
% % \chadded{Before they became public companies, Uber, DoorDash, and GrubHub relied heavily on venture capital funding to support their growth. To secure funding, business models typically need to be designed for \textit{scalability}~\cite{graham2012startup,sullivan2016blitzscaling}. As we discuss above, designing for scalability results in oversimplification of work processes. Moreover, because platforms fail to see the invisible labor of human intervention that is crucial to addressing infrastructural breakdowns, they believe they are the `sole authors of their success and broadly proclaim the successes of scale and abstraction'~\cite{qadri2022seeing}. }
% \subsection{Business models and economic incentives enable and constrain design recommendations intended to support human intervention}
% Mainstream platforms prioritize massive growth in hopes of achieving monopolization over the market, at which point they can dictate the terms of participation (Graham 2012, Sullivan 2016). To achieve growth, platforms must operate at scale. At scale, the metis (local knowledge) is rejected in favor of standardized, low-context, low-resolution global knowledge (Qadri, Scott). In other words, business models built for scale are unable to support the interaction of deep situated human knowledge needed to make their infrastructures more flexible. 

% When making design recommendations intended to create a more just and equitable platform economy that supports human actors, researchers should consider the business they’re operating within. Some business models (e.g. subsidarity) can be better suited to supporting human intervention & local knowledge than scalability models. If researchers want to create a more just & equitable platform economy they should explore how subsidiarity models (like Nosh) can be supported through technological innovations. 

\chdeleted{Domain expertise is essential to address breakdowns}
\chdeleted{Despite the responsibility of breakdowns falling on users, our participants noted that they were often penalized by mainstream platforms for stepping in when the intervention did not fit into the intended design. As D2 pointed out, DoorDash would threaten to take away a delivery if they did not exactly follow the prescribed route, even if their desired route avoided delays and roadblocks. Being unable to exercise discretion in their jobs left restaurateurs and drivers feeling like they lacked the agency to make decisions and have input, even though they were domain experts. Disregarding domain expertise is a longstanding trend in the design of algorithmic systems
%~\cite{petreGamingSystemPlatform2019,sambasivanDeskillingDomainExpertise2022,starLayersSilenceArenas1999}
. Failing to recognize users' domain expertise in conducting food delivery emerged as one weakness in the logic of mainstream food delivery platforms. In contrast, Nosh recognized the essential role of domain expertise and, in many cases, their platform \textbf{relied} upon it. As a result, our participants had \textbf{agency} over their participation. Re-iterating what R6 said: \textit{``DoorDash and Grubhub are fantastic technology companies that deliver food. Nosh is a fantastic food delivery company that has some technology.''}}  

\chdeleted{Design for the platform economy should incentivize human intervention}
\chdeleted{The design of systems in the platform economy is typically defensive: platforms are concerned with workers gaming the system. Thus platform owners design systems to harshly penalize behavior that deviates from what they prescribe
% ~\cite{rahmanInvisibleCageWorkers2021a,watkinsTookPicGot2020,gray2019ghost}
. However, doing so penalizes users for attempting to rely on their expertise to repair breakdowns as they occur
%~\cite{qadriPlatformWorkersInfrastructures2021}
. Nosh did \textit{not} penalize users for leaning on their domain expertise, rather they incorporated it as a fixture in their platform. Platform administrators embodied this notion of human intervention and input as essential to the function of a delivery platform: they were able to understand edge cases in ways algorithms could not. Centering human intervention in the Nosh platform was a key factor in motivating users to join and enabling the constant repair of the platform in light of its low-fidelity technological infrastructure. Building on this case study, we propose several design recommendations for building systems in the platform food delivery industry that could incentivize human intervention:} 

    \chdeleted{Design routing algorithms that allow for courier discretion (e.g., avoid threatening drivers for reasonable deviations from the prescribed route). }
    \chdeleted{Make a concerted effort to keep humans in the loop (e.g., have a group of designated platform administrators for each locale to act as support staff).}
    \chdeleted{ Allow for transparent two-sided negotiation in dispute resolution processes rather than relying on cookie-cutter feedback forms and pre-determined solutions (e.g., build a stronger customer relationship management process to track issues and resolutions).}

\chdeleted{We provide a speculative example of our design recommendations in action to illustrate how this more human-centred technology stack might work. One scenario where we could apply these designs is during a two-batch order when a courier picks up two separate orders that have different drop off locations. Issues with batch orders are common in mainstream platforms: long wait times at restaurants frustrate couriers and customers~\cite{after-brickBatchingOrdersJust2021}. With our recommendations, if the restaurant preparing the second order suddenly changed the estimated preparation time due to a last-minute dinner rush, the driver could drop off the first order rather than wait for the second order to be prepared---letting the first get cold and risking upsetting the customer---\textbf{because} they would not be penalized for going against the prescribed route. If a customer was unhappy with their order, a local platform dispatcher could reach out to understand the problem and determine an acceptable solution. Doing so would clarify which party might be at fault, thereby avoiding penalizing the incorrect party for something out of their control. Through increased transparency, restaurants and couriers could better understand reparative actions from the platform. As our findings show, centering human intervention in coordinated work systems is essential to increasing user confidence: the ability to understand and be heard by human intermediaries increased user agency and reinforced positive perceptions of Nosh.}  

\chdeleted{However, these design recommendations --- though empirically informed --- are virtually impossible for mainstream platforms to implement due to incompatible business models and economic constraints. Thus, in the next section, we discuss how economic incentives shape design in action and how HCI researchers can reflect upon these constraints when making design recommendations.} 

% \chdeleted{\subsection{Business model and economic structure enable and constrain design recommendations}}
% \chdeleted{Design recommendations are limited in impact if they fail to consider the business model, organizational constraints, and economic dimensions at hand. Thus, HCI scholars need guidance to navigate design recommendations that may not be supported by platforms' economic incentives and business model.}

% \chdeleted{\subsubsection{Why our design recommendations wouldn't work in a mainstream food delivery platform}}
% \chdeleted{While the design recommendations we make above are empirically informed, they are derived within the context of an indie food delivery model. It would be difficult, if not impossible, to apply these recommendations to a mainstream food delivery platform given the values and economic constraints at hand. We review each recommendation and explain which factors of mainstream models hamper their efficacy.} 
%     \chdeleted{Making Room for Courier Discretion: In mainstream platforms, allowing for driver discretion would introduce complexity into their fleet management systems which oversee thousands, not dozens, of couriers and would obstruct their ability to prevent gaming behavior by couriers. Essentially, the scale at which mainstream platforms operate constrains the efficacy of this design recommendation. Additionally, each local Nosh hub hires couriers through an interview process, while mainstream platforms offer a ``log on and drive'' model, limiting the ability to verify courier expertise and capability which contributes to the defensive design of their algorithmic management systems~\cite{rahmanInvisibleCageWorkers2021a}.} 
    
%     \chdeleted{romote Humans-in-the-Loop in Delivery Operations: Restaurants, customers, and couriers valued the presence of human platform administrators who intervened when systems broke down. The human agents in Nosh were helpful to the other stakeholders because they were locally situated: each hub had its own staff of platform administrators that assisted customers, restaurants, and couriers operating within that hub. Thus, these platform administrators could provide relevant and responsive support that understood the contexts in which other stakeholders were operating. In contrast, mainstream food delivery platforms operate at a national scale and do not have regional hubs staffed with local support agents to support the commerce of each hub~\cite{beharBuildingUnifiedChat2022,GrubhubEasyCustomer}. Providing the localized support that restaurants, customers, and couriers value would necessitate that mainstream platforms decentralize their operations and establish regional hubs.}
    
%     \chdeleted{Build Systems That Support Transparent Two-sided Dispute Resolution: Restaurants we spoke to were appreciative of the transparency and support they received from Nosh when problems arose, characterizing Nosh as straightforward and transparent, in contrast to experiences with mainstream platforms as frustrating and one-sided. For Nosh, it was extremely important to maintain restaurant satisfaction \textit{because Nosh was entirely dependent on restaurants for investment}. In contrast, mainstream platforms---as we depict in Figure~\ref{fig:financialflows}---do not have the same degree of financial obligation to restaurants \textit{because they have access to venture capital and shareholder investment}. These differences in financial dependence fundamentally shape how stakeholders are treated in both systems. It would be difficult to enforce the implementation of more nuanced dispute resolution processes without strong economic incentives. Reiterating what R2 said: \textit{``...it's not just Nosh's financial success, they're also looking out for each individual  restaurant's success because \textbf{[Nosh is]} those individual restaurants''} (emphasis added).}


% As our \chreplaced{findings}{finding} demonstrate, human intervention is both \chreplaced{commonplace}{normal} and necessary in the platform economy. \chadded{Moreover, restaurants, customers, and couriers are willing to join a financially riskier and less technologically sophisticated indie platform because this platform supported human intervention whereas mainstream platforms punished intervention. In particular, stakeholders associated Nosh's respect for human intervention when breakdowns occurred with increased agency within an algorithmic system.} Technical infrastructures underlying the platform economy sometimes break down in local contexts, requiring people to repair them. However, mainstream platforms and indie platforms handle breakdowns in vastly different ways. Nosh’s handling of breakdowns demonstrates why human intervention should be incentivized rather than penalized\chreplaced{.}{ and we propose several mechanisms through which human intervention can be promoted.}

% \chreplaced{In our discussion, we first draw upon critical infrastructuring literature concerning repair work to contextualize our finding that human intervention played a crucial role in making the food delivery process viable. We then compare and contrast the values embedded in Nosh's and mainstream platforms' infrastructures to demonstrate how the values of the latter inform socio-technical systems that fail to support human intervention. In doing so, we highlight how business models play a fundamental role in informing the value systems of gig work platforms. Finally, we argue that business models should be used as an analytical framework when making design recommendations because they enable and constrain the efficacy and intent of researchers' interventions.}{To explore the feasibility of these design recommendations, we call attention to the importance of business models and economic constraints of platforms seeking to incentivize human intervention.}

% \chdeleted{We first briefly restate our research questions and corresponding findings to provide a high-level overview of the implications for design. We then translate these implication for design into concrete recommendations with considerations for business model and economic constraints.}

% \chdeleted{\begin{itemize}}
%     \chdeleted{\item} \chdeleted{\textbf{RQ1: What motivates stakeholders to join an indie platform?}}
%     \chdeleted{\begin{itemize}}
%         \chdeleted{\item}\chdeleted{ \textbf{Findings}: We find that restaurants, couriers, and customers join Nosh because they are afforded a higher degree of agency and financial security.}
%         \chdeleted{\item} \chdeleted{\textbf{Implications for Design}: Design of automated systems in food delivery (\textit{e.g.} Routing systems, dispute resolution, etc,.) should not penalize human intervention and should instead accept that human intervention is necessary.} 
%         \chdeleted{\item}\chdeleted{\textbf{Explanation}: The sentiments of agency and ability to attain a higher degree of financial security are inextricable from the presence of human intervention in the face of breakdowns. Having a platform administrator act as a buffer between users and technical systems enabled stakeholders to negotiate and build trust with an entity they felt understood and looked out for them.} 
%     \chdeleted{\end{itemize}}
%     \chdeleted{\item \textbf{RQ2: What are the capabilities and limitations of the sociotechnical infrastructure that powers an indie platform?}}
%     \chdeleted{\begin{itemize}}
%         \chdeleted{\item \textbf{Findings}: The infrastructure of Nosh is made up of a patchwork of software systems that tend to breakdown and frustrate users. Users overcome these frustrations through human intervention, usually on the part of platform administrators. The current system works well enough at a local level, because there are local support staff, but would most likely fail if scaled up.} 
%         \chdeleted{\item \textbf{Implications for Design}: Design of food delivery platform systems needs to take into account the business model and economic incentives at hand.}
%         \chdeleted{\item \textbf{Explanation}: Nosh's model was able to continue operating with relatively unsophisticated technology infrastructure \textit{because} their business model was set up to service local hubs. Each local hub had its own support staff that had rich knowledge of the stakeholders in that community and the ability to address their concerns effectively. Additionally, Nosh was able to rationalize its human labor costs because they were entirely reliant upon restaurants and customers for profits so they had extremely strong incentives to provide excellent support service.} 
%     \chdeleted{\end{itemize}}
% \chdeleted{\end{itemize}}

% \chdeleted{In sum, users joined Nosh because of the human intervention, thus design for systems to support food delivery should account for key role it plays. This level of human intervention would not be viable under mainstream business models that have differing economic incentive structures. However, it is worthwhile to explore how technical solutions can be developed to support alternative business models like Nosh because they offer a fundamentally different, more human-centric, organization of work in the food delivery platform economy that promotes agency, respect, and financial security. We expand on these claims below in more detail.} 
  
% \subsection{Human intervention is normal and necessary in the platform economy}
% \chreplaced{\subsubsection{Breakdowns are inevitable in the platform economy}}{\subsubsection{Breakdowns are inevitable in food delivery platforms}}
% During the course of platform-mediated food delivery, breakdowns are guaranteed to occur: unexpected traffic jams block routes, restaurants overlook details of an order during rush hour, and customers receive cold food. \chadded{Previous HCI research on the platform economy demonstrates that these types of breakdowns are bound to occur due to mismatches between assumptions that platform designers make and reality that workers face~\cite{qadri2022seeing,qadriPlatformWorkersInfrastructures2021,chandra2017market}. For example, Qadri and D'Ignazio point out that Gojek, a popular rideshare and food delivery platform in Indonesia, "sees" the landscape of work in a fundamentally different way than the drivers do~\cite{qadri2022seeing}. Gojek, like other mainstream gig work platforms, relies on large datasets that are "granular but low-context and low-resolution"~\cite{qadri2022seeing} to inform its algorithmic decision-making. These datasets fail to incorporate the rich and locally situated knowledge that drivers draw upon to navigate the highly variable and unpredictable nature of gig work. Mainstream gig work platforms rely upon an oversimplified view of the work they organize thus resulting in breakdowns.}\chadded{The design of infrastructures necessitates simplification to reduce complexity~\cite{pipek2009infrastructuring}. These decisions are often implicit during the design process and thus the assumptions made are rarely evident until breakdowns occur~\cite{pipek2009infrastructuring,rice2006handbook,lee2006human,dye2019if}. }
% %insert something on broken-world thinking to normalize breakdowns in the platform economy and shift to a focus on the ongoing labors, interests, and powers underpinning the platfomr economy 
% \chdeleted{Previous work has highlighted that systems of coordinated workflows fail due to a disparity between how they are designed and how they are actually used in practice---making breakdowns inevitable~\cite{grudinWHYCSCWAPPLICATIONS}}. \chadded{However, as our findings show, when breakdowns occur, those affected engage in acts of repair through bricolage---stiching together disparate pieces of technology to accomplish their work~\cite{vallgaarda2015interaction,jackson2014RethinkingRepair}.} 
% %However, the decisions about what simplification to make when developing design standards are ethically loaded because they entail a value judgement~\cite{rice2006handbook}. 
% %\chreplaced{~\cite{grudinWHYCSCWAPPLICATIONS,starLayersSilenceArenas1999,straussSocialOrganizationMedical1997}}{

% \chreplaced{\subsubsection{Humans engage in critical infrastructuring to repair breakdowns}}{\subsubsection{Domain expertise is essential to address breakdowns}}
% %when breakdowns occur people must step in to repair systems

% \chadded{Our participants discussed how in both mainstream platforms and in Nosh they had to engage in repair work when breakdowns occurred.}
% Despite the responsibility of breakdowns falling on users, our participants noted that they were often penalized by mainstream platforms for stepping in when the intervention did not fit into the intended design. As D2 pointed out, DoorDash would threaten to take away a delivery if they did not exactly follow the prescribed route, even if their desired route avoided delays and roadblocks. Being unable to exercise discretion in their jobs left restaurateurs and drivers feeling like they lacked agency to make decisions and have input, even though they were domain experts. Disregarding domain expertise is a longstanding trend in the design of algorithmic systems~\cite{petreGamingSystemPlatform2019,sambasivanDeskillingDomainExpertise2022,starLayersSilenceArenas1999}. Failing to recognize users' domain expertise in conducting food delivery emerged as one weakness in the logic of mainstream food delivery platforms. In contrast, Nosh recognized the essential role of domain expertise and, in many cases, their platform \textbf{relied} upon it. As a result, our participants had \textbf{agency} over their participation. Re-iterating what R6 said: \textit{``DoorDash and Grubhub are fantastic technology companies that deliver food. Nosh is a fantastic food delivery company that has some technology.''}  

% \chreplaced{\subsubsection{Platforms' values dictate what labor they "see"}}{\subsubsection{Design for the platform economy should incentivize human intervention}}
% %people repair breakdowns but this repair work is typically invisible 
% %what labor platforms see and recognize is dictated by their values --> if they value automation, then slow messy human labor isn't going to be recognized as vital to the system
% %transition to how increasing platforms' vision is contingent on platforms valuing those new forms of sight --> business models & economic incentives 
% The design of systems in the platform economy is typically defensive: platforms are concerned with workers gaming the system. Thus platform owners design systems to harshly penalize behavior that deviates from what they prescribe~\cite{rahmanInvisibleCageWorkers2021a,watkinsTookPicGot2020,gray2019ghost}. However, doing so penalizes users for attempting to rely on their expertise to repair breakdowns as they occur~\cite{qadriPlatformWorkersInfrastructures2021}. Nosh did \textit{not} penalize users for leaning on their domain expertise, rather they incorporated it as a fixture in their platform. Platform administrators embodied this notion of human intervention and input as essential to the function of a delivery platform: they were able to understand edge cases in ways algorithms could not. Centering human intervention in the Nosh platform was a key factor in motivating users to join and enabling the constant repair of the platform in light of its low-fidelity technological infrastructure. Building on this case study, we propose several design recommendations for building systems in the platform food delivery industry that could incentivize human intervention: 

% \begin{itemize}
%     \item Design routing algorithms that allow for courier discretion (e.g., avoid threatening drivers for reasonable deviations from the prescribed route). 
%     \item Make a concerted effort to keep humans in the loop (e.g., have a group of designated platform administrators for each locale to act as support staff).
%     \item Allow for transparent two-sided negotiation in dispute resolution processes rather than relying on cookie-cutter feedback forms and pre-determined solutions (e.g., build a stronger customer relationship management process to track issues and resolutions).
% \end{itemize}

% We provide a speculative example of our design recommendations in action to illustrate how this more human-centred technology stack might work. One scenario where we could apply these designs is during a two-batch order when a courier picks up two separate orders that have different drop off locations. Issues with batch orders are common in mainstream platforms: long wait times at restaurants frustrate couriers and customers~\cite{after-brickBatchingOrdersJust2021}. With our recommendations, if the restaurant preparing the second order suddenly changed the estimated preparation time due to a last-minute dinner rush, the driver could drop off the first order rather than wait for the second order to be prepared---letting the first get cold and risking upsetting the customer---\textbf{because} they would not be penalized for going against the prescribed route. If a customer was unhappy with their order, a local platform dispatcher could reach out to understand the problem and determine an acceptable solution. Doing so would clarify which party might be at fault, thereby avoiding penalizing the incorrect party for something out of their control. Through increased transparency, restaurants and couriers could better understand reparative actions from the platform. As our findings show, centering human intervention in coordinated work systems is essential to increasing user confidence: the ability to understand and be heard by human intermediaries increased user agency and reinforced positive perceptions of Nosh.  

% However, these design recommendations --- though empirically informed --- are virtually impossible for mainstream platforms to implement due to incompatible business models and economic constraints. Thus, in the next section, we discuss how economic incentives shape design in action and how HCI researchers can reflect upon these constraints when making design recommendations. 

% \subsection{Business model and economic structure enable and constrain design recommendations}
% Design recommendations are limited in impact if they fail to consider the business model, organizational constraints, and economic dimensions at hand. Thus, HCI scholars need guidance to navigate design recommendations that may not be supported by platforms' economic incentives and business model.

% \subsubsection{Why our design recommendations wouldn't work in a mainstream food delivery platform}
% While the design recommendations we make above are empirically informed, they are derived within the context of an indie food delivery model. It would be difficult, if not impossible, to apply these recommendations to a mainstream food delivery platform given the values and economic constraints at hand. We review each recommendation and explain which factors of mainstream models hamper their efficacy. 


% \begin{itemize}
%     \item \textbf{Making Room for Courier Discretion:} In mainstream platforms, allowing for driver discretion would introduce complexity into their fleet management systems which oversee thousands, not dozens, of couriers and would obstruct their ability to prevent gaming behavior by couriers. Essentially, the scale at which mainstream platforms operate constrains the efficacy of this design recommendation. Additionally, each local Nosh hub hires couriers through an interview process, while mainstream platforms offer a ``log on and drive'' model, limiting the ability to verify courier expertise and capability which contributes to the defensive design of their algorithmic management systems~\cite{rahmanInvisibleCageWorkers2021a}. 
    
%     \item \textbf{Promote Humans-in-the-Loop in Delivery Operations:} Restaurants, customers, and couriers valued the presence of human platform administrators who intervened when systems broke down. The human agents in Nosh were helpful to the other stakeholders because they were locally situated: each hub had its own staff of platform administrators that assisted customers, restaurants, and couriers operating within that hub. Thus, these platform administrators could provide relevant and responsive support that understood the contexts in which other stakeholders were operating. In contrast, mainstream food delivery platforms operate at a national scale and do not have regional hubs staffed with local support agents to support the commerce of each hub~\cite{beharBuildingUnifiedChat2022,GrubhubEasyCustomer}. Providing the localized support that restaurants, customers, and couriers value would necessitate that mainstream platforms decentralize their operations and establish regional hubs.
    
%     \item \textbf{Build Systems That Support Transparent Two-sided Dispute Resolution:} Restaurants we spoke to were appreciative of the transparency and support they received from Nosh when problems arose, characterizing Nosh as straightforward and transparent, in contrast to experiences with mainstream platforms as frustrating and one-sided. For Nosh, it was extremely important to maintain restaurant satisfaction \textit{because Nosh was entirely dependent on restaurants for investment}. In contrast, mainstream platforms---as we depict in Figure~\ref{fig:financialflows}---do not have the same degree of financial obligation to restaurants \textit{because they have access to venture capital and shareholder investment}. These differences in financial dependence fundamentally shape how stakeholders are treated in both systems. It would be difficult to enforce the implementation of more nuanced dispute resolution processes without strong economic incentives. Reiterating what R2 said: \textit{``...it's not just Nosh's financial success, they're also looking out for each individual  restaurant's success because \textbf{[Nosh is]} those individual restaurants''} (emphasis added).
% \end{itemize}

% \subsubsection{A path forward: Broadening the scope of design research to include policy and economic considerations}
% HCI scholars studying the platform economy often share the goal of trying to improve the conditions for participants by mitigating the negative impacts of technical systems through re-imagining their design. However, the technical interventions proposed often fail to consider the role of policy and economic incentives in shaping their feasibility~\cite{jacksonPolicyKnotReintegrating2014}. Attempting to improve conditions in the platform economy solely through technical interventions without considering the contexts in which those interventions would operate limits HCI scholars' ability to understand \textbf{\textit{what}} these interventions will fundamentally change: stopping at design leaves many questions unanswered. It is well established that the platform economy, despite its claims of offering liberatory access to on-demand work, further entrenches systems of oppression and marginalization (\textit{e.g.}~\cite{mcmillancottomWherePlatformCapitalism2020}); But what, realistically, are technical design recommendations doing to fundamentally reorganize the structure of the platform economy to avoid predatory inclusion and precarious conditions?  

% We call for HCI researchers seeking to improve conditions in the platform economy to examine two paths forward: 
% \begin{enumerate}
%     \item \textbf{Consider the ``Policy Knot'' that shapes the efficacy of design recommendations.} As Jackson and colleagues suggest, it is imperative for HCI scholars to think through how policy plays a key constitutive role in shaping the deployment and effects of technology~\cite{jacksonPolicyKnotReintegrating2014}. In the case of food delivery platforms, we call for HCI scholars to examine how policy, such as securities law, constrain the viability of alternative \textit{business models} that are necessary to support technical interventions that improve conditions of participation. HCI scholars do not need to be completely reliant on external domain expertise for guidance on how to study policy constraints on organizations. Rather, they can turn to early HCI and CSCW work, such as that done by Susan Leigh Star, Wanda Orlikowski, and Anselm Strauss for methdological guidance on conducting empirical research that incorporates policy and organizational factors as key elements of design investigations~\cite{orlikowskiInformationTechnologyStructuring1991,orlikowskiStudyingInformationTechnology1991,starLayersSilenceArenas1999,straussSocialOrganizationMedical1997}. 
%     \item \textbf{Continue to examine alternative models within the platform economy.} As Glen Weyl suggests, it is essential for scholars to consider and contribute to the plurality of options in the marketplace~\cite{weylWhyAmPluralist2022}. In other words, it is important that scholars continue to investigate how we can further diversify the options available for participation rather than settle into the mindset that we must operate only within existing options. In the context of food delivery platforms, we call for HCI scholars to continue investigating how alternative models for food delivery can be viable \textit{and} simultaneously support participant well-being. This could look like HCI scholars exploring technical mechanisms for governance and coordination across multiple localized hubs that operate under one parent company that provides technical and knowledge resources.  
% \end{enumerate}

% Complicating design recommendations with broader considerations for the social, political, and economic contexts at hand is not new to the fields of HCI and CSCW, especially in the context of systems of coordinated work ~\cite{starLayersSilenceArenas1999,straussSocialOrganizationMedical1997,grudinWHYCSCWAPPLICATIONS}. By presenting our design recommendations and then complicating them by considering the constraints of business models and economic incentives, we draw attention to the need for HCI scholars to consider how proposed technical interventions will work to fundamentally re-shape some of the root causes of negative impacts experienced by users. We urge HCI scholars to consider the role of policy in informing the impacts of design, however well-intentioned that design may be, and encourage them to continue exploring how a plurality of options for participation in the platform economy can be supported through technical design. In the words of Susan Leigh Star and Anslem Strauss, two eminent figures in the field of infrastructure studies within CSCW and HCI, we call for HCI researchers to \textit{``look in every circumstance at how the application affects relations of power and the nature of work.''}~\cite{starLayersSilenceArenas1999}. 

==> ChiRevisionsVersion/5_Limitations_Future_Work.tex <==
\section{Limitations}
Our results might not generalize to other indie platforms because we studied a single platform. This platform's location and idiosyncrasies are likely to influence our insights.  Also,  our participant sample is biased because those who responded to our call for participation felt strongly enough about expressing their opinion that they chose to sit for an hour-long interview.  In the future, we plan to expand this research to hundreds of other indie platforms in the United States and gather latent data from online sources beyond interviews.

==> ChiRevisionsVersion/6_Conclusion.tex <==
\section{Conclusion}

We discovered the essential role that human intervention plays in making food delivery platform users feel respected. Restaurants, couriers, platform administrators, and customers all took the risk of participating in a relatively untested model of indie delivery because they were given a greater degree of agency and financial security which made them feel respected in ways they were not when participating in mainstream food delivery platforms. When breakdowns occurred during the process of food delivery, stakeholders were able to understand, establish control over, and shape the outcome of the situation. Drivers, restaurants, and customers valued the ability to interact and negotiate with a human representative in a way they were unable to with the algorithmic systems of mainstream platforms. Human intervention from Nosh platform administrators played a key role in smoothing over breakdowns as administrators acted as a buffer between stakeholders and the technology. Drivers also stepped up to intervene when algorithmic systems broke down and felt comfortable doing so because they knew a human dispatch agent was available to reason with. We \chreplaced{argue for platform infrastructure design}{put forth recommendations to build routing, dispatching, and customer service systems for food delivery platforms} that incentivize human intervention given the inevitability of its occurrence. We \chreplaced{highlight the role that business models play in enabling and constraining the design of infrastructures that support human intervention. Specifically, we show that business models that prioritize scalability are ill-suited to supporting human intervention whereas business models that operate as subsidiarities are better able to do so.}{caveat our recommendations with the note that incentivization of human intervention is not viable under most business models of mainstream food delivery.} Thus we call for HCI scholars to return to traditions from the early days of the field to be attentive to the broader social, political, and economic contexts at hand when making design recommendations. 

==> ChiRevisionsVersion/Changes.tex <==
\DIFdelbegin \DIFdel{section}%DIFDELCMD < {%%%
\DIFdel{Introduction}%DIFDELCMD < }
%DIFDELCMD < %%%
\DIFdel{Mainstream food delivery platforms , such as }\textit{\DIFdel{UberEats}}%DIFAUXCMD
\DIFdel{, }\textit{\DIFdel{DoorDash}}%DIFAUXCMD
\DIFdel{, and }\textit{\DIFdel{Grubhub}}%DIFAUXCMD
\DIFdel{, more than doubled in  popularity in the United States during the COVID-19 pandemic \mbox{%DIFAUXCMD
\cite{OrderingRapidEvolution}}\hspace{0pt}%DIFAUXCMD
. This growth helped them further cement themselves as an essential element of most restaurants' business models, and allowed them to charge commission rates of up to 30\% in exchange for access to their large customer base~\mbox{%DIFAUXCMD
\cite{DeliveryAppsGrubhub2021, thompsonHiddenCostFood2020}}\hspace{0pt}%DIFAUXCMD
. The platforms '
near-monopolistic power often forces restaurants to decide whether to pass on these higher costs and risk losing price-conscious customers or to subsume the costs themselves, reducing already-thin profit margins}\DIFdelend \DIFaddbegin \section{\DIFadd{Introduction}}
%DIF > what is the topic? Indie platforms
\DIFadd{In recent years, the negative impacts of gig work platforms---digital platforms that coordinate short-term, on-demand work---have become apparent. Scholars and journalists alike have extensively documented the precarity~\mbox{%DIFAUXCMD
\cite{ravenelleSideHustleSafety2021,ma2022brush,dziezaRevoltDeliveryWorkers2021}}\hspace{0pt}%DIFAUXCMD
, the invasive surveillance~\mbox{%DIFAUXCMD
\cite{ravenelle2019we}}\hspace{0pt}%DIFAUXCMD
, and the psychological tolls~\mbox{%DIFAUXCMD
\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a} }\hspace{0pt}%DIFAUXCMD
of mainstream gig work platforms, such as Uber, DoorDash, and Deliveroo. In response to these negative impacts, users of mainstream gig work platforms have begun to explore alternative, indie''}\footnote{\DIFadd{We borrow both the term and meanings associated with ``indie'' from music, film, games, and other industries where indie was used to identify small, independent artists supported by an enthusiastic local fanbase who operated separately from the mainstream.}} \DIFadd{platforms~\mbox{%DIFAUXCMD
\cite{}}\hspace{0pt}%DIFAUXCMD
. Indie platforms are localized, community-centric, independent businesses that rely on white-label software}\footnote{\DIFadd{White label software is software that an organization pays for to brand as its own. This software is often sold under a subscription or transaction fee. Users usually do not know the software maker.}} \DIFadd{to offer an alternative to mainstream services. These indie platforms claim to offer users more favorable terms of participation and better treatment of users. Despite the growing popularity of indie gig work platforms, there is very little HCI research exploring users’ motivations for joining and their experiences within these alternative platforms}\DIFaddend .

\DIFdelbegin \DIFdel{Mainstream platformshave been resisted by restauranteurs \mbox{%DIFAUXCMD
\cite{atkinsonMoreJobFood2021}}\hspace{0pt}%DIFAUXCMD
, couriers }\DIFdelend %DIF > what is the context? Food delivery 
\DIFaddbegin \DIFadd{In this paper, we are particularly interested in indie food delivery platforms. During the COVID-19 pandemic, use of mainstream food delivery platforms like DoorDash and GrubHub more than doubled ~\mbox{%DIFAUXCMD
\cite{OrderingRapidEvolution}}\hspace{0pt}%DIFAUXCMD
. However, with the increased use of these platforms came increased dissatisfaction with them due to high commissions rates and fees~\mbox{%DIFAUXCMD
\cite{popper2020diners}}\hspace{0pt}%DIFAUXCMD
, an untenable pace of work~}\DIFaddend \cite{dziezaRevoltDeliveryWorkers2021}, and \DIFdelbegin \DIFdel{local governments \mbox{%DIFAUXCMD
\cite{bomeyDoorDashGrubHubUber}}\hspace{0pt}%DIFAUXCMD
, among others. This discontent}\DIFdelend \DIFaddbegin \DIFadd{one-sided communication~\mbox{%DIFAUXCMD
\cite{thompsonHiddenCostFood2020, DeliveryAppsGrubhub2021,lord2022critical,ma2022brush}}\hspace{0pt}%DIFAUXCMD
. Moreover, restaurants and couriers felt that mainstream food delivery platforms did not support the human intervention needed to make a complex process like food delivery possible~\mbox{%DIFAUXCMD
\cite{figueroaEssentialUnprotectedAppbased,dziezaRevoltDeliveryWorkers2021,griswoldAreFoodDelivery2022}}\hspace{0pt}%DIFAUXCMD
. Discontent with the unfavorable terms offered by mainstream platforms}\DIFaddend , coupled with the availability of \DIFdelbegin \DIFdel{white label software}\footnote{\DIFdel{White label software is software that an organization pays for to brands as its own. This software is often sold under a subscription or transaction fee. Users usually do not know the software maker.}}%DIFAUXCMD
\addtocounter{footnote}{-1}%DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{white-label software}\DIFaddend , facilitated the rise of \DIFdelbegin \DIFdel{``indie ''}\footnote{\DIFdel{We borrow both the term and meanings associated with ``indie'' from music, film, games, and other industries where indie was used to identify small, independent artists supported by an enthusiastic local fanbase who operated separately from the mainstream.}} %DIFAUXCMD
\addtocounter{footnote}{-1}%DIFAUXCMD
\DIFdel{platforms }\DIFdelend \DIFaddbegin \DIFadd{indie food delivery platforms as an alternative. HCI has examined mainstream food platforms~\mbox{%DIFAUXCMD
\cite{li2021learning,lord2022critical,gonzalez2022designing}}\hspace{0pt}%DIFAUXCMD
, but despite their growing popularity, indie food delivery platforms remain understudied}\DIFaddend .  
\DIFdelbegin \DIFdel{Indie platformsare localized, community-centric, independent businesses that rely on white-label software to offer an alternative to mainstream services. 
}\DIFdelend 

%DIF > what did we do about the problem
While some restaurants\DIFdelbegin \DIFdel{and drivers }\DIFdelend \DIFaddbegin \DIFadd{, couriers, and consumers }\DIFaddend have turned to indie platforms as a result of their negative experience with mainstream platforms, this model has downsides too\DIFdelbegin \DIFdel{: Indie platformsare financially riskier because they }\DIFdelend \DIFaddbegin \DIFadd{. Unlike mainstream platforms, indie platforms }\DIFaddend lack the established customer base and technology capabilities to build and maintain a polished food ordering and distribution service~\cite{DeliveryAppsGrubhub2021}. \DIFdelbegin \DIFdel{Nonetheless, the stakeholders we talked to, which included restauranteurs, couriers, customers, and platform staff, have been willing to take on these risks to have access to a platform that is embedded within their local community. 
}\DIFdelend \DIFaddbegin \DIFadd{To understand why stakeholders would take on the risks associated with joining an indie platform and how they navigate the socio-technological ecosystem of an indie platform, we ask:
}\DIFaddend 

\DIFdelbegin \DIFdel{In this paper, we investigate how indie food delivery platforms operate and what motivates people to join them. We do this by interviewing }\DIFdelend \DIFaddbegin \begin{description}
\item [\DIFadd{RQ1:}] \textit{\DIFadd{What }\textbf{\DIFadd{motivates}} \DIFadd{stakeholders to join an indie platform?}} 
\item [\DIFadd{RQ2:}] \textit{\DIFadd{What are the capabilities and limitations of the socio-technical }\textbf{\DIFadd{infrastructure}} \DIFadd{that powers an indie platform?}} 
\end{description}


%DIF > what did we do?
\DIFadd{To answer our research questions, we interviewed }\DIFaddend 28 stakeholders---\textit{restauranteurs}, \textit{couriers}, \textit{customers}, and \textit{administrators}---of an indie platform called \textit{Nosh}, which operates in the northern region of a state in the Western United States\footnote{The state name has been anonymized for review}. \DIFdelbegin \DIFdel{While previous HCI research has thoroughly documented the detrimental effects that mainstream platforms have on users (e.g., financial precarity~\mbox{%DIFAUXCMD
\cite{ravenelleSideHustleSafety2021}}\hspace{0pt}%DIFAUXCMD
, invasive surveillance~\mbox{%DIFAUXCMD
\cite{ravenelle2019we}}\hspace{0pt}%DIFAUXCMD
, and pyschological tolls~\mbox{%DIFAUXCMD
\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a}}\hspace{0pt}%DIFAUXCMD
), few studies have explored how users seek out alternatives, such as indie platforms, that could offer them more favorable terms of participation. In this paper we explore }\DIFdelend \DIFaddbegin \DIFadd{We asked }\DIFaddend what motivates restaurants, customers, and couriers to seek out alternative avenues for participation in the food delivery industry through joining an indie platform \textbf{and} how this indie platform functions, fails, and is repaired. \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{We are guided by two main research questions:
}%DIFDELCMD < \begin{description}
\begin{description}%DIFAUXCMD
%DIFDELCMD < \item [%%%
\DIFdel{RQ1:}%DIFDELCMD < ] %%%
\textit{\DIFdel{What }\textbf{\DIFdel{motivates}} %DIFAUXCMD
\DIFdel{stakeholders to join an indie platform?}} %DIFAUXCMD
\DIFdel{We were interested in learning why stakeholders would take the risks associated with a newer indie platform that has a smaller customer base and less technological sophistiation.
}%DIFDELCMD < \item [%%%
\DIFdel{RQ2:}%DIFDELCMD < ] %%%
\textit{\DIFdel{What are the capabilities and limitations of the sociotechnical }\textbf{\DIFdel{infrastructure}} %DIFAUXCMD
\DIFdel{that powers an indie platform?}} %DIFAUXCMD
\DIFdel{We were interested in learning how users navigate the comparatively lower-fidelity technology used by indie platforms and if they engaged in additional work to compensate for failures in the technology. 
}
\end{description}%DIFAUXCMD
%DIFDELCMD < \end{description}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \DIFadd{We utilized thematic analysis to qualitatively code our data. 
%DIF > Using thematic analysis we identified two key themes: (1) all stakeholders highly value human intervention in the process of food delivery (2) human intervention is crucial to making platform-mediated food delivery function.
}\DIFaddend 

\DIFdelbegin \DIFdel{We provide three design recommendations for routing, customer support, and dispute resolution processes within food deliveryplatforms that promote stakeholder well-being}\DIFdelend %DIF > what was our contribution?
\DIFaddbegin \DIFadd{Drawing on a conceptual lens that brings together the platform economy and infrastructure studies from Science and Technology Studies, we find that human intervention is a natural and necessary part of platform-mediated food delivery}\DIFaddend . Specifically, \DIFdelbegin \DIFdel{our work makes two primary contributions: 
}%DIFDELCMD < \begin{enumerate}
%DIFDELCMD <     \item %%%
\DIFdel{We highlight the role of human intervention . For example, we identify the crucial role of platform administrators as intermediaries between stakeholders and the technical systems when breakdowns occur. We illustrate how human intervention is crucial to repair work  to address }\DIFdelend \DIFaddbegin \DIFadd{we found that human intervention plays such a crucial role in the process of food delivery that users are willing to leave platforms that penalize this intervention for alternative platforms that support it. Human intervention is essential to the repair work that addresses }\DIFaddend infrastructural breakdowns and integral to perceptions of agency and respect that stakeholders seek. \DIFdelbegin %DIFDELCMD < \item %%%
\DIFdel{We demonstrate the need for HCI scholarship }\DIFdelend \DIFaddbegin \DIFadd{Additionally, we find that }\texit{business models} \DIFadd{play a vital role in shaping whether socio-technical systems will support human intervention. This paper contributes an analytical framework for understanding the role of business models in shaping socio-technical systems of digital labor platforms to the HCI literature. In particular, we highlight the need }\DIFaddend to consider the role of business models \DIFaddbegin \DIFadd{as an analytical frame }\DIFaddend when making design recommendations for the platform economy. %DIF < We do this through illustrating how the design of systems is constrained by the business models and economic incentives structures in which they operate. 
\DIFdelbegin %DIFDELCMD < \end{enumerate}
%DIFDELCMD <  %%%
\DIFdelend \DIFaddbegin \DIFadd{We conclude by calling for HCI scholars seeking to improve conditions for participants in the platform economy to consider how a platform’s business model enables and constrains the intent of their design recommendations.  }\DIFaddend

==> ChiRevisionsVersion/scrap.tex <==
\section{Introduction}
%what is the topic? Indie platforms
In recent years, the negative impacts of gig work platforms---digital platforms that coordinate short-term, on-demand work---have become apparent. Scholars and journalists alike have extensively documented the precarity~\cite{ravenelleSideHustleSafety2021,ma2022brush,dziezaRevoltDeliveryWorkers2021}, the invasive surveillance~\cite{ravenelle2019we}, and the psychological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a} of mainstream gig work platforms, such as Uber, DoorDash, and Deliveroo. In response to these negative impacts, users of mainstream gig work platforms have begun to explore alternative, indie''\footnote{We borrow both the term and meanings associated with ``indie'' from music, film, games, and other industries where indie was used to identify small, independent artists supported by an enthusiastic local fanbase who operated separately from the mainstream.} platforms~\cite{}. Indie platforms are localized, community-centric, independent businesses that rely on white-label software\footnote{White label software is software that an organization pays for to brand as its own. This software is often sold under a subscription or transaction fee. Users usually do not know the software maker.} to offer an alternative to mainstream services. These indie platforms claim to offer users more favorable terms of participation and better treatment of users. Despite the growing popularity of indie gig work platforms, there is very little HCI research exploring users’ motivations for joining and their experiences within these alternative platforms.  

%what is the context? Food delivery 
In this paper, we are particularly interested in indie food delivery platforms. During the COVID-19 pandemic, use of mainstream food delivery platforms like DoorDash and GrubHub more than doubled ~\cite{OrderingRapidEvolution}. However, with the increased use of these platforms came increased dissatisfaction with them due to high commissions rates and fees~\cite{popper2020diners}, an untenable pace of work~\cite{dziezaRevoltDeliveryWorkers2021}, and one-sided communication~\cite{thompsonHiddenCostFood2020, DeliveryAppsGrubhub2021,lord2022critical,ma2022brush}. Moreover, restaurants and couriers felt that mainstream food delivery platforms did not support the human intervention needed to make a complex process like food delivery possible~\cite{figueroaEssentialUnprotectedAppbased,dziezaRevoltDeliveryWorkers2021,griswoldAreFoodDelivery2022}. Discontent with the unfavorable terms offered by mainstream platforms, coupled with the availability of white-label software, facilitated the rise of indie food delivery platforms as an alternative. HCI has examined mainstream food platforms~\cite{li2021learning,lord2022critical,gonzalez2022designing}, but despite their growing popularity, indie food delivery platforms remain understudied.    

%what did we do about the problem
While some restaurants, couriers, and consumers have turned to indie platforms as a result of their negative experience with mainstream platforms, this model has downsides too: Indie platforms are financially riskier because they lack the established customer base and technology capabilities to build and maintain a polished food ordering and distribution service~\cite{DeliveryAppsGrubhub2021}. Given the financial risk, why would stakeholders, specifically restaurants, couriers, and consumers, join an indie food delivery platform?  How do stakeholders negotiate the technological capabilities of indie platforms which are less sophisticated than mainstream options? To understand why stakeholders would take on the risks associated with joining an indie platform and how they navigate the socio-technological ecosystem of an indie platform, we ask:

\begin{description}
\item [RQ1:] \textit{What \textbf{motivates} stakeholders to join an indie platform?} 
\item [RQ2:] \textit{What are the capabilities and limitations of the socio-technical \textbf{infrastructure} that powers an indie platform?} 
\end{description}


%what did we do?
To answer our research questions, we interviewed 28 stakeholders---\textit{restauranteurs}, \textit{couriers}, \textit{customers}, and \textit{administrators}---of an indie platform called \textit{Nosh}, which operates in the northern region of a state in the Western United States\footnote{The state name has been anonymized for review}. While previous HCI research has thoroughly documented the detrimental effects that mainstream platforms have on users (e.g., financial precarity~\cite{ravenelleSideHustleSafety2021}, invasive surveillance~\cite{ravenelle2019we}, and psychological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a}), few studies have explored how alternatives, such as indie platforms, could offer users more favorable terms of participation. In this paper we explore what motivates restaurants, customers, and couriers to seek out alternative avenues for participation in the food delivery industry through joining an indie platform \textbf{and} how this indie platform functions, fails, and is repaired. 

%what was our contribution?
Drawing on a conceptual lens that brings together the platform economy and infrastructure studies from Science and Technology Studies, we find that human intervention is a natural and necessary part of platform-mediated food delivery. Specifically, we found that human intervention plays such a crucial role in the process of food delivery that users are willing to leave platforms that penalize this intervention for alternative platforms that support it. Human intervention is essential to the repair work that addresses infrastructural breakdowns and integral to perceptions of agency and respect that stakeholders seek. Additionally, we find that \texit{business models} play a vital role in shaping whether socio-technical systems will support human intervention. This paper contributes an analytical framework for understanding the role of business models in shaping socio-technical systems of digital labor platforms to the HCI literature. In particular, we highlight the need to consider the role of business models as an analytical frame when making design recommendations for the platform economy. We conclude by calling for HCI scholars seeking to improve conditions for participants in the platform economy to consider how a platform’s business model enables and constrains the intent of their design recommendations. 

%ABC platform is an indie food platform that services ABC space. 

%Within the food delivery sector of the gig economy, discontent with mainstream platforms has grown since the start of the COVID-19 pandemic. Food delivery platforms coordinate the provision of food from restaurants, directly to consumers via couriers. Mainstream food delivery platforms charge commission rates of up to 30\% in exchange for access to their large customer base~\cite{DeliveryAppsGrubhub2021, thompsonHiddenCostFood2020}. During COVID-19, restaurants were dependent on access to mainstream food delivery platforms to continue their business and thus had to decide whether to pass on these higher costs and risk losing price-conscious customers or to subsume the costs themselves, reducing already-thin profit margins. Discontent with the unfavorable terms offered by mainstream platforms, coupled with the availability of white-label software, facilitated the rise of indie food delivery platforms as an alternative. While indie platforms, beyond the sector of food delivery, have grown in prominence over recent years, there has been little HCI research examining the sociotechnical infrastructure of these alternative systems. A better understanding of how users choose to join, engage in, and are impacted by indie platforms has implications for the design of a more just and equitable platform economy.  

%estaurants relied on these platforms during the pandemic to continue their business and thus had little bargaining power to negotiate the high commission rates mainstream platforms charged~\cite{DeliveryAppsGrubhub2021, thompsonHiddenCostFood2020}. Couriers were pushed to work at extremely rapid paces which, in some cases, resulted in bodily injury~\cite{dziezaRevoltDeliveryWorkers2021}. Consumers expressed dissatisfaction with the high fees mainstream platforms charged~\cite{popper2020diners}. 

==> OLD_sections/0_Introduction.tex <==
\section{Introduction}
Mainstream food delivery platforms, such as \textit{UberEats}, \textit{DoorDash}, and \textit{Grubhub}, more than doubled in  popularity in the United States during the COVID-19 pandemic \cite{OrderingRapidEvolution}. This growth helped them further cement themselves as an essential element of most restaurants' business models, and allowed them to charge commission rates of up to 30\% in exchange for access to their large customer base~\cite{DeliveryAppsGrubhub2021, thompsonHiddenCostFood2020}. Restauranteurs \cite{atkinsonMoreJobFood2021}, couriers \cite{dziezaRevoltDeliveryWorkers2021}, and local governments \cite{bomeyDoorDashGrubHubUber} have resisted these mainstream platforms because  platforms'
near-monopolistic power often forces restaurants to decide whether to pass on these higher costs and risk losing price-conscious customers or to subsume the costs themselves, reducing already-thin profit margins. This discontent, coupled with the availability of white label software\footnote{White label software is software that an organization pays for to brands as its own. This software is often sold under a subscription or transaction fee. Users usually do not know the software maker.}, facilitated the rise of ``indie''\footnote{We borrow both the term and meanings associated with ``indie'' from music, film, games, and other industries where indie was used to identify small, independent artists supported by an enthusiastic local fanbase who operated separately from the mainstream.} platforms. 
Indie platforms are localized, community-centric, independent businesses that rely on white-label software to offer an alternative to mainstream services. 

While some restaurants and drivers have turned to indie platforms as a result of their negative experience with mainstream platforms, this model has downsides too: Indie platforms are financially riskier because they lack the established customer base and technology capabilities to build and maintain a polished food ordering and distribution service~\cite{DeliveryAppsGrubhub2021}. Nonetheless, the stakeholders we talked to, which included restauranteurs, couriers, customers, and platform staff, have been willing to take on these risks to have access to a platform that is embedded within their local community. 

In this paper, we investigate how indie food delivery platforms operate and what motivates people to join them. We do this by interviewing 28 stakeholders---\textit{restauranteurs}, \textit{couriers}, \textit{customers}, and \textit{administrators}---of an indie platform called \textit{Nosh}, which operates in the northern region of a state in the Western United States\footnote{The state name has been anonymized for review}. While previous HCI research has thoroughly documented the detrimental effects that mainstream platforms have on users (e.g., financial precarity~\cite{ravenelleSideHustleSafety2021}, invasive surveillance~\cite{ravenelle2019we}, and psychological tolls~\cite{prasslHumansServicePromise2018,rosenblatAlgorithmicLaborInformation2016a}), few studies have explored how users seek out alternatives, such as indie platforms, that could offer them more favorable terms of participation. In this paper we explore what motivates restaurants, customers, and couriers to seek out alternative avenues for participation in the food delivery industry through joining an indie platform \textbf{and} how this indie platform functions, fails, and is repaired. 


We are guided by two main research questions:
\begin{description}
\item [RQ1:] \textit{What \textbf{motivates} stakeholders to join an indie platform?} We were interested in learning why stakeholders would take the risks associated with a newer indie platform that has a smaller customer base and less technological sophistiation.
\item [RQ2:] \textit{What are the capabilities and limitations of the sociotechnical \textbf{infrastructure} that powers an indie platform?} We were interested in learning how users navigate the comparatively lower-fidelity technology used by indie platforms and if they engaged in additional work to compensate for failures in the technology. 
\end{description}

We provide three design recommendations for routing, customer support, and dispute resolution processes within food delivery platforms that promote stakeholder well-being. Specifically, our work makes two primary contributions: 
\begin{enumerate}
    \item We highlight the role of human intervention. For example, we identify the crucial role of platform administrators as intermediaries between stakeholders and the technical systems when breakdowns occur. We illustrate how human intervention is crucial to repair work  to address infrastructural breakdowns and integral to perceptions of agency and respect that stakeholders seek. 
    \item We demonstrate the need for HCI scholarship to consider the role of business models when making design recommendations for the platform economy. %We do this through illustrating how the design of systems is constrained by the business models and economic incentives structures in which they operate. 
\end{enumerate}



==> OLD_sections/1_Literature_Review.tex <==
\section{Literature Review}
Researchers and journalists have identified structural flaws in food delivery and ride hailing platforms, ranging from exploitation~\cite{van2017platform,ravenelle2019we,moore2021augmented} to algorithmic control~\cite{woodcock2020algorithmic} to discrimination~\cite{beerepoot,adermon2022gig}. Despite these concerns, these platforms continue to grow and entrench themselves in communities around the world. Food delivery platforms create a two-sided market: they match supply of food from restaurants to demand for food from consumers and coordinate the delivery of food through a fleet of couriers~\cite{parwezCOVID19PandemicWork2022}. During the lockdown phase of the COVID-19 pandemic, food delivery platforms provided a means for local restaurants to continue their business despite shutting down brick-and-mortar locations. Since then, food delivery platforms have cemented themselves as a permanent fixture in the restaurant industry generating record sales and volume ~\cite{pewresearch, mckinsey}. 

Despite the usefulness of these food delivery platforms, they present challenges to both the restauranteurs and the couriers who rely upon them. Restaurants experience financial precarity as a result of high commission rates and drivers are subject to intrusive surveillance, both of which were exacerbated during the pandemic ~\cite{thorbecke2020impact}. While previous research has documented the harms caused by mainstream food delivery platforms, little work has been done to examine \textbf{how workers and communities have sought to address these harms by supporting local, independent platforms}. In this literature review, we explore the role that food delivery platforms play in supporting the restaurant industry, problems endemic to food delivery platforms, and emergent solutions to those problems. We draw upon infrastructure theory to add context to our findings of how these platforms function, break down, and are repaired.  

\subsection{What are Food Delivery Platforms?}
GrubHub, founded in 2004, was one of the first food delivery platforms in the United States~\cite{OnlineFoodOrdering2022}. Food delivery platforms coordinate the request, preparation, and delivery of food by connecting restaurants, drivers, and customers through their applications. In other words, they are a platform aggregator: they aggregate supply and demand~\cite{kenneyRisePlatformEconomy2016,zwickWelcomeGigEconomy2018}. These platforms have become a fixture in the restaurant industry, with sales and volume skyrocketing for the largest delivery platforms in recent years~\cite{pewresearch,mckinsey}. %Food delivery platforms such as DoorDash, UberEats, and GrubHub  enable consumers to obtain food, drivers to find work, and restaurants to sell their goods. Users rely on networked online interfaces to conduct an exchange of goods and services. 
While food delivery platforms were popular before 2020, they became an integral part of restaurants' revenue streams after consumers became accustomed to ordering take-out online during the lockdown phase of COVID-19 ~\cite{mckinsey,pewresearch,smithPeopleHaveEat}. These platforms can be thought of as infrastructure---they are the foundation that underpins the large-scale systems of the food delivery industry~\cite{hanseth2010design}. Like all infrastructures, food delivery platforms are sociotechnical systems that are imbued with the values of their designers: They shape and are shaped by social practices~\cite{star1996steps,friedmanValueSensitiveDesign2013a}. 

\subsubsection{Value Misalignment Between Designers and Users of Food Delivery Platforms}
Food delivery platforms are designed by software engineers and funded by venture capitalists and are thus imbued with their values~\cite{zuboff2015big}. Food delivery platforms, like DoorDash, are designed by software engineering teams who prioritize high-speed, low-cost delivery by assigning orders to gig workers available nearby regardless of gig workers' preferences~\cite{weinsteinUsingMLOptimization2021}. Couriers are constantly driven to deliver more, faster: the expected speed of their next delivery is determined by the speed they were able to achieve with past deliveries ~\cite{dziezaRevoltDeliveryWorkers2021}. In some cases, this has led to couriers getting into fatal traffic accidents as they navigate roads at high speeds on electric power bicycles capable of reaching upwards of 20 miles an hour~\cite{figueroaEssentialUnprotectedAppbased}. Platform interfaces serve as artifacts that reveal the underlying values of their designers; there are few, if any, features on the couriers' mobile application interface that allow for them to articulate their preferences to the platform~\cite{liBottomUp}. When values of designers fail to align with values of users, problems arise which can result in users being harmed ~\cite{Semaan2019,friedmanValueSensitiveDesign2013a}. 

\subsection{What are the Problems with Food Delivery Platforms?}
During the COVID-19 pandemic, demand for the largest food delivery services like Grubhub and UberEats grew as delivery became an integral part of restaurants' business models~\cite{smithPeopleHaveEat}. However, researchers have identified several harms specific to food delivery platforms, including exacerbating workers’ and restaurants’ economic insecurity and pervasive algorithmic control~\cite{parwezCOVID19PandemicWork2022,frankeConnectingEdgeCycles2021,huangRidersStormAmplified2022,woodcock2020algorithmic}. Gig platform scholars assert that these harms are endemic to gig work which functions on the basis of predatory inclusion---the inclusion of marginalized populations into seemingly democratizing arrangements on extractive terms~\cite{mcmillancottomWherePlatformCapitalism2020}. This model of predatory inclusion coupled with opaque algorithmic management creates precarious working conditions~\cite{mcmillancottomWherePlatformCapitalism2020, woodcockGigEconomyCritical2020, van2017platform, popanEmbodiedPrecariatDigital2021, ravenelleSideHustleSafety2021}. While gig platforms market themselves as a novel way for workers to be their own boss, they often fail to disclose the emotional, physical, and financial costs workers incur by doing so. 

\subsubsection{Problems that couriers experience in the food delivery economy}
Unlike traditional food delivery services (\textit{e.g.}, Pizza Hut phone order delivery), platform delivery services heavily incorporate algorithms into their operations to not only convey logistical information to couriers about their tasks, but also to track their performance~\cite{goods2019your}. This omnipresent surveillance allows companies like UberEats to track the rate at which food couriers accepted or denied delivery requests as well as their customer ratings to compile a performance rating of each worker~\cite{veenPlatformCapitalAppetiteControl2020}. Constant surveillance and uncertainty about how they are being managed causes emotional and psychological stress for couriers~\cite{caloTAKINGECONOMYUBER2017,woodcock2020algorithmic,rosenblatAlgorithmicLaborInformation2016a}. Opacity around algorithmically determined payments creates additional precarity for workers~\cite{goods2019your,calacciBargainingBlackBox2022}. 

Couriers participating in the platform food delivery industry take on financial risk as part of their work. For example, shifting consumer demands, poor weather conditions, and irregular unpaid wait times for restaurant food preparations are common occurrences that can bring couriers’ earnings to below minimum wage~\cite{goods2019your}. Opaque algorithmic management also causes wage insecurity. Platforms will often update their interfaces and algorithms without warning couriers beforehand about how changes will impact their earnings~\cite{calacciBargainingBlackBox2022}. For instance, when Postmates updated their interface to include customizable tipping amounts, couriers feared earning less because consumers may not always be aware that they should tip their delivery driver~\cite{shapiro2018between}. The economic toll of using delivery platforms also extends to restaurants.

\subsubsection{Problems that restaurants experience in the food delivery economy}
After indoor dining was restricted during the pandemic, many restaurants signed up for food delivery services as an alternative revenue stream. However, the mainstream platforms’ high commission rates cut into the earnings of already struggling local businesses~\cite{saxenaDeliveryAppsAre2019}. Restaurants were hesitant to raise prices because doing so may drive away price-sensitive consumers~\cite{DeliveryAppsGrubhub2021, thompsonHiddenCostFood2020}. This put participating restaurants in a situation where they had to take a hit on their profit margins to avoid potentially driving away consumers. These negative impacts have driven some restaurants and couriers to explore alternative options for participating in the food delivery platform economy.  

\begin{figure}[h]
\caption{Software and Services in the Unbundling Economy as described by the founder of a tech company in the food delivery industry}
\label{fig:unbundling}
\includegraphics[width=5cm,height=10cm]{images/unbundling.png}
\end{figure}

\subsection{The Emergence of ``Indie'' Platforms as a Response to Infrastructural Breakdowns}
Over the past few years, small, localized, and community-centric alternative gig platforms have surfaced~\cite{atkinsonMoreJobFood2021}. These indie platforms rose to fill the gaps left by mainstream services. Namely, they claim to offer restaurants, drivers, and customers a service that charges lower commissions, cares about the stakeholders involved, and is on the side of the community ~\cite{atkinsonMoreJobFood2021, schneiderExitCommunityStrategies2020,WhyAreRestaurants2021,DeliveryCoopsProvide}. However, there are also drawbacks to indie platforms: They usually do not have as large of a customer base or as sophisticated of technology as mainstream platforms~\cite{DeliveryAppsGrubhub2021}. Thus far, academic research into these new models has been limited, often only focusing on one subset that function as co-operatives~\cite{bundersFeasibilityPlatformCooperatives2022a,scholz2016and,schor2021after}. Our research seeks to expand the conversation around these alternative designs by applying learnings from the CSCW and HCI infrastructure literature to understand why these platforms emerge, how they function, and their limitations and advantages. 

\subsubsection{Indie platforms rely on the ``unbundling'' economy for technical infrastructure}
Indie platforms draw upon the “unbundling” economy to build their own services from the bottom up. This economy provides software and services for individual elements of the food delivery process: point of sales systems, order aggregation services, and last mile delivery fleets (see Figure~\ref{fig:unbundling} below)~\cite{wangCommissionfreeOnlineOrders2020,wangArmingRebelsFood2021}. But these piecemeal systems that attempt to integrate disparate pieces of software and services often breakdown due to incompatibility and difficulty of use. However, prior literature in HCI provides guidance on how users engage in \textit{bricolage} to make piecemeal systems work when mainstream offerings breakdown~\cite{vallgaarda2015interaction,jackson2014RethinkingRepair}. Through the process of bricolage, users extend and repair existing systems through human labor to build an infrastructure that better meets their needs~\cite{vallgaarda2015interaction,jackson2014RethinkingRepair}.


\subsubsection{Human labor plays a key role in supporting indie platforms}
Indie platforms build their services by integrating multiple disparate pieces of software into one technology stack, usually without having a fully staffed software engineer team on hand~\cite{DeliveryCoopsProvide}. In this low resource environment, technological breakdowns are inevitable~\cite{DeliveryCoopsProvide}. Despite this, indie platforms have continued to survive and grow in prominence~\cite{atkinsonMoreJobFood2021,WhyAreRestaurants2021}. Journalistic accounts report indie platform owners pointing to their small-scale, localized nature and human-centric design as a crucial element of their success~\cite{DeliveryCoopsProvide,holtzCanCoOpsFix2022,atkinsonMoreJobFood2021}. However, little empirical work has been done to understand how indie platforms manage to overcome technological short-comings. We draw upon the concept of bricolage to better understand how users of indie platforms overcome failures in their technology stack to create a cohesive food delivery service all within a low resource environment.   

This paper draws upon infrastructure literature and applies it to the context of the food delivery platform economy to develop a better understanding of why users join indie platforms and how these platforms continue to survive despite their lower levels of technological sophistication. We identify how stakeholders surface the values embedded in the infrastructures of mainstream platforms, which become evident during breakdowns, and how value mis-alignment motivates them to join indie platforms. We examine how top-down construction of infrastructures fails to account for local contexts and highlight the importance of designing to incentivize human intervention in the face of breakdowns. This work expands on design literature in the platform economy by providing guidance for how HCI scholars can develop systems that align with local communities' needs and mesh with the economic incentives of the business model at hand. 




==> OLD_sections/2_Methods.tex <==
\section{Background on mainstream and indie food delivery platforms}
In this paper, we differentiate between mainstream and indie food delivery platforms. Here we describe the characteristics of each to highlight the key differences between the two models. We then provide additional detail about the empirical setting where we conducted the research.

\subsection{Mainstream food delivery platforms}
% Here's what GrubHub, DoorDash, Uber Eats do operationally and how they describe their business strategy
Mainstream platforms have business models that are predicated on \textit{market capture}, or the monopolization of a given market. Mainstream platforms have access to large pools of venture capital funding that enables them to operate at a loss ~\cite{DoorDashSharesSink, GrubHubOrdersKeep}. Thus, mainstream platforms are not solely reliant on commissions from orders for profit; rather, they simply need to demonstrate growth or the potential for growth to continue to receive funding. This means that mainstream platforms' success is not strictly predicated on the success of the restaurants and drivers participating in them. This business strategy informs both the technical design of their systems and therefore shapes the nature of interactions that stakeholders have with each other and the platform. 

\begin{figure}[t]
\caption{Difference in financial flows between mainstream platforms and Nosh}
\label{fig:financialflows}
\includegraphics[width=\textwidth]{images/fig1.jpg}
\end{figure}

\subsection{Nosh: an indie food delivery platform}
\subsubsection{Organizational and financial structure} 
In contrast to mainstream platforms, Nosh's business model is rooted in the local communities in which it operates. 
Nosh operates as a "hub and spoke" business model. This means that the parent company, Nosh, provides the technology, brand, and initial seed capital for the smaller, local Nosh "hubs". When Nosh comes to a new community, they establish a local Nosh delivery service (\textit{e.g.}, think of how franchises like McDonald's operate). Each local Nosh delivery service is funded by a coalition of local restaurants that invest seed money into their hub. These "investor" restaurants get voting power over operational decisions in their locale. The parent company helps each local get started by hiring dispatchers and drivers from the community. The parent company also provides the application and technical infrastructure needed to run the application. In return, each local Nosh hub shares a percentage of its profit with the parent company. Once dispatchers and drivers have been hired, the investor restaurants begin delivering through the Nosh application. Because Nosh does not have access to venture capital, the platform relies on commissions from their orders and investment from local restaurants. In other words, Nosh's success as a business model is predicated on its stakeholders' success. In Figure~\ref{fig:financialflows} we illustrate how the economic structure of Nosh differs from that of mainstream platforms, particularly how monetary incentives shape relationships between stakeholders and the platform.

Mainstream models rely upon investments from venture capitalists and individual shareholders to finance their operations. This makes mainstream platforms less dependent upon patronage from customers and restaurants as they have access to alternative cash flows. Nosh's model differs from mainstream platforms in terms of economic incentives because the primary investors in the platform are the restaurants themselves. As investor/owners of each local Nosh hub, restaurants contribute to operational decisions and are the platform's primary source of cash flow. The platform's viability is thus tied to stakeholders’ fiscal well-being. Through this model, Nosh is \textbf{beholden} to its stakeholders in ways that mainstream platforms are not. This impacts how the Nosh platform operates, especially in times of breakdown.

%\subsubsection{Nosh the Platform} 
\subsubsection{Nosh relies on a patchwork of technical systems to function}
Food delivery relies upon multiple parties and disparate pieces of software being able to communicate with each other. Nosh uses a suite of proprietary and software-as-a-service technologies to run their business that include:
\begin{itemize}
\item \textit{DataDreamers} for delivery logistics. Although Nosh reported moving to another company's software.
\item \textit{WhenIWork} for courier scheduling and to chat with couriers.  
\item \textit{Zendesk} for customer support.
\item \textit{Slack} for internal communications between dispatchers. 
\item \textit{Google Suite} for generating earning reports for restaurants.
\end{itemize}

While these pieces of software are more affordable than a vertical integration model, breakdowns and confusion often occur frustrating stakeholders. ()

\subsection{Empirical Setting} %take out methods & put in background section
We conducted an interview study with four stakeholder groups participating in Nosh: restauranteurs, couriers, platform administrators, and customers, to understand what motivates people to join an indie platform. At the time of our interviews, Nosh was operating in two regions. One region encompassed multiple mid-sized cities. The other contained only one major metropolitan area. We have anonymized the region and city names for peer review. We conducted interviews from August to December of 2021. The region is also served by mainstream platforms such as GrubHub, UberEats, DoorDash, and Postmates. %Below we detail our approach for understanding why people joined Nosh and the work they performed within the platform to sustain it. 

\section{Methods}
%Samantha to describe recruitment method
Our study aims to better understand the workings of an indie food delivery operation. We conducted 28 interviews with four stakeholder groups participating in Nosh: restaurants, couriers, customers, and platform administrators. Before conducting the interviews, our protocol and procedures were certified by our institutional review boards. The interview protocols differed for each stakeholder group but all sought to surface why the subject chose to use Nosh and how they participated in Nosh. We include the interview protocols for each stakeholder group in the appendix. Below we provide more detail on our positionality as researchers, the participants, interview protocol, data analysis, and limitations. 

%COMMENTING OUT WHILE WE WRITE IT
%\subsection{Positionality Statement}
%Before we continue, we think it would be helpful present the positionality of the (five?) authors of this paper, as it may effect how we view the data. 

%Nikoo: 
%- (Nationality, gender, ethnicity: U.S. born woman of Middle-Eastern 5descent)
%- Age and Education: undergraduate student at an Ivy League institution in her early 20's

% Andrés: Mexican-born and raised, now US-based, male, 42, Ivy league professor, former tech worker <-- i feel like this might deanonymize us easily :)
% Andrés: 
    % no experience a courier or restauranteur 
    % customer: have used several mainstream FDPs, including Uber Eats, Doordash, Postmates. Have not used an indie platform
    % admin: former tech worker, and  platform administrator (but not FDP)

\subsection{Participant Recruitment}
%Our participant pool comprises individuals from four stakeholder groups within Nosh: delivery drivers, restaurateurs, customers, and platform dispatchers or administrators of Nosh. In total, 28 participants across these four stakeholder groups sat for interviews. We selected these stakeholder groups because they played key roles in the food delivery industry. Additional detail about stakeholders is included  in Table~\ref{table:stakeholderlist}.


%\subsubsection{Recruitment Strategy}
%We recruited participants through Nosh via an email list. 
We contacted the founder of Nosh who helped us distribute a call for participation to an email list that was sent out to all restaurants, drivers, platform administrators, and customers that used Nosh. %Once we established contact with participants, we scheduled them for one-hour interviews conducted via Zoom. We read a consent script to participants and received verbal consent to have their interviews recorded and used for this study. We transcribed and removed personally identifiable information from the interviews.  We compensated participants for their time with a \$20 Amazon gift card. 

%\subsubsection{Participant Summary}
In total, we conducted 28 interviews across four stakeholder groups: restauranteurs (n=7), couriers (n=6), customers (n=10), and platform administrators (n=5). %We had seven restauranteurs, six drivers, ten customers, and five platform administrators.
The majority of restauranteurs worked for or owned fast-casual businesses (R1, R2, R4, R5, R6, R7). We spoke to platform administrators who did back-end work (P2), customer-facing work (P1, P5), and managerial work (P3, P4). The drivers we spoke to were evenly split among part-time (D1, D2, D4) and full-time drivers (D3, D5, D6). We  break down our participant demographics in Table~\ref{table:stakeholderlist}.
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}\\

\begin{table}[]
\caption{List of participants broken down by the four stakeholder categories: restauranteurs, platform administrators, couriers, and customers}
\label{table:stakeholderlist}
\begin{tabular}{ll}
\toprule
\textbf{Participant} & \textbf{Occupation Description}    \\
\midrule
\multicolumn{2}{c}{\textit{Restauranteurs}} \\
\hline
R1                   & COO - Chicken Wing Restaurant\\

R2                   & Owner - Tea Shop                \\

R3                   & Owner - Seafood Fine Dining     \\

R4                   & Owner - Wood Fired Pizza        \\

R5                   & Owner - Fast-Casual Take Out    \\

R6                   & Owner - Chicken Wing Restaurant \\

R7                   & Owner - Burger Restaurant       \\
\hline
\multicolumn{2}{c}{\textit{Platform Administrators}}                       \\
\hline

P1                   & Dispatcher                                    \\

P2                   & Data Analyst                                  \\

P3                   & Co-Director of Operations                     \\

P4                   & Co-Director of Operations                     \\

P5                   & Dispatcher                                    \\
\hline
\multicolumn{2}{c}{\textit{Couriers}}                       \\
\hline

D1                   & Driver - Part Time                                    \\

D2                   & Driver - Part Time                                  \\

D3                   & Driver - Full Time                     \\

D4                   & Driver - Part Time                     \\

D5                   & Driver - Full Time                                    \\

D6                   & Driver - Full Time                                    \\
\hline
\multicolumn{2}{c}{\textit{Customers}}                       \\
\hline

C1                   & Health Care Professional                                    \\

C2                   & Office Worker                                  \\

C3                   & Office Worker                     \\

C4                   & Homemaker                     \\

C5                   & Office Worker                                    \\

C6                   & Office Worker                                    \\

C7                   & Office Worker                                    \\

C8                   & Undisclosed                                  \\

C9                   & Office Worker                     \\

C10                   & Undisclosed                    \\
\bottomrule

\end{tabular}
\end{table}

\subsection{Interview Protocol}
The first, second, and third authors conducted one-hour interviews via Zoom. We informed participants of their right to skip  questions or stop the process anytime. We obtained their verbal consent for recording the interview and gave them the option to sign up for a follow-up survey for future research. We transcribed the interviews and anonymized the transcripts. We compensated participants for their time with a \$20 Amazon gift card. 


Our interviews followed semi-structured scripts based on the participant's group affiliation\footnote{see the Appendix for interview protocols}. These scripts focused on surfacing key motivations for participating in Nosh and understanding how participants interacted with the platform. For example, depending on their role, we discussed the pros and cons of delivering for Nosh (drivers), collaborating with Nosh (restaurateurs), ordering from Nosh (customers), and working for Nosh (dispatchers). The first, second, and third authors manually corrected the automatically-generated transcriptions provided by Zoom by cross-referencing them with the audio recordings. %We then moved on to analyze the corrected transcripts.
%%need to include transition sentence 
\subsection{Data Analysis}
After transcribing each interview, the first, second, and third authors coded the contents using thematic analysis. To standardize the analysis between three people, we conducted preliminary coding where the researchers independently analyzed the same batch of interviews. We then convened afterward to compare and discuss our findings. We also conducted card-sorting exercises to arrive at the final codes. Later, we compiled repeating themes in a centralized codebook, which we then used to code the remainder of the interviews.

%Our work reveals two major sets of findings. In Section~\ref{sec:motivations}, we present two primary reasons why restaurants, couriers, and customers were motivated to join Nosh: they achieved a greater level of agency and a greater degree of financial security when participating in Nosh compared to mainstream platforms. In the Table 2~\ref{tab:Table 2} we break down the motivations of restaurants, couriers, and customers for using Nosh. Then in Section~\ref{sec:patchwork}, we present how all stakeholders and technology functioned in tandem to make Nosh work. In Table 3 we break down the pieces of technology each stakeholder group interacted with and the type of repair work they engaged in when using the Nosh platform. 




==> OLD_sections/3_Findings.tex <==


\section{Results}

We frame our findings around two key themes: 
\begin{enumerate}
    \item Users' motivations for participating in indie platforms and 
    \item How users and technology come together to make indie platforms work
\end{enumerate}

We first identify the essential roles of agency and financial security in motivating restaurants, couriers, and customers to join Nosh. We highlight how the presence of human intervention in the face of breakdowns is a differentiating factor between mainstream platforms and Nosh. Then we examine how users interact with Nosh's technical systems, paying special attention to the key role of platform administrators in serving as buffers between users and the technical systems.

\subsection{Why do stakeholders join an indie platform? More agency and financial security}\label{sec:motivations}

\begin{table}[]
\caption{Restaurant, Courier, and Customer Motivations for Participating in Nosh}
\label{table:motivations}
\begin{tabular}{ll}
\toprule
\textbf{Stakeholder Group} & \textbf{Motivations for Participation}    \\
\midrule
Restaurants                & \makecell{Lower commissions, Increased operational oversight, \\Dislike of mainstream platforms} \\\\

Couriers                   & \makecell{Floor pay, Guaranteed shifts, Increased autonomy}                                    \\\\

Customers                  & \makecell{Support local, Dislike of mainstream platforms, \\Better customer service} \\ \bottomrule
\end{tabular}
\end{table}

Restaurateurs and couriers joined the indie platform because of a desire for more agency and financial security. Similarly, customers joined because they perceived the indie platform as more ethical, precisely for the same reasons: more agency and financial security for restaurateurs and couriers. See Table~\ref{table:motivations} for a synthesis of these motivations.


%\subsubsection{Stakeholders Preserve A Greater Degree of Agency in Nosh Compared to Mainstream Platforms}
\subsubsection{More agency motivates stakeholders to join}
When participating in mainstream platforms, stakeholders (couriers, restauranteurs, and customers) noted that they are required to fit themselves into the logics of the platforms with little room for negotiation. Processes for participation, operation, and dispute resolution were predetermined by mainstream platforms. This limited stakeholders' ability to exert meaningful control over their participation, advocate for themselves, and come to resolutions they perceived to be fair. In contrast, stakeholders felt that their agency was preserved when using Nosh, which motivated their adoption of the service. Stakeholders’ perception of agency was closely aligned with the presence of human intervention: the ability to interact, reason, and negotiate with a human representative from Nosh gave them a sense of agency that they lacked when participating in mainstream platforms. We demonstrate how agency was defined and identified by restaurants, couriers, and customers below.


\begin{itemize}
\item \textbf{Restauranteurs' agency through transparency and operational input.}
Negative experiences with mainstream platforms, such as encounters with dark patterns, drove restauranteurs to seek out alternatives. For example, restauranteurs pointed to non-consensual listings of their business on mainstream platforms as a violation of their agency: 
\begin{quote}\textit{
     ``Grubhub will find our menu put it online without telling us...and then so you'll get a phone call from somebody and then they'll place an online order to pick up. And when they pick up it's it's a Grubhub driver. What they do later is contact you and say hey look you had X amount of deliveries [through] Grubhub, and you know, do you want to sign up for Grubhub?'' (R5)
}\end{quote}

In contrast, because each local hub of Nosh operates as a co-operative run by local restauranteurs, restauranteurs had a direct role in influencing business operations: 
\begin{quote}\textit{
    ``there's a lot of people, giving input and their thoughts, [Nosh] is truly a cooperative where you know matters of importance are voted on and discussed openly. It's very transparent operation from Nosh, the other services, you know no transparency [is] there you know it's just a plug and play... I don't have any say on what happens once I sign up.'' (R6)
}\end{quote}

Having a say over and transparency into operations meant that, in Nosh, restaurants were partners with agency to negotiate their participation. Restauranteurs felt that their ability to negotiate terms of participation with Nosh led to a more equitable relationship than the one they had with mainstream platforms. 

\item \textbf{Courier's agency through respect for discretionary decisions.}
In mainstream platforms, couriers get their work allocated through an algorithmic system. Also, mainstream platforms tend to punish couriers for deviating from the prescribed instructions even if they had good reason to do so. \begin{quote}\textit{
     ``One thing I also like with Nosh versus DoorDash – Nosh does not track my movements and my location in a way that... If I'm not heading to the restaurant and if I'm biding my own time, it's not going to tell me to turn around or else I'll lose the order. That's something that I remember with DoorDash, that even if there was a large wait time and I didn't head in the direction of the restaurant first, the app would track that and say, 'Are you heading to the restaurant? Looks like you're not heading in the direction of the  restaurant, if you're not going to be heading there in the next couple minutes, we're going to reassign your order to somebody else'.'' (D2)
}\end{quote}
When couriers worked for Nosh, they were able to exercise their best judgement, even if it went against what the dispatching algorithm prescribed, and not be punished for it. The ability to exert control over their work without fear of retribution meant that couriers had a higher degree of agency when working with Nosh.  Several of them pointed out that they felt comfortable deviating from the instructions of the dispatching algorithm because they knew there was always a human dispatcher supervising the system. 
\begin{quote}\textit{
    ``overall, our system is much more fair than other services that I worked for because you have that human aspect of problem solving.'' (D5)
}\end{quote}

Platform administrators could be spoken to and rationalized with, unlike an algorithm. 

\item \textbf{Customers agency through an ability to get a human for support.} Customers discussed their dispute resolution experience with mainstream platforms, emphasizing the one-sided nature of the process with mainstream platforms. \begin{quote}\textit{''One of the times I ordered formula, [Postmates]...delivered the wrong kind. So I reached out and I they told me I could return the item. I mean, I get in my car, go return the item, and get what I wanted, and then they gave me a credit. Which I was, like all right fine whatever like that's very irritating that like you should really just send somebody out with the correct thing. And then they refunded my account, but it was a credit on Postmates and then, when I went to use it had been...a while my credit expired...I ended up...not getting that money at all.'' (C2)
 }\end{quote}Here C2 details the frustration that many customers felt with mainstream platforms: they weren't given an option to negotiate what kind of resolution they wanted. In contrast, with Nosh, customers were able to contact a real, local person, for help. Customers feel like they had agency over the situation because they were able to speak with a human and have a say in resolving problems. Customers pointed to the fact that platform administrators always asked them ``what can we do to make this right'' as evidence of their ability to negotiate the outcome. 
\end{itemize}
In sum, stakeholders' sense of agency was intimately linked to the presence of human intervention during the course of food delivery. Platform administrators acted as intermediaries between stakeholders and the technical infrastructure of Nosh. Stakeholders could interact and negotiate with platform administrators in a way that they could not with the automated interfaces of mainstream platforms. The ability to engage in two-sided interactions was critical to stakeholders’ agency.

\subsubsection{Greater financial security motivates stakeholders to join}

Mainstream platforms dictate the financial costs and benefits of participation. Stakeholders reported that this one-sided negotiation infringed on their ability to achieve financial security in the already low-margin business. With Nosh, restauranteurs reported having lower commission rates and peace of mind knowing that the platform's financial success was tied to theirs. Couriers reported that they had transparency into the fees Nosh extracted from each order, plus the satisfaction of guaranteed floor-pay\footnote{Floor pay is a minimum payment per shift regardless of the number of orders based on the local minimum wage. If couriers did not meet local hourly minimum wages while working, and were not "gaming" the system by simply rejecting orders assigned to them, their wage was supplemented by Nosh so that it was equal to the local hourly minimum wage.}, reducing the precarity endemic to independent contractor jobs. Below, we demonstrate how restaurants and couriers were able to attain higher degrees of financial security with Nosh and how customers perceived this as an indicator that Nosh was a more ethical options for food delivery. 


\begin{itemize}

\item \textbf{Restauranteurs' financial security through lower fees and co-ownership.} Restauranteurs reported being too small to negotiate the, on average, 30\% commission that mainstream platforms charged them. Thus, restauranteurs with already thin profit margins had to raise menu prices to make up for the high commissions charged by mainstream platforms, which they worried would affect their customer base: 
\begin{quote}\textit{
    ``Commission rates are important... and we do raise our prices significantly on delivery platforms to recover a portion of that commission'' (R7). 
}\end{quote}
Nosh offered a more financially sound alternative because they charged a 15-20\% commission rate, according to conversations the research team had with Nosh administrators.  

Additionally, since each Nosh hub is owned and operated by local restauranteurs, the financial success of the platform is tied to that of the restaurant owners. Thus, restauranteurs had the added security knowing that,  \textit{``...it's not just Nosh's financial success. They're also looking out for each individual  restauranteurs success, because \textit{\textbf{[Nosh is]}} those individual restauranteurs``} (R2, emphasis added).

\item \textbf{Couriers' financial security through floor pay and guaranteed shifts.} 
Couriers reported that, in mainstream platforms, the work was not as flexible as platforms claim because they cannot actually \textit{get} work when they log onto the platform. 
\begin{quote}\textit{
     ``One of the things with the scheduling and the shifts that they [Nosh] offer is there as a preventative measure to not over-saturate the market with drivers because when you sign on for like DoorDash or like Grubhub, or any of those, there could be hundreds and hundreds of drivers... with Nosh, you know, you can kind of be the big fish in a small pond. If you work hard, and you're efficient and fast, you can make all the money. So there's less saturation I guess is probably the main thing I like about it.'' (D3)
}\end{quote}
This courier explicitly calls out Nosh's scheduling system as a key element in promoting financial security. Couriers we interviewed characterized Nosh's hybrid scheduling-open shift system as being \textit{both} more flexible and secure than the "log on and drive" model of mainstream platforms. Nosh's hybrid scheduling-open shift system allows couriers to submit their preferred schedules a week in advance and then assigns couriers shifts based on their availability and preferences. For example, a courier who wanted to work on Tuesday evenings might be assigned the Tuesday dinner rush shift. Couriers could drop shifts, without penalty, after they were assigned by notifying Nosh dispatchers and these shifts would become available in the open shifts tab of the courier's mobile application. This scheduling model combined with Nosh's guaranteed floor-pay provided couriers with a sense of financial security that motivated their participation in Nosh. 
\end{itemize}

Increased agency and financial security made stakeholders feel respected by Nosh: the platform centered food delivery and the stakeholders upholding it. As one restaurant put it:\textit{ “DoorDash and Grubhub are fantastic technology companies that deliver food. Nosh is a fantastic food delivery company that has some technology.”} (R6). This restauranteur  highlights the primary trade-off that stakeholders who choose to participate in Nosh make: access to top-of-the-line technology to facilitate food delivery versus access to more human-centred services that promote agency and respect. Nosh's respect for agency and financial security of restaurants and couriers motivated customers to join as they sought more ethical alternatives for food delivery platforms. 

\subsubsection{Perception of ethicality motivate customers}
 Customers felt that the way Nosh handled the financial aspect of food delivery was more ethical than mainstream platforms.
 Nosh gave couriers and restauranteurs a degree of financial security that they were not able to achieve when working for mainstream platforms. For customers, this motivated them to patronize Nosh because they felt this made the platform a more ethical alternative for food delivery.

Customers articulated feeling strongly about how both restauranteurs and couriers were treated financially by food delivery companies: 
\begin{quote}\textit{
    ``I mean I read the news article, you know, in the Times about how Grubhub and DoorDash are just ripping off restaurants like it's not okay take advantage of people during a pandemic, so I prefer not to use companies that do that.'' (C3)
}\end{quote}

The majority of customers we interviewed described being avid supporters of local restaurants before the COVID-19 pandemic. When the pandemic began, customers sought out ways to patronize local restaurants in an effort to support their community: \textit{``I love that [Nosh] is local so that's my biggest thing...it has a lot of like my favorite local restauranteurs''} (C4). 

Customers noted that even though other food delivery platforms, like DoorDash and UberEats, also had some local restaurants listed, they preferred ordering from Nosh because it was \textit{``just a little bit more ethical''} (C1). For customers, ethical meant that the platform treated both couriers and restauranteurs with respect by not engaging in exploitative financial practices. %such as taking cuts of couriers tips or charging exorbitant commission fees for restauranteurs. While customers did not have first-hand knowledge about tip distribution or restaurant commissions, they put a lot of stock in popular narratives about mainstream platforms' mistreatment of couriers and restauranteurs. Customers perceived Nosh as respecting restaurateurs and couriers in the way Nosh handled the financial dimensions of food delivery.

%Restaurateurs, couriers, and customers participated in a relatively untested model of indie food delivery because doing so enabled them to exert agency in a way they were previously unable to with mainstream food delivery platforms. Restaurateurs and couriers benefited from a greater degree of financial security, which customers viewed favorably as an indicator that Nosh was a more ethical option for food delivery. A key factor to supporting agency among stakeholders and providing financial security was the presence of human intervention in the process of food delivery: platform administrators negotiated operations with restaurateurs and engaged in the extensive labor necessary to schedule shifts for couriers. How then does Nosh’s infrastructure differ from that of mainstream platforms \textbf{and} how do these difference lead to fundamentally different interactions that stakeholders have with the platform? 

\subsection{What Makes Nosh Work?: A patchwork of technical systems held together by human intervention}\label{sec:patchwork}

Nosh is a patchwork of technical systems held together by human intervention. Nosh relies upon multiple disparate pieces of software to operate. Breakdowns in their patchwork technology stack are commonplace and must be repaired through human intervention. This human intervention is what compels stakeholders to participate in Nosh. However, human intervention requires deep local knowledge, takes time, and requires money. In this section, we outline the contours of Nosh’s technology stack and identify how stakeholders engage in repair work to address gaps and breakdowns, paying special attention to the role of platform administrators. We provide a summary of what technologies each stakeholder interacts with and how they engage in repair work in Table~\ref{table:repairwork}.

\subsubsection{Stakeholders struggle with Nosh's patchwork of technical systems}
Restauranteurs we interviewed complained that Nosh's ordering system was clunky and required them to operate not only a separate order aggregation system, but also a tablet dedicated solely to Nosh orders. Mainstream food delivery platforms can integrate directly with most restaurants' point-of-sale software and order aggregation systems, reducing friction in the system. Couriers complained that as a result of the complicated order aggregation system, restaurants often forgot important steps such as starting a countdown timer that couriers relied on to estimate when the order would be ready for pickup: 
\begin{quote}\textit{
    ``it's hard you know because everybody wants to point fingers so it's hard...to say like if they're actually just like \textbf{not able to understand how the app works} or they just didn't start the order because they you know were lazy or busy or whatever. And they're just like oh like, it wasn't actually my fault, like \textbf{the App is bad}.'' (D3, emphasis added)
}\end{quote}

Nosh’s complex technical interface and the inability to integrate it into existing infrastructure resulted in frequent breakdowns that impacted restauranteurs and couriers. Platform administrators, despite their familiarity with the system, also articulated difficulty in navigating the patchwork technical stack Nosh used. 

During the course of a shift, platform administrators said they used, on average, four different platforms simultaneously. One platform administrator describes their shift as follows: \begin{quote}\textit{
    ``No it's an it's a nightmare, we need to...streamline it because my computer just wants to it's like about to  start on fire, because I've got so many things running yeah so so slow, because I always have a million things open''(P3)
}\end{quote} 
Having to jump back and forth between platforms introduced inefficiencies and confusion into their work. Administrators would actively monitor WhenIwork to manage their fleet of couriers, triage customer service requests that came through ZenDesk, answer phone calls from restauranteurs, and coordinate refunds with payroll administrators via Slack. One administrator who oversaw operations at the Fort Collins hub said they wished they could purchase a software from Salesforce to better streamline their workflow but it was prohibitively expensive. 

Administrators acted as the buffer between stakeholders and Nosh’s technical infrastructure. When couriers disagreed with delivery instructions or assigned tasks, administrators would be alerted to the situation. For example, couriers recounted times when they were assigned a delivery for a restaurant that was far away towards the end of their shift. In this situation, since the couriers wanted to stop working when their shift ended, they reached out to a platform administrator via chat and asked them to manually re-assign the order to someone else. Another example of human intervention by platform administrators occurs when restaurants ask them for the same detailed profit and loss reports they received from mainstream platforms. Because the DataDreamers software that Nosh used did not support report generation, backend administrators would manually compile these. The limitations of Nosh's technical infrastructure pushed stakeholders to engage in additional invisible labor to make up for shortcomings: 
\begin{quote}\textit{
    ``The point I'm  trying to make is the platform that we currently use is very limited. So there are many things that we can't access, although the  data is there, so we have to kind of find alternatives in order for us  to create visual reports so that we can analyze the data send it to  our couriers and our restauranteurs, etc.'' (P2)
}\end{quote}

Repair work and invisible labor were essential to making Nosh function properly. At all points in the food delivery process, the technical infrastructure of Nosh was subject to breakdowns. Stakeholders throughout the food delivery process intervened when the technical systems broke down, relying on human-intervention to rectify the situation.

\subsubsection{Human intervention was necessary to overcome breakdowns}

Human operators in Nosh overcame breakdowns through invisible but essential labor. This labor is what the other stakeholders like because they want to interact with people and not machines when things go wrong. However, this requires deep local knowledge and money, and takes time. 

Human mediation plays a critical role in Nosh's operational logic. Platform administrators regularly intervene during the course of food delivery to provide emotional and informational support to restauranteurs, couriers, and customers. As restauranteurs started re-opening and became busier with dine-in traffic, couriers would often have to wait long periods of time to pick up their order. This wait time was compounded with the possibility that restauranteurs did not use the Nosh interface correctly to time the order preparation. To defuse potentially tense situations between restauranteurs and couriers, Nosh administrators 
\begin{quote}\textit{
    ``actually created these templates to send to our couriers that are acting out, getting frustrated with restauranteurs...say[ing] hey we know you're frustrated but we're all a team here let's work together,  here are some ways that you can you know, deal with those types of situations, you  can walk away, you can contact us, you can you know, take a deep  breath.'' (P3).
}\end{quote} 
The goal of these interactions was to show couriers that Nosh stood behind them and wanted to support their well being on the job. Couriers appreciated these interactions, often explicitly calling out the the unique degree of personal connection they had with administrators during our interviews.

A healthy skepticism of the capabilities of the technology used further motivated stakeholders to engage in and rely upon human mediation. Couriers developed rich mental models of what food delivery looked like from the restaurant perspective and anticipated where breakdowns might occur, then worked to address those failure points before problems arose. For example, couriers knew that the restaurant-facing UI was complicated and often led to mistakes with timing so they would call up restauranteurs directly and inquire about order status: 
\begin{quote}\textit{
    ``So I would literally call every single time every restaurant like ‘I have this order. here's the order number/ here's the name. Anything else you need can you can you let me know if this food has been received by you and do you have any idea how long it's going to take and obviously you know whoever's answering, like the hostess or whoever they're just going to say it's going to take this long, and then you have to like multiply it by three you know, because they don't really know.'' (D3)
}\end{quote}

Many couriers we spoke to learned how to discern whether the person on the phone worked front or back of house and knew they had to speak with someone from the back of the house if they were to get an accurate estimate for their order.

Administrators were also aware that the algorithmic systems underlying the food delivery process were subject to breakdowns. They treated the algorithmic systems they used in a proactive manner; anticipating that it would breakdown and require human intervention. As one administrator put it: \textit{``our job as dispatchers is to skim and identify issues.''} Administrators played a vital role in manually checking and correcting the logic of the algorithmic system when complications common to food delivery occurred. This contrasts sharply with mainstream platforms, which have little flexibility built in for when situations deviate from what the algorithm prescribes. For example, a courier described a situation where they were delivering multiple orders but a restaurant had forgotten to start the timer on their end, introducing delays into the process. The courier knew that waiting for the order to be completed would result in the order they had already picked up getting cold, potentially displeasing a customer. The courier reached out to Nosh's dispatchers and informed them of the situation. The dispatcher, understanding that these problems arise in food delivery manually changed the delivery routing system to allow the courier to make a single delivery without being penalized for not picking up the delayed order. Platform administrators are trained to manually intervene in the order dispatching system because they know that problems, such as the one described above, do occur.

Stakeholders act as the glue that holds the technical infrastructure of Nosh together. Platform administrators played a key role in maintaining the cohesiveness of the system: they engage in crucial repair work that takes the form of human-to-human interactions to mediate and patch over breakdowns. Restaurateurs, couriers, and customers point to these interactions as being integral to their perception of being respected and having agency during the process of food delivery. However, platform administrators articulate the limitations of their the technology when it comes to supporting the business operating at a larger scale. As one administrator put it: \textit{``you will break the business because there's no way that you can  support the current infrastructure in a big city it's just not gonna work.''} (P2). This highlights a major tension in designing within the platform economy: at scale, human-to-human interactions that promote sentiments of respect and agency are often untenable.
%Brian pls help the tabl isn't going in the right place
\begin{table}[ht]
    \caption{Technologies Stakeholders Interact With and Repair Work Performed}
    \begin{tabular}{lll}
    \toprule
    \textbf{Stakeholder Group}       & \textbf{Primary Technologies Used}                                                 & \textbf{Repair Work Performed}                        \\
    \midrule
    Restaurants             & \makecell{Nosh tablet}                                                               & \makecell{NA}                                           \\\\
    Couriers                & \makecell{DataDreamers app, \\WhenIWork, Cell Phone}                                   & \makecell{Communicating with \\restaurants and customers} \\\\
    Customers               & \makecell{Nosh mobile app}                                                           & \makecell{NA}                                           \\\\
    Platform Administrators & \makecell{DataDreamers app, WhenIWork, \\ZenDesk, GSuite, Slack, \\Cell Phone, Computer} & \makecell{Re-routing orders, \\dispute resolution} \\ \bottomrule       
    \end{tabular}
\label{table:repairwork}
\end{table}

==> OLD_sections/4_Discussion.tex <==
\section{Discussion}

As our finding demonstrate, human intervention is both normal and necessary in the platform economy. Technical infrastructures underlying the platform economy sometimes break down in local contexts, requiring people to repair them. However, mainstream platforms and indie platforms handle breakdowns in vastly different ways. Nosh’s handling of breakdowns demonstrates why human intervention should be incentivized rather than penalized and we propose several mechanisms through which human intervention can be promoted. To explore the feasibility of these design recommendations, we call attention to the importance of business models and economic constraints of platforms seeking to incentivize human intervention. 

We first briefly restate our research questions and corresponding findings to provide a high-level overview of the implications for design. We then translate these implication for design into concrete recommendations with considerations for business model and economic constraints.

\begin{itemize}
    \item \textbf{RQ1: What motivates stakeholders to join an indie platform?}
    \begin{itemize}
        \item \textbf{Findings}: We find that restaurants, couriers, and customers join Nosh because they are afforded a higher degree of agency and financial security.
        \item \textbf{Implications for Design}: Design of automated systems in food delivery (\textit{e.g.} Routing systems, dispute resolution, etc,.) should not penalize human intervention and should instead accept that human intervention is necessary. 
        \item \textbf{Explanation}: The sentiments of agency and ability to attain a higher degree of financial security are inextricable from the presence of human intervention in the face of breakdowns. Having a platform administrator act as a buffer between users and technical systems enabled stakeholders to negotiate and build trust with an entity they felt understood and looked out for them. 
    \end{itemize}
    \item \textbf{RQ2: What are the capabilities and limitations of the sociotechnical infrastructure that powers an indie platform?}
    \begin{itemize}
        \item \textbf{Findings}: The infrastructure of Nosh is made up of a patchwork of software systems that tend to breakdown and frustrate users. Users overcome these frustrations through human intervention, usually on the part of platform administrators. The current system works well enough at a local level, because there are local support staff, but would most likely fail if scaled up. 
        \item \textbf{Implications for Design}: Design of food delivery platform systems needs to take into account the business model and economic incentives at hand.
        \item \textbf{Explanation}: Nosh's model was able to continue operating with relatively unsophisticated technology infrastructure \textit{because} their business model was set up to service local hubs. Each local hub had its own support staff that had rich knowledge of the stakeholders in that community and the ability to address their concerns effectively. Additionally, Nosh was able to rationalize its human labor costs because they were entirely reliant upon restaurants and customers for profits so they had extremely strong incentives to provide excellent support service. 
    \end{itemize}
\end{itemize}

In sum, users joined Nosh because of the human intervention, thus design for systems to support food delivery should account for key role it plays. This level of human intervention would not be viable under mainstream business models that have differing economic incentive structures. However, it is worthwhile to explore how technical solutions can be developed to support alternative business models like Nosh because they offer a fundamentally different, more human-centric, organization of work in the food delivery platform economy that promotes agency, respect, and financial security. We expand on these claims below in more detail. 
  
\subsection{Human intervention is normal and necessary in the platform economy}
\subsubsection{Breakdowns are inevitable in food delivery platforms} 
During the course of platform-mediated food delivery, breakdowns are guaranteed to occur: unexpected traffic jams block routes, restaurants overlook details of an order during rush hour, and customers receive cold food. Previous work has highlighted that systems of coordinated workflows fail due to a disparity between how they are designed and how they are actually used in practice---making breakdowns inevitable~\cite{grudinWHYCSCWAPPLICATIONS}. 
% For example, GrubHub's ``Free Lunch'' promotion program in May 2020 offered customers a heavy discount on orders placed through the platform. As a result, restaurants, who were not told about the promotion beforehand, were overwhelmed with orders and ended up losing money because couriers were so overworked that they could not pick up the prepared food~\cite{fortneyAnyoneSurprisedGrubhub2022}. While this is an extreme example, it showcases how breakdowns become the burden of both couriers and restaurants ~\cite{qadriPlatformWorkersInfrastructures2021}.  

\subsubsection{Domain expertise is essential to address breakdowns} 
Despite the responsibility of breakdowns falling on users, our participants noted that they were often penalized by mainstream platforms for stepping in when the intervention did not fit into the intended design. As D2 pointed out, DoorDash would threaten to take away a delivery if they did not exactly follow the prescribed route, even if their desired route avoided delays and roadblocks. Being unable to exercise discretion in their jobs left restaurateurs and drivers feeling like they lacked agency to make decisions and have input, even though they were domain experts. Disregarding domain expertise is a longstanding trend in the design of algorithmic systems~\cite{petreGamingSystemPlatform2019,sambasivanDeskillingDomainExpertise2022,starLayersSilenceArenas1999}. Failing to recognize users' domain expertise in conducting food delivery emerged as one weakness in the logic of mainstream food delivery platforms. In contrast, Nosh recognized the essential role of domain expertise and, in many cases, their platform \textbf{relied} upon it. As a result, our participants had \textbf{agency} over their participation. Re-iterating what R6 said: \textit{``DoorDash and Grubhub are fantastic technology companies that deliver food. Nosh is a fantastic food delivery company that has some technology.''}  

\subsubsection{Design for the platform economy should incentivize human intervention}
The design of systems in the platform economy is typically defensive: platforms are concerned with workers gaming the system. Thus platform owners design systems to harshly penalize behavior that deviates from what they prescribe~\cite{rahmanInvisibleCageWorkers2021a,watkinsTookPicGot2020,gray2019ghost}. However, doing so penalizes users for attempting to rely on their expertise to repair breakdowns as they occur~\cite{qadriPlatformWorkersInfrastructures2021}. Nosh did \textit{not} penalize users for leaning on their domain expertise, rather they incorporated it as a fixture in their platform. Platform administrators embodied this notion of human intervention and input as essential to the function of a delivery platform: they were able to understand edge cases in ways algorithms could not. Centering human intervention in the Nosh platform was a key factor in motivating users to join and enabling the constant repair of the platform in light of its low-fidelity technological infrastructure. Building on this case study, we propose several design recommendations for building systems in the platform food delivery industry that could incentivize human intervention: 

\begin{itemize}
    \item Design routing algorithms that allow for courier discretion (e.g., avoid threatening drivers for reasonable deviations from the prescribed route). 
    \item Make a concerted effort to keep humans in the loop (e.g., have a group of designated platform administrators for each locale to act as support staff).
    \item Allow for transparent two-sided negotiation in dispute resolution processes rather than relying on cookie-cutter feedback forms and pre-determined solutions (e.g., build a stronger customer relationship management process to track issues and resolutions).
\end{itemize}

We provide a speculative example of our design recommendations in action to illustrate how this more human-centred technology stack might work. One scenario where we could apply these designs is during a two-batch order when a courier picks up two separate orders that have different drop off locations. Issues with batch orders are common in mainstream platforms: long wait times at restaurants frustrate couriers and customers~\cite{after-brickBatchingOrdersJust2021}. With our recommendations, if the restaurant preparing the second order suddenly changed the estimated preparation time due to a last-minute dinner rush, the driver could drop off the first order rather than wait for the second order to be prepared---letting the first get cold and risking upsetting the customer---\textbf{because} they would not be penalized for going against the prescribed route. If a customer was unhappy with their order, a local platform dispatcher could reach out to understand the problem and determine an acceptable solution. Doing so would clarify which party might be at fault, thereby avoiding penalizing the incorrect party for something out of their control. Through increased transparency, restaurants and couriers could better understand reparative actions from the platform. As our findings show, centering human intervention in coordinated work systems is essential to increasing user confidence: the ability to understand and be heard by human intermediaries increased user agency and reinforced positive perceptions of Nosh.  

However, these design recommendations --- though empirically informed --- are virtually impossible for mainstream platforms to implement due to incompatible business models and economic constraints. Thus, in the next section, we discuss how economic incentives shape design in action and how HCI researchers can reflect upon these constraints when making design recommendations. 

\subsection{Business model and economic structure enable and constrain design recommendations}
Design recommendations are limited in impact if they fail to consider the business model, organizational constraints, and economic dimensions at hand. Thus, HCI scholars need guidance to navigate design recommendations that may not be supported by platforms' economic incentives and business model.

\subsubsection{Why our design recommendations wouldn't work in a mainstream food delivery platform}
While the design recommendations we make above are empirically informed, they are derived within the context of an indie food delivery model. It would be difficult, if not impossible, to apply these recommendations to a mainstream food delivery platform given the values and economic constraints at hand. We review each recommendation and explain which factors of mainstream models hamper their efficacy. 


\begin{itemize}
    \item \textbf{Making Room for Courier Discretion:} In mainstream platforms, allowing for driver discretion would introduce complexity into their fleet management systems which oversee thousands, not dozens, of couriers and would obstruct their ability to prevent gaming behavior by couriers. Essentially, the scale at which mainstream platforms operate constrains the efficacy of this design recommendation. Additionally, each local Nosh hub hires couriers through an interview process, while mainstream platforms offer a ``log on and drive'' model, limiting the ability to verify courier expertise and capability which contributes to the defensive design of their algorithmic management systems~\cite{rahmanInvisibleCageWorkers2021a}. 
    
    \item \textbf{Promote Humans-in-the-Loop in Delivery Operations:} Restaurants, customers, and couriers valued the presence of human platform administrators who intervened when systems broke down. The human agents in Nosh were helpful to the other stakeholders because they were locally situated: each hub had its own staff of platform administrators that assisted customers, restaurants, and couriers operating within that hub. Thus, these platform administrators could provide relevant and responsive support that understood the contexts in which other stakeholders were operating. In contrast, mainstream food delivery platforms operate at a national scale and do not have regional hubs staffed with local support agents to support the commerce of each hub~\cite{beharBuildingUnifiedChat2022,GrubhubEasyCustomer}. Providing the localized support that restaurants, customers, and couriers value would necessitate that mainstream platforms decentralize their operations and establish regional hubs.
    
    \item \textbf{Build Systems That Support Transparent Two-sided Dispute Resolution:} Restaurants we spoke to were appreciative of the transparency and support they received from Nosh when problems arose, characterizing Nosh as straightforward and transparent, in contrast to experiences with mainstream platforms as frustrating and one-sided. For Nosh, it was extremely important to maintain restaurant satisfaction \textit{because Nosh was entirely dependent on restaurants for investment}. In contrast, mainstream platforms---as we depict in Figure~\ref{fig:financialflows}---do not have the same degree of financial obligation to restaurants \textit{because they have access to venture capital and shareholder investment}. These differences in financial dependence fundamentally shape how stakeholders are treated in both systems. It would be difficult to enforce the implementation of more nuanced dispute resolution processes without strong economic incentives. Reiterating what R2 said: \textit{``...it's not just Nosh's financial success, they're also looking out for each individual  restaurant's success because \textbf{[Nosh is]} those individual restaurants''} (emphasis added).
\end{itemize}

\subsubsection{A path forward: Broadening the scope of design research to include policy and economic considerations}
HCI scholars studying the platform economy often share the goal of trying to improve the conditions for participants by mitigating the negative impacts of technical systems through re-imagining their design. However, the technical interventions proposed often fail to consider the role of policy and economic incentives in shaping their feasibility~\cite{jacksonPolicyKnotReintegrating2014}. Attempting to improve conditions in the platform economy solely through technical interventions without considering the contexts in which those interventions would operate limits HCI scholars' ability to understand \textbf{\textit{what}} these interventions will fundamentally change: stopping at design leaves many questions unanswered. It is well established that the platform economy, despite its claims of offering liberatory access to on-demand work, further entrenches systems of oppression and marginalization (\textit{e.g.}~\cite{mcmillancottomWherePlatformCapitalism2020}); But what, realistically, are technical design recommendations doing to fundamentally reorganize the structure of the platform economy to avoid predatory inclusion and precarious conditions?  

We call for HCI researchers seeking to improve conditions in the platform economy to examine two paths forward: 
\begin{enumerate}
    \item \textbf{Consider the ``Policy Knot'' that shapes the efficacy of design recommendations.} As Jackson and colleagues suggest, it is imperative for HCI scholars to think through how policy plays a key constitutive role in shaping the deployment and effects of technology~\cite{jacksonPolicyKnotReintegrating2014}. In the case of food delivery platforms, we call for HCI scholars to examine how policy, such as securities law, constrain the viability of alternative \textit{business models} that are necessary to support technical interventions that improve conditions of participation. HCI scholars do not need to be completely reliant on external domain expertise for guidance on how to study policy constraints on organizations. Rather, they can turn to early HCI and CSCW work, such as that done by Susan Leigh Star, Wanda Orlikowski, and Anselm Strauss for methdological guidance on conducting empirical research that incorporates policy and organizational factors as key elements of design investigations~\cite{orlikowskiInformationTechnologyStructuring1991,orlikowskiStudyingInformationTechnology1991,starLayersSilenceArenas1999,straussSocialOrganizationMedical1997}. 
    \item \textbf{Continue to examine alternative models within the platform economy.} As Glen Weyl suggests, it is essential for scholars to consider and contribute to the plurality of options in the marketplace~\cite{weylWhyAmPluralist2022}. In other words, it is important that scholars continue to investigate how we can further diversify the options available for participation rather than settle into the mindset that we must operate only within existing options. In the context of food delivery platforms, we call for HCI scholars to continue investigating how alternative models for food delivery can be viable \textit{and} simultaneously support participant well-being. This could look like HCI scholars exploring technical mechanisms for governance and coordination across multiple localized hubs that operate under one parent company that provides technical and knowledge resources.  
\end{enumerate}

Complicating design recommendations with broader considerations for the social, political, and economic contexts at hand is not new to the fields of HCI and CSCW, especially in the context of systems of coordinated work ~\cite{starLayersSilenceArenas1999,straussSocialOrganizationMedical1997,grudinWHYCSCWAPPLICATIONS}. By presenting our design recommendations and then complicating them by considering the constraints of business models and economic incentives, we draw attention to the need for HCI scholars to consider how proposed technical interventions will work to fundamentally re-shape some of the root causes of negative impacts experienced by users. We urge HCI scholars to consider the role of policy in informing the impacts of design, however well-intentioned that design may be, and encourage them to continue exploring how a plurality of options for participation in the platform economy can be supported through technical design. In the words of Susan Leigh Star and Anslem Strauss, two eminent figures in the field of infrastructure studies within CSCW and HCI, we call for HCI researchers to \textit{``look in every circumstance at how the application affects relations of power and the nature of work.''}~\cite{starLayersSilenceArenas1999}. 

==> OLD_sections/5_Limitations_Future_Work.tex <==
\section{Limitations}
Our results might not generalize to other indie platforms because we studied a single platform. This platform's location and idiosyncrasies are likely to influence our insights.  Also,  our participant sample is biased because those who responded to our call for participation felt strongly enough about expressing their opinion that they chose to sit for an hour-long interview.  In the future, we plan to expand this research to hundreds of other indie platforms in the United States and gather latent data from online sources beyond interviews.

==> OLD_sections/6_Conclusion.tex <==
\section{Conclusion}

We discovered the essential role that human intervention plays in making food delivery platform users feel respected. Restaurants, couriers, platform administrators, and customers all took the risk of participating in a relatively untested model of indie delivery because they were given a greater degree of agency and financial security which made them feel respected in ways they were not when participating in mainstream food delivery platforms. When breakdowns occurred during the process of food delivery, stakeholders were able to understand, establish control over, and shape the outcome of the situation. Drivers, restaurants, and customers valued the ability to interact and negotiate with a human representative in a way they were unable to with the algorithmic systems of mainstream platforms. Human intervention from Nosh platform administrators played a key role in smoothing over breakdowns as administrators acted as a buffer between stakeholders and the technology. Drivers also stepped up to intervene when algorithmic systems broke down and felt comfortable doing so because they knew a human dispatch agent was available to reason with. We put forth recommendations to build routing, dispatching, and customer service systems for food delivery platforms that incentivize human intervention given the inevitability of its occurrence. We caveat our recommendations with the note that incentivization of human intervention is not viable under most business models of mainstream food delivery. Thus we call for HCI scholars to return to traditions from the early days of the field to be attentive to the broader social, political, and economic contexts at hand when making design recommendations. 

==> OLD_sections/7_scrap.tex <==
Stakeholders who participate in mainstream platforms are required to fit themselves into the logics of the platforms with little room for negotiation. For example, restaurants have little to no say over dispute resolution, drivers can't reason with a dispatching algorithm that penalizes them for taking alternative routes, and customers are often met with platitudes and generic solutions when problems arise with their orders. Stakeholders felt that the rigid structure and design of mainstream delivery stripped down food delivery to a mere exchange of goods and services and in doing so, removed vital humanistic elements from the process. In contrast, indie platforms like Nosh preserves stakeholder agency in the food delivery process and aligns well with stakeholder values, which were key motivations for participation across all stakeholder groups. According to stakeholders, Nosh facilitated fair and transparent dispute resolution, gave drivers agency to choose routes during the delivery process, and offered customers personalized solutions when problems arose with their orders. However, many of these positive aspects of Nosh's service were necessitated by shortcomings in technical features of the platform that required expensive and time consuming human labor to compensate.  

\subsubsection{Restaurants participated in Nosh due to increased transparency into delivery process, lower commission fees, and a desire to be respected by delivery platforms}
Restaurants gain greater agency over their role in the food delivery process because Nosh gives them the ability to provide input which is then taken into account to directly shape the delivery platform's operations. Each Nosh location operates as a collective where restaurants invest in the delivery service and therefore have a say over how business is conducted. Restaurants described feeling as if they had much more meaningful control over and understanding of the food delivery process as part of Nosh. This juxtaposes sharply with how restaurants viewed their participation in mainstream platforms with R6 summarizing the comparison by saying: \begin{quote}
    "there's a lot of people, giving input and their thoughts, it [Nosh] is truly a cooperative where you know matters of importance are voted on and discussed openly. It's very transparent operation from Nosh, the other services, you know no transparency [is] there you know it's just a plug and play...I don't have any say on what happens once I sign up." (R6)
\end{quote}
Having a say over operations helped bolster restaurants' perception that, in Nosh, they were truly partners with the service rather than just provisioners of a good that the service would oversee itself. Restaurants contrasted this with previous negative experiences they had with mainstream platforms which they described as "not hav[ing] the restaurants' best interests at heart" (R1). Despite their negative experiences, several restaurant owners chose to supplement Nosh with participation in mainstream platforms. They expressed anxiety over losing customers who wanted to order off an "app that's already on [their] phone" (R1) when relying solely on indie platforms. Restaurants felt compelled to meet consumers where they were by signing on with mainstream platforms, despite the poor treatment they would receive. This pressure to sign on with mainstream platforms is a well-documented part of their marketing strategy where dominant platforms tell restaurants they risk falling behind and being the "only one on their block not on the platform" \cite{sharmaConvenienceDeliveryApps2021}. In some cases, restaurants described "dark patterns" employed by mainstream platforms where the platform would post the restaurant's menu and contact information on their app, without permission, and allow users of the app to place orders to the restaurant through their platform \cite{DarkPatternsInterfaces}, \cite{DCAttorneyGeneral}. R5 described this deceptive practice as: \begin{quote}
    "GrubHub will find our menu put it online without telling us...and then so you'll get a phone call from somebody and then they'll place an online order to pick up. And when they pick up it's it's a GrubHub driver. What they do later is contact you and say hey look you had X amount of deliveries [through] GrubHub, and you know, do you want to sign up for GrubHub?" (R5)
\end{quote}  
Restaurants felt like such behaviors indicated that mainstream platforms did not value their agency. During the COVID-19 pandemic, restaurants realized "it became essential for us to have delivery service" (R3) and thus sought out access to delivery platforms such as GrubHub and DoorDash. However, negative experiences with mainstream platforms drove restaurants to seek out alternatives where they would have more agency over their role in the food delivery process and would be treated with respect. \par

Restaurants mentioned that mainstream platforms failed to treat them with respect during dispute resolution processes as well. In contrast, Nosh, despite its lacking technology and smaller customer base, gives restaurants confidence in their service because they know that "[Nosh's] customer service arm is there to support us" (R1). Food delivery, as one restaurant owner put it, has "...a general amount of just error rate that we have to acknowledge..." (R1). Indie platforms, like Nosh, stand out to restaurants because "...as a local company, Nosh has always made it a very strong piece of their platform to be better than the big companies at rectifying those problems." (R1). Several other restaurant owners articulated this same sentiment. Nosh was better at working with stakeholders to resolve issues as they arose during the food delivery process, instead of offering frustrating  cookie-cutter solutions  or adjudicating disputes in isolation as mainstream platforms did. In some cases, restaurants did receive support from mainstream platforms when problems arose. However, access to that support was conditioned on restaurants doing a certain volume of business with the platform: "because we do X amount of volume with DoorDash we do have a dedicated customer service person" (R1). With mainstream platforms, restaurants had to "pay to play" to access both helpful customer support and the platforms' customer base. \par

Restaurants reported paying a 30\% commission to mainstream platforms, on average, in order to conduct business with them. Restaurants that were of a certain size were able to exercise some negotiating power over commission rates, but overwhelmingly, restaurants in our sample were small businesses that could not leverage their sales volume to effectively negotiate. Thus, restaurants with already thin profit margins had to raise menu prices to make up for the high commissions charged by mainstream platforms, which they worried would affect their customer base: "Commission rates are important...and we do raise our prices significantly on delivery platforms to recover a portion of that commission" (R7). Nosh offered a more financially sound alternative for many smaller businesses. Nosh charged between 15-20\% commission rate, according to conversations the research team had with Nosh administrators, and the cities in which Nosh operated subsidized restaurants' (and customers') delivery fees through the platform \cite{CityBoulderBrings}. Restaurants who participated in Nosh expressed that their low commission rates and other benefits helped them squeeze by during the critical time of the pandemic. 

Restaurants felt that they were treated with far greater consideration by Nosh than by mainstream platforms. This perception stemmed from their contrasting experiences with customer service as well as their view that Nosh's commission scheme aligned with what they could afford: "...it's not just Nosh's  financial success they're also looking out for each individual  restaurants success, because \textit{they are} those individual restaurants" (R2, emphasis added). Nosh operationalized respect and trust in their relationships with restaurants in how they treated them financially and professionally.

\subsubsection{Drivers participate in Nosh because the feel like the platform treats them with respect and provides financial stability}
Similar to restaurants, drivers felt that Nosh treated them with more respect than mainstream platforms did. Nosh gave drivers more agency over their role in delivery, financial security, and equitable treatment. With mainstream platforms, drivers described being treated like agents of the dispatching algorithm which dictated their activity and penalized them for deviation from the norm. This treatment reinforced drivers' beliefs that mainstream platforms did not recognize the value of their local expertise when it came to navigating routes for delivery nor did it value their ability to think through and problem solve on their own: the algorithm knew best. With Nosh, drivers were able to push back against the dispatching algorithm when assignments didn't make sense due to the local nature of the platform: \begin{quote}
    "with Nosh we have kind of a unique situation, because it is more localized and customer oriented...we do have an [AI] that assigns orders to us, to a degree, but there's also dispatchers who are creating human intervention periodically. And I know that because I probably drive more than every other Nosh driver." (D5)
\end{quote}
Drivers describe Nosh's dispatching algorithm as a system that is heavily mediated by human dispatchers. This understanding that there were humans who could intervene to assist drivers increased the trust that drivers had in the system and bolstered drivers' perceptions of Nosh as being fairer than mainstream platforms. D5 illustrates this point, saying: "Overall, our system is much more fair than other services that I worked for because you have that human aspect of problem solving." (D5). The perception that algorithms are more fair when human intervention plays a role is supported by existing research on trust in automated systems \cite{}. Drivers felt that the involvement of human dispatchers at Nosh enabled them to say no when they were assigned orders that didn't make sense to them, reinforcing their sense of agency. Additionally, drivers felt that their ability to select best routes for delivery and exert control over the delivery process was respected at Nosh because the platform did not track their location during the delivery process: \begin{quote}
    "One thing I also like with Nosh versus DoorDash – Nosh does not track my movements and my location in a way that... If I'm not heading to the restaurant and if I'm biding my own time, it's not going to tell me to turn around or else I’ll lose the order. That's something that I remember with DoorDash, that even if there was a large wait time and I didn't head in the direction of the restaurant first, the app would track that and say, 'Are you heading to the restaurant? Looks like you're not heading in the direction of the  restaurant, if you're not going to be heading there in the next couple minutes, we're going to reassign your order to somebody else.'" (D2) 
\end{quote}
D2 clearly articulates a sentiment voiced by all the drivers in our study: Nosh treats drivers with respect throughout the delivery process by trusting them to conduct the delivery properly without paternalistic levels of oversight and control. Nosh, unlike mainstream delivery platforms, has an intensive vetting process when hiring drivers, which allows them to develop a rapport not present in the "log on and drive" models of mainstream platforms. While Nosh's hiring process created higher barriers to entry to becoming a driver, drivers felt that this gatekeeping mechanism was important to promoting financial security: \begin{quote}
    "One of the things with the scheduling and the shifts that they [Nosh] offer is there as a preventative measure to not over-saturate the market with drivers because when you sign on for like Door Dash or like Grub Hub, or any of those, there could be hundreds and hundreds of drivers...with Nosh, you know, you can kind of be the big fish in a small pond. If you work hard, and you're efficient and fast, you can make all the money. So there's less saturation I guess is probably the main thing I like about it." (D3)
\end{quote}

Nosh's scheduling system provides an interesting contrast to the "log on and drive" models of mainstream platforms. Mainstream platforms emphasize the \textit{flexibility} of delivering for them when advertising to potential drivers. These platforms associate their flexibility with drivers' ability to log on and drive whenever they like. However, this low barrier to entry for drivers often results in over-saturation of the local driver supply which in turns makes it difficult for drivers to actually score work while logged on, according to drivers we interviewed who also drove for mainstream platforms. Gig platforms' reliance on an oversupply of drivers is a well-documented critique of these platform's business models \cite{marshallGigCompaniesFear}. As such, drivers who participate in mainstream platforms have voiced concerns about the work not being as flexible as platforms claim because they cannot actually \textit{get} work when they log onto the platform. Drivers we interviewed characterized Nosh's hybrid scheduling-open shift system as being \textit{both} more flexible and secure than the "log on and drive" model of mainstream platforms. Nosh's hybrid scheduling-open shift system allows drivers to submit their preferred schedules a week in advance and then assigns drivers shifts based on their availability and preferences. For example, a driver who wanted to work on Tuesday evenings might be assigned the Tuesday dinner rush shift. Drivers could drop shifts after they were assigned by notifying Nosh dispatchers and these shifts would become available in the open shifts tab of the driver's mobile application. This scheduling model combined with Nosh's guaranteed floor-pay provided drivers with a sense of financial security that motivated their participation in Nosh. 
%transition sentence to customers?

\subsubsection{Customers participate in Nosh because they see it as an ethical alternative in the food delivery economy that enables them to support local businesses}
%call dispatchers, "what would make this right", keep money in local economy
Customers participated in Nosh because they perceived Nosh as being an ethical food delivery option that enabled them to support local businesses during the pandemic. Customers, like restaurants and drivers, felt that Nosh treated them with respect during dispute resolution which bolstered customers' perceptions of Nosh as a company that truly cared for its community of users. However, the higher quality of customer service that Nosh provided is not as seamless as that provided by mainstream platforms which are able to leverage technical affordances within their apps to handle dispute resolution. 

The majority of customers we interviewed described being avid supporters of local restaurants before the Covid-19 pandemic. When the pandemic began, customers sought out ways to patronize local restaurants in an effort to support their community: " I love that [Nosh] is local so that's my biggest thing...it has a lot of like my favorite local restaurants" (C4). Customers noted that even though other food delivery platforms, like DoorDash and UberEats, also had some local restaurants listed they preferred ordering from Nosh because it was "just a little bit more ethical" (C1). For customers, ethical meant that the platform treated both drivers and restaurants with respect by not engaging in exploitative financial practices such as taking cuts of drivers tips or charging exorbitant commission fees for restaurants. While customers did not have first-hand knowledge about tip distribution or restaurant commissions, they put a lot of stock in popular narratives about mainstream platforms' mistreatment of drivers and restaurants with one customer justifying their support of Nosh by saying: \begin{quote}
"I mean I read the news article, you know, in the Times about how GrubHub and DoorDash are just ripping off restaurants like it's not okay take advantage of people during a pandemic, so I prefer not to use companies that do that." (C3) \end{quote}

Customers felt that Nosh not only treated restaurants and drivers better than mainstreams platforms but also treated them with more respect during the dispute resolution process. When an order went wrong (i.e. missing an item, taking longer than expected, etc.), customers were able to easily contact a real, local person from dispatch for help. A phrase that stood out to customers across the board was "what can we do to make this right?". According to conversations with platform administrators, dispatchers were trained to always ask the customer what solution they desired rather than simply presenting them with a pre-configured solution. This is noticeably different from mainstream platforms where dispute resolution is usually carried out without immediate human intervention, through a form within the app that has pre-configured options for the types of issues you can dispute \cite{}. The dispute is then routed to a customer service queue and a solution is determined, usually unilaterally, by the platform and automatically added to the customer's account. Customers we spoke to discussed their dispute resolution experience with mainstream platforms, emphasizing the one-sided nature of the process with mainstream platforms with one describing it as such: \begin{quote}
    "One of the times I ordered formula, [Postmates]...delivered the wrong kind. So I reached out and I they told me I could return the item. I mean, I get in my car, go return the item, and get what I wanted, and then they gave me a credit. Which I was, like all right fine whatever like that's very irritating that like you should really just send somebody out with the correct thing. And then they refunded my account, but it was a credit on Postmates and then, when I went to use it had been...a while my credit expired...I ended up having to not end up not getting that money at all." (C2) 
\end{quote}
While customers appreciated the two-sided nature of dispute resolution with Nosh, this type of involved problem solving is not as seamless as the resolution process offered by mainstream platforms. However, customers felt that the trade off between convenience and quality of service was justifiable as they ended up getting a solution that they actually met their needs with Nosh. Mainstream platforms, by nature of their scale, cannot offer customized solutions in every situation; by necessity they design their dispute resolution process to be as generalizable as possible. This highlights a key tension between scale and quality of service when designing food delivery platforms. 



% While mainstream food delivery platforms are able build beautiful, interactive, and highly personalized mobile app interfaces customers we interviewed described these interfaces as being overwhelming and not particularly useful when ordering. Most customers said that since they already knew the restaurants they wanted to order from, they had no need to browse through recommended options when ordering. However, customers did note that Nosh's simple interface did not allow for some of the filters that would be useful for them. For example, several participants had food allergies and wanted to be able to screen options by allergy-friendliness but Nosh's UI did not support this kind of filtering. While most mainstream platforms have a filter for food allergens, the customers we spoke to said that they would still be wary to trust these labels on the app unless they had been to the restaurant they were ordering from before and had first-hand knowledge that the restaurant was in fact allergen-friendly. Since the restaurants on Nosh are all local, customers with allergies were able to overcome the lack of an allergen-filter within the Nosh app because they had first-hand knowledge of what restaurants were "safe" to order from. Nonetheless, customers with allergies articulated a desire for a feature in Nosh that would allow them to make note of what restaurants were safe for them to order from in the future. 

\subsubsection{Platform administrators participated in Nosh because they believed in the "local-first" mission of the company but spent most of their time compensating for technical shortcomings}
%treated as valuable team members, enjoy the inter-personal relations aspect of their work, empowered to problem solve, able to work remotely 
Platform administrators participated in Nosh primarily because they believed in Nosh's mission of supporting local communities through locally owned and operated food delivery. Additionally, administrators voiced a strong passion for working in a small start-up environment, often comparing themselves to scrappy underdogs challenging the main players in the food delivery space. While platform administrators were enthusiastic about Nosh's mission to support local communities their ability to do so was often impeded by a weak IT ecosystem that forced them to spend significant portions of time patching up technical shortcomings.

Of the administrators we interviewed, all but one had prior experience working in the restaurant and/or food delivery industries. They overwhelmingly articulated a strong resonance with Nosh's mission to support local communities, often drawing connections between their previous experiences working in the restaurant industry industry and their desire to support local establishments. As one administrator put it: " working with restaurants and actually being able to help them and benefit them through delivery is really rewarding for me [given] my past life as a cook" (P4). Many felt like they had an active role in supporting the local economy through their position as an administrator at Nosh. Administrators detailed the amount of labor they put into forming and maintaining relationships with local community partners: \begin{quote}
    "I mean if  there's an issue with [the restaurant's] tablet we get somebody in there  within 24 hours like if not within a couple hours. We have people that  are in in walking into the restaurants constantly checking in" (P1) 
\end{quote} 

Platform administrators efforts to support local communities extended beyond the care with which they treated restaurants. Administrators expended a significant amount of effort to manually schedule delivery drivers according to individual preferences. This scheduling process ensured that drivers were able to work the shifts they wanted but also gave drivers the flexibility to pick from open, unclaimed shifts. Each week, drivers submit their preferred work schedule through the When I Work application, a popular workforce management software. A platform administrator then aggregates all the shift preference data and creates a schedule, trying their best to match driver preferences with availability and leaving unclaimed shifts open for drivers to claim at any time. None of the drivers we spoke with voiced any concerns about not being scheduled when they wanted to work. In addition, administrators worked to provide emotional support to drivers through cultivating personal relationships: \begin{quote}
    "I think they like the personal interaction or  dispatchers come on every morning they talk to the to the drivers say  hey how's it going. You know, some of them even have my dispatchers phone  numbers and they text you know...we're not this faceless  company right we're just we're people that are here. We're here to  listen to the drivers and and in and try to accommodate their needs  and their frustrations."  (P3)
\end{quote}

Administrators we spoke with referenced the phrase "what can we do to make this right?" when discussing their commitment to customer satisfaction. When problems occurred with a delivery an administrator would contact the customer, asking them what solution they desired instead of prescribing a pre-configured solution to the problem at hand. Additionally, platform administrators said that they considered the perspectives and well-being of all involved parties during the dispute resolution process: "We're going to get the  restaurant taken care of we're going to get the customer taken care  of...at the end of the day, that's all that matters to us." (P1). In this case, the platform administrator detailed how Nosh would pay the cost for remaking the meal that was delivered cold so that the restaurant would not be penalized for a situation they could not control. This was corroborated by restaurants we interviewed who noted that this consideration differentiated Nosh from mainstream platforms that would penalize restaurants without thoroughly investigating the dispute at hand. 

However, platform administrators efforts to support local communities and workers were impeded by technical shortcomings in the Nosh IT ecosystem. As one administrator put it, they are constantly "putting out fires" caused by technical failures in the ordering and dispatching system. For example, drivers claim that the Nosh application often crashes making it difficult to perform timely deliveries. Administrators say in these cases, they have to manually intervene to help drivers troubleshoot and coordinate delivery pick up times with the restaurants while the application restarts. This additional step often causes delays that frustrate all stakeholders involved. Administrators serve as the back-up system for Nosh, manually orchestrating deliveries when their technology fails. 

As a small company, Nosh does not have the resources to hire in-house software engineers to develop custom back-end software, rather they rely on white-label to run their operations. As such, Nosh is limited by the technical capabilities of the white-label software and is unable to generate the reports and information that restaurants and drivers are used to receiving when working with mainstream delivery platforms. To compensate for this shortcoming, Nosh's sole data analyst (P2) spends half of their work week manually generating reports, validating data, and resolving financial disputes:  \begin{quote}
    "The point I'm  trying to make is the platform that we currently use is very limited. So there are many things that we can't access, although the  data is there, so we have to kind of find alternatives in order for us  to create visual reports so that we can analyze the data send it to  our drivers and our restaurants, etc" (P2)
\end{quote}.  
While P2 has built some automation into this process through creating Excel macro scripts and Google Data Studios dashboard, they acknowledge that if Nosh were to grow any bigger, the current workflow would be unsustainable because of the amount of manual labor it requires. 

Because Nosh's technology ecosystem is prone to failures, administrators explain that they spend the majority of their workday smoothing over technical failures through human intervention; Breakdowns caused by faulty POS tablets are addressed through phone calls and in-person visits to restaurants, driver frustrations with long wait times are assuaged through direct 1:1 messaging with administrators, customer complaints about the clunky ordering interface are fielded by administrators via phone calls. While this labor makes Nosh functional, administrators across the board were quick to call out the unsustainable nature of Nosh's current operations. As one administrator pointed out, with the current IT ecosystem that Nosh uses, it would not be feasible for the platform to service a larger city than Fort Collins. Administrators often had to juggle multiple pieces of software with limited interoperability because Nosh could not afford to purchase a fully integrated operating service. The limited interoperability meant that administrators had to spend significant amounts of time manually bridging the gaps between disparate pieces of software which put constraints on their efficiency and ability to scale up services. In addition, due to the limited interoperability of software breakdowns would often occur, forcing administrators to take on the additional labor of reaching out to affected stakeholders to smooth over incidents. Ironically, stakeholders identified the presence of administrators during breakdowns as one of the main reasons they were attracted to using Nosh; administrators were able to offer stakeholders human contact which made the stakeholders feel respected and cared for. However, as multiple administrators pointed out, it is unsustainable for Nosh to continue operating in its current fashion because the reliance on human intervention constrains the platform's ability to operate efficiently.




\subsection{"Indie" platforms are comprised of modular building blocks that enable lower barrier to entry for small business but tend to breakdown in large-scale contexts}
Unlike mainstream platforms that use a vertical integration model to run their delivery services, Nosh relies on patchwork of third-party software and hardware. Nosh utilizes software and hardware made available through the "unbundling" marketplace ––a relatively new cottage industry that aims to provide the tools and services needed to build your own version of popular platforms. In the context of food delivery, the unbundling marketplace offers restaurants, and small independent delivery platforms, the ability to create and run their own delivery service through access to POS systems, website builders, white-label ordering software, order integration services, and delivery logistics. Nosh draws upon the the unbundling marketplace to build its platform and is thus constrained by the affordances of these third party services. Nosh utilizes a white-label restaurant delivery software called Data Dreamers to handle order placement, order fulfillment, dispatching, and report generation. While this patchwork of software and services enables Nosh to operate as a small, "indie" platform, problems with interoperability and technical limitations lead to breakdowns in large-scale contexts. As one platform administrator put it: "No it's an it's a nightmare, we need to...streamline it because my computer just wants to it's like about to  start on fire, because I've got so many things running yeah so so slow, because I always have a million things open" (P3). The administrator lamented that while they would like to purchase a service such as those offered Salesforce to streamline their operations, the cost would be untenable and therefore they were stuck using more readily available disparate pieces of software to run the business. 

%CUT THIS - TOO MUCH DETAIL While Data Dreamers provides the bulk of functionality that Nosh needs to run its platform, it lacks some affordances, such as driver scheduling and admin team communications. Nosh relies on WhenIWork, a popular workforce management software, to handle driver scheduling, Slack to handle admin team communications, Zendesk to handle customer complaints, and Google Suite to handle restaurant interactions and customized report generation.

\subsubsection{Limited software interoperability causes frustration within and between stakeholder groups}
Food delivery relies upon multiple parties and disparate pieces of software being able to communicate with each other. In the context of software, this ability to communicate with other pieces of software is called \textit{interoperability}. Mainstream delivery platforms do not typically have to deal with interoperability between disparate pieces of software because they utilize a vertical integration model, where software for each part of the delivery process is built in-house and maintained by a fleet of dedicated software engineers. Nosh utilizes a suite of software to run their business that include DataDreamers (delivery logistics), WhenIWork (driver scheduling), Zendesk (customer relations), Slack (internal communications), and Google Suite (report generation). While these pieces of software are more affordable than a vertical integration model, breakdowns often occur as a result of limited interoperability, frustrating stakeholders. 

Restaurants we interviewed complained that Nosh's ordering system was clunky and required them to operate not only a separate order aggregation system, but also a tablet dedicated solely to Nosh orders. Mainstream food delivery platforms can integrate directly with most restaurants POS and order aggregation systems, reducing friction in the system. As a result of the added friction restaurants experienced working with Nosh, many would shut their tablets off and stop taking orders from Nosh when the kitchen became too busy. Drivers complained that as a result of the complicated order aggregation system, restaurants often forgot important steps such as starting a countdown timer that drivers relied on to estimate when the order would be ready for pickup: \begin{quote}
    "it's hard you know because everybody wants to point fingers so it's hard it's hard to say like if they're actually just like not able to understand how the app works or they just didn't didn't start the order because they you know were lazy or busy or whatever. And they're just like oh like, it wasn't actually my fault, like the App is bad." (D3)
\end{quote}
As a result of confusions caused by poor interoperability, drivers sometimes had to wait for long periods at the restaurant which would then in turn frustrate customers who were given an inaccurate delivery time. Conflict resolution processes with refunded orders was also complicated by the myriad of disparate pieces of software Nosh utilized. While Nosh customer service representatives were trained to give customers whatever it would take to make the situation right, back-end administrators had to manually triage the payment situation according to the type of refund offered and the party whom was responsible for the situation that triggered the refund. The tendency of the system to breakdown sowed distrust amongst stakeholders: "like you can only do so much you can only refund so many orders and  and tell and hold people off for so long to a point where you start to  compromise. You know people don't trust what you're saying" (P3). In an effort to mitigate tensions caused by breakdowns, platform administrators and drivers engaged in additional labor to interface with affected stakeholders, bridging gaps caused by technical malfunctions. 

\subsection{Indie platforms rely heavily on invisible human labor, but this is unsustainable for large-scale contexts}
%distrust of tech; double check with human 
%because tech is constantly breaking down, the people rely less on the technology and more on each other to get work done
%tech for food delivery rather than food delivery for tech (participant quote on this) 
%dispute resolution & troubleshooting is done by phone
%pre-existing relationships supplement tech; people know what restaurants they can trust
While the ability to purchase individual pieces of food delivery service software from the unbundling economy is essential to Nosh's viability, the patchwork nature of the technology stack often results in breakdowns, frustrations, and operational inefficiencies. Platform administrators and drivers act as the glue that holds Nosh's patchwork system together. Through engaging in essential critical infrastructuring, administrators and drivers are able to overcome breakdowns and restaurants and customers feel taken care of because they are being reached out to personally. This human intervention contrasts sharply with the operational logic of mainstream platforms that mediate most interactions through automated systems, a dynamic that frustrates many restaurants and customers. However, relying heavily upon human intervention is not sustainable for delivery businesses that intend to scale-up operations. 

Human mediation plays a critical role in Nosh's operational logic. Platform administrators regularly intervene during the course of food delivery to provide emotional and informational support to restaurants, drivers, and customers. As restaurants started re-opening and became busier with dine-in traffic, drivers would often have to wait long periods of time to pick up their order. This wait time was compounded with the possibility that restaurants did not use the Nosh interface correctly to time the order preparation because. To defuse potentially tense situations between restaurants and drivers Nosh administrators "actually created these templates to send to our drivers that are acting out, getting frustrated with restaurants...say[ing] hey we know you're frustrated but we're all a team here let's work together,  here are some ways that you can you know, deal with those types of situations, you  can walk away, you can contact us, you can you know, take a deep  breath." (P3). The goal of these interactions was to show drivers that Nosh stood behind them and wanted to support their well being on the job. Drivers appreciated these interactions, often explicitly calling out the the unique degree of personal connection they had with administrators during our interviews. 

A healthy skepticism of the capabilities of the technology used further motivated stakeholders to engage in and rely upon human mediation. Drivers developed rich mental models of what food delivery looked like from the restaurant perspective and anticipated where breakdowns might occur, then worked to address those failure points before problems arose. For example, drivers knew that the restaurant-facing UI was complicated and often led to mistakes with timing so they would call up restaurants directly and inquire about order status. Many drivers we spoke to learned how to discern whether the person on the phone worked front of back of house and knew they had to speak with someone from the back of the house if they were to get an accurate estimate for their order. Drivers also took on additional ownership over the relationship with customers, with one driver putting it this way: "I always text my customers so that they know if there's any questions, they can talk to me directly." (D2). While subtle, many drivers we interviewed referred to Nosh customers as "my" customers, introducing a degree of intimacy in an otherwise impersonal algorithmically mediated industry. 

Platform administrators treated the algorithmic systems they used in a paternalistic manner; anticipating that it would breakdown and require human intervention. As one administrator put it: "our job as dispatchers is to skim and identify issues". Administrators played a vital role in manually checking and correcting the logic of the algorithmic system when complications endemic to food delivery occurred. This contrasts sharply with how mainstream platforms operate in that mainstream platforms have little flexibility built in for when situation deviate from what the algorithm prescribes. For example, a driver described a situation where they were delivering multiple orders but a restaurant had forgotten to start the timer on their end, introducing delays into the process. The driver knew that waiting for the order to be completed would result in the order they had already picked up getting cold, potentially displeasing a customer. The driver reached out to Nosh's dispatchers and informed them of the situation. The dispatcher, understanding that these problems arise in food delivery manually changed the delivery routing system to allow the driver to make a single delivery without being penalized for not picking up the delayed order. Platform administrators are trained to manually intervene in the order dispatching system because they know that problems, such as the one described above, do occur. However, training new dispatchers to be ready to make these interventions is time consuming and labor intensive as one administrator put it: "it's a lot of variables and so it's hard to really give  somebody that black and white textbook on how to train for this  position. So it's really just hands on learning that they learn over time." (P1). While the critical infrastructuring that platform administrators and drivers perform result in human-to-human interaction that makes other stakeholders feel respected and encouraged to continue participating in Nosh, it is unsustainable at scale. 

Administrators and drivers engage in critical infrastructuring because the technology they use is prone to breaking down. These critical infrastructuring efforts typically take the form of human-to-human interactions to mediate and patch over breakdowns. Restaurants, drivers, and customers point to these interactions as being integral to their perception of being respected and having agency during the process of food delivery. Platform administrators, however, articulate a desire for the technology to work better in order to support the business operating at a larger scale. As one administrator put it: "you will break the business because there's no way that you can  support the current infrastructure in a big city it's just not gonna work." (P2). This highlights a major tension in designing within the platform economy: at scale, human-to-human interactions that promote sentiments of respect and agency are often untenable. 

Food delivery, like much other gig work, is assumed to be a transactional, sanitized process scrubbed of the messiness of human interaction conducted through slick UI/UX interfaces. However, this perspective of food delivery as an interface market is overly simplistic. There are many moving pieces involved, many humans involved, that have to coordinate their action to make it work. In mainstream models, this coordination is facilitated by complex algorithms and sleek interfaces; however, this does not negate the fact that at the end of the day it is still humans who have to cooperate to make this intricate dance work. In Nosh, the technology stack is not as sophisticated as those built by mainstream platforms, so stakeholders bypass a lot of machine interfacing and instead interface directly with each other. Mainstream food delivery platforms make assumptions regarding the types of communication likely to occur in the ordering and delivery process. They then heavily scaffold these communication processes through tools such as feedback forms or pre-populated complaint forms. Limiting the depth of information that can be transmitted from one stakeholder to another via the platform has ramifications for the type and quality of information transmitted. Since mainstream food delivery platforms are designed with values of scale in mind, they necessarily simplify the kinds of information that can be transmitted. Doing so causes interactions between stakeholders to lose important context and in some ways, sterilizes conversations. Stakeholders in Nosh expressed their frustration with having to shoehorn their concerns into the allowable formats on mainstream food delivery platforms and articulated a desire for lower-fidelty communication technologies that preserved the richness of human-to-human interaction.

Restaurants have recently began articulating concerns about being the "only one [restaurant] on their block not on the platform" ~\cite{sharmaConvenienceDeliveryApps2021}. 

Bottom-up designed infrastructures are socio-technical systems, therefore, they are imbued with the norms and values of their co-creators~\cite{star1996steps}. This makes them potentially more resilient than top-down designed infrastructures as individual stakeholders are able to build a system that meets their needs and values rather than conform to a system where their needs and values are inferred by a removed third-party. 

For example, DoorDash is a mainstream food delivery platform that aims to capture the majority of the food delivery market through its prominent marketing campaigns and vertical integration model that makes it a "one-stop-shop" for restaurants looking to expand their delivery business. Mainstream platforms have significant advantages when compared to ``indie'' platforms; they are able to provide access to a large consumer base and they offer the convenience of managing most aspects of the service ``in-house''~\cite{sharmaConvenienceDeliveryApps2021}. Additionally, since "Indie" platforms are reliant on third-party modular building blocks to assemble their business models, they are often constrained by what is available in the "unbundling" marketplace and face difficulty in integrating individual blocks into a cohesive supply chain. Most mainstream platform economy businesses operate on an ``economies of scale'' logic: the assumption that profit can be achieved in the long run if a domination of the market occurs, allowing for increased production~\cite{zuboff2015big, WhatAreEconomies, kelsoNowThatDoorDash, jordanChallengesLargescaleDigital2017, shermanCanUberEver}. "Indie" platforms are, for the most part, unable to compete with mainstream platforms when it comes to economies of scale. 


The nature of "Indie" platforms, namely their bottom-up designed infrastructure, has been studied in other contexts within the fields of CSCW and HCI (e.g, open source software, postcolonial computing, accessibility studies)~\cite{irani2010postcolonial, Branham2015Invisiblework, robinson2018phenomenological}. We draw upon work examining an theorizing bottom-up infrastructures within the CSCW and HCI literature and extend this line inquiry by applying it to the study of the platform economy. We build upon existing work in CSCW and HCI analyzing the platform economy through studying a new paradigm of platform design: bottom-up designed "Indie" platforms. 

FINDINGS SCRAP
In this section, we first demonstrate that stakeholders defined and operationalized definitions of agency to motivate their participation in Nosh. We then show that stakeholders identified differences in their ability to achieve financial security in mainstream platforms versus Nosh. 

LIT REVIEW SCRAP
These platforms are information infrastructures that support the food delivery industry.

When infrastructures fail to operate in a given context, \textit{infrastrutural breakdowns} occur~\cite{star1996steps}. Studying moments of breakdown is key to understanding the infrastructure at hand and the values which are embedded in them: infrastructres and the values of their designers become visible when breakdowns occur ~\cite{star1996steps}. The source of infrastructural breakdowns can often be traced to the values embedded within the infrastructure itself; the underlying values of infrastructures serve to privilege some users above others~\cite{bowker1994information, Semaan2019}.

In this paper we examine how infrastructural breakdowns within mainstream food delivery platforms \textbf{and} they way in which these breakdowns are handled by mainstream platforms push restaurants, couriers, and customers to indie platforms for food delivery.

Due to the value-ladden nature of food delivery platform infrastructures, situations occur where the design constraints of the platform lead to breakdowns in local contexts. For example, when food delivery platforms program their algorithmic management systems to minimize delivery time, this privileges consumers who can get their meals faster but disadvantages delivery workers who are measured against an accelerating standard for speed, resulting in unsafe driving and navigation techniques~\cite{winnerArtifactsHavePolitics1980, dziezaRevoltDeliveryWorkers2021}. 

Food delivery platforms also exert control over workers’ behaviors by practicing information asymmetries: Goods and colleagues documented delivery companies withholding logistical information like the delivery address to drivers in the initial request which prevents them from making an informed decision about whether to accept the task~\cite{goods2019your}. This information obfuscation hinders workers from making rational informed decisions to maximize their earnings~\cite{veenPlatformCapitalAppetiteControl2020}. The economic toll of using delivery platforms also extends to restaurants. 

Algorithmic management inflicts more than just financial harms for couriers; it also serves as a mechanism for control~\cite{ravenelle2019we,prasslHumansServicePromise2018,richardsonPlatformsMarketsContingent2020}.

%Restauranteurs knew that delivery had become an essential part of their business model, since customers grew accustomed to the service during the lockdown period. However, 
%where they would have more agency over their participation and role in the food delivery process. 
%Restauranteurs characterized this behavior as misleading and deceitful. Restauranteurs  said the mainstream platform's lack of transparency limited their agency as managers. Because they were not treated as equal partners in determining their participation, restauranteurs felt left in the dark by mainstream platforms. 


%Couriers felt similarly to restauranteurs: they perceived that their ability to exert agency over their role in the food delivery industry was better served by Nosh than by mainstream platforms. 

%This human interaction was key to customers’ sense of agency as well. 

%with one customer putting it as such: \begin{quote}\textit{
%    ``I also feel like that one [Nosh] is just a little bit more ethical...through Nosh I definitely felt like restauranteurs, you know don't get as much as many fees taken out and for the couriers like I feel like I trust that the couriers are getting the full tip that I give on Nosh versus like DoorDash and like UberEats. I've heard a lot of like scandals of like you tip and then they take some of the tip before they tell the driver how much you tip so I want my driver to really get the full tip and everything so now Nosh is really the primary one I've used.'' (C1)
%}\end{quote} 
%This perception that Nosh was treating restauranteurs and couriers with more respect in regards to their financial remuneration motivated customers to patronize the service. 

%Restauranteurs that were of a certain size were able to exercise some negotiating power over commission rates, but overwhelmingly, restauranteurs in our sample were small businesses that could not leverage their sales volume to effectively negotiate. 

%, and the cities in which Nosh operated subsidized restauranteurs' (and customers') delivery fees through the platform \cite{CityBoulderBrings}. restauranteurs who participated in Nosh expressed that their low commission rates and other benefits helped them squeeze by during the critical time of the pandemic.

%Participating in Nosh enabled restauranteurs to achieve a level of financial security that was difficult to achieve when participating in mainstream platforms. Similarly, couriers articulated that Nosh enabled them to have a greater degree of financial security than they had with mainstream platforms thus motivating them to join. 

%Nosh's scheduling system provides an interesting contrast to the "log on and drive" models of mainstream platforms. Mainstream platforms emphasize the \textit{flexibility} of delivering for them when advertising to potential couriers. These platforms associate their flexibility with couriers' ability to log on and drive whenever they like. However, this low barrier to entry for couriers often results in over-saturation of the local driver supply which in turns makes it difficult for couriers to actually score work while logged on, according to couriers we interviewed who also drove for mainstream platforms. Gig platforms' reliance on an oversupply of couriers is a well-documented critique of these platform's business models \cite{marshallGigCompaniesFear}. As such,

DISCUSSION SCRAP

in Table~\ref{table:rqsfindings}. 

\begin{table}[]
\label{table:rqsfindings}
\resizebox{\textwidth}{!}{
\begin{tabular}{lll}
\toprule
\makecell{\textbf{Research Question}}                                                                                         & \makecell{\textbf{Findings}}                                                                                                & \makecell{\textbf{Design Implications}}                                                                                                              \\
\midrule
\makecell{RQ1: What motivates stakeholders \\to join an indie platform?}                                                        & \makecell{Agency over participation, \\financial security}                                                                    & \makecell{Build routing and dispute resolution systems \\that make room for agency, \\\\Build governance systems to support \\local models of food delivery} \\\\\\
\makecell{RQ2: What are the capabilities and limitations \\of the sociotechnical infrastructure \\that powers an indie platform?} & \makecell{Poorly integrated technology stack \\frustrates stakeholders, \\\\Human intervention critical \\to addressing breakdowns} & \makecell{Anticipate human intervention \\when building tech systems, \\\\Build tech systems to support \\local contexts not global scale}\\     \bottomrule             
\end{tabular}}
\caption{Summary of Research Questions, Findings, and Resulting Design Recommendations}
\end{table}
Qadri shows that platforms are reliant on \textit{human infrastructures} to step up when they breakdown: couriers know that the platforms assign orders to drivers close to restaurants but that, due to to traffic, they cannot park in front of restaurants so they build apps to spoof their location~\cite{qadriPlatformWorkersInfrastructures2021}. In this case, couriers identified how the platform broke down (it did not account for parking by restaurants to be unavailable) and stepped in (they built applications that allowed them to get orders AND park where it was allowed).


The ability to navigate unexpected obstacles to get back on track can be described as \textit{articulation work}~\cite{straussSocialOrganizationMedical1997}. The articulation work performed by stakeholders is an essential constitutive element of the platform-mediated food delivery process. However, under mainstream models of food delivery the \textit{algorithmic systems} which coordinate cooperative work between stakeholders fail to account for this articulation work. As Star and colleagues note~\cite{starLayersSilenceArenas1999}, the failure to account for articulation work in the creation of computer support cooperative systems may lead to system breakdowns and further inequities. 

Mainstream food delivery platforms are designed in a top-down manner with a rigid conception of what the process entails~\cite{qadriPlatformWorkersInfrastructures2021}. These models often fail to account for the invisible work that occurs behind the scenes. Reflecting on how D2 juxtaposed their experience delivering for DoorDash and delivery for Nosh, we see that the former penalized them for using their discretion to take a route other than the one proposed by the DoorDash routing algorithm. In this case, DoorDash neglected to account for the importance of discretion when designing their routing algorithm. The role of discretion is essential in an industry as unpredictable as food delivery. Restaurants must exercise discretion in determining timing of an order; drivers exercise discretion is picking the best routes for delivery based on familiarity with the locale; and, platform administrators determine acceptable conflict resolution proposals. However, this discretion appears to remain largely invisible to mainstream platform designers. 

Having discretion is key to the articulation work that stakeholders in Nosh engaged in to smooth over infrastructural breakdowns. Platform administrators used discretion to create support systems for drivers during stressful times, and drivers relied on their discretion to time order pick ups correctly in light of inconsistencies with restaurant timing. Nosh trusted and relied upon stakeholders’ discretion to facilitate the process of food delivery when breakdowns occurred. This engendered a feeling of respect amongst restaurants and drivers; they felt that Nosh gave them the agency to be active partners in the food delivery business. While there are good arguments for and against the visibility of discretionary labor when designing computer supported cooperative work (CSCW) systems, it is clear that the role of discretion is essential in performing articulation work~\cite{suchman1995making}. 

The question of how to ascertain the “right” level of visibility when designing CSCW systems is an old one~\cite{starLayersSilenceArenas1999} yet it remains especially relevant today in light of the platform economy. Prior literature shows us that guidelines for coordinating work should have malleability and built-in local control~\cite{schmidt1996coordination}. Drawing on our findings and these guidelines, we put forth the following design recommendations: 

In our work, we recommend that HCI scholars investigate how routing algorithms can make room for user discretion and agency and how to build more human-in-the-loop support systems. These recommendation would not be actionable in the context of a business like DoorDash  because it does not align with the company’s business model and economic incentives. DoorDash seeks to create a monopoly over the supply and demand of food delivery services. Most mainstream platforms operate with this logic~\cite{bomeyDoorDashGrubHubUber,carballasmichowskiRidehailingDoomedMonopoly2018,luWillFoodDelivery}. The infrastructure of these mainstream platforms is inextricably linked with the economic and political contexts in which they operates; they shape and are shaped by the political economy of the platform~\cite{star1996steps}. As we illustrate in Figure 1, the economic structure of mainstream platforms rely on funding from venture capitalists and individual shareholders. These investors base their valuation of the platform on its potential to return profit and the ability to return profit relies on massive growth and monopolization~\cite{srnicek2017platform}\footnote{Platforms like DoorDash, UberEats, and GrubHub operate at a loss, as their yearly SEC filings show. However, they continue to garner investment because promise investors future of market monopolization where they gain control over food delivery in a given region and increase the "rents" or price of participation}.   

Mainstream platforms must therefore optimize for \textbf{scale} and thus they design their technology with scalability in mind~\cite{luuPrinciplesBuildingML2022}. Our restaurants and couriers identified the generic, automated treatment they received from mainstream platforms as a primary motivation for seeking out alternatives for food delivery. They sought human connection, or at least a sign that the platform cared about their well-being as workers and business owners. An inability to question, let alone contest, the outputs of the algorithmic systems mainstream delivery platforms use to organize the process of food delivery left restaurants and drivers feeling like they lacked agency. While Nosh the parent company, would like to one day attain scale (e.g. have multiple local Nosh hubs operating), the goal of each individual hub is \textbf{not} to achieve scale or monopolization of the market. Thus, they are able to incorporate human intervention as a cornerstone of their operations.  


where operations were functioning without an intention to scale, restaurants and drivers felt seen because they had the ability to reach out and get help from someone who would understand their situation. After all, you cannot negotiate with an algorithm the same way you can negotiate with a human. Nosh's model facilitated human intervention effectively because it was 

In doing so, automation is a natural replacement for slow human decision making because it is much quicker (and cheaper) to assume that an ML model is the source of ground truth for routing than it is to hire a human agent to mediate the dispatching and routing process. Thus recommending to a mainstream platform like DoorDash that they should enable and incentivize human intervention in their platform would be nonsensical. In line with a proposal put forth by Jackson and colleagues, we urge HCI scholars designing systems for the platform economy to consider the ``policy knot" at hand~\cite{jacksonPolicyKnotReintegrating2014}. 

Considering the co-constituitive relationships between policy, design, and practice is essential for HCI scholar to disentangle how designs we propose may go on to shape policy that allows for harms to be enacted in practice~\cite{jacksonPolicyKnotReintegrating2014, alkhatibLiveTheirUtopia2021a}. HCI scholars have played a pivotal role in shaping the platform economy; many of the innovations that allow for distributed systems of work emerged from the CSCW and HCI fields~\cite{khovanskayaToolsManagementAdapting2019}. This is not to say that HCI researchers are the sole reason why gig workers experience negative impacts when participating in the platform economy; legal frameworks often supports socio-tecnical arrangements that allow for exploitation~\cite{bodieLawEmployeeData}. Focusing in on the relationships between policy, design, and practice gives researchers the opportunity to reflect on questions such as: Should this design be implemented? And what social, political, and economic pre-requsites are needed to support the intended function of this design?

In our study, stakeholders took the risk of participating in a relatively untested food delivery model because the human intervention facilitated interactions that engendered agency and respect. As a business, Nosh knew it could rely upon human intervention to step up when technology broke down. Thus, we put forth design recommendations advocating for the incorporation and incentivization of human intervention in technical systems supporting food delivery. However, Nosh was able to rely on human intervention because their business model was centered around its presence. Through their hub-and-spoke model, each geographic location had its own platform administrators and drivers that supported the local network of restaurants and customers. These local workers had rich knowledge about the area that enabled them to exercise discretion effectively. Thus, Nosh’s localized business model was essential in supporting and incentivizing the human intervention that stakeholders prized. In a model like DoorDash, where there are no localized hubs that have local staff dedicated to supporting that one community, it would be difficult to operationalize, let alone, incentivize effective human intervention. 

This is all to say that when HCI researchers make design recommendations they must examine the contexts in which their designs will be deployed. If we are to put forth design recommendations that are intended to mitigate harms and uplift users, we must consider if those recommendations are even actionable under the contexts in which users operate. HCI researchers interested in designing for the platform economy must investigate how existing business models and economic incentives hamper the efficacy of their proposals. In doing so, we may be able to move (backwards) to a time where, as field,
% We examine the advantages and downfalls of bottom-up designed infrastructures in the platform economy through an in-depth case of an "Indie" food delivery platform operating in Northern Colorado and answer the following questions:
% \begin{itemize}
%     \item RQ1: What problems in mainstream platforms motivate stakeholders to participate in "Indie" platforms? % problems
%     \item RQ2: What tools do stakeholders use and what are the affordances and challenges that these tools present? %unbundling
%     \item RQ3: How do indie platforms mediate interactions between stakeholders?
% \end{itemize}

INTRO SCRAP
%Most restaurants currently use mainstream platforms to conduct their delivery business. However, these platforms maintain near-monopolistic control over conditions of participation which leaves not only restaurants, but also other stakeholders in the food delivery industry with little negotiating power \cite{griswoldAreFoodDelivery2022, thompsonHiddenCostFood2020}. 
% Although, HCI scholars have documented the detrimental effects of mainstream platforms \cite{}, to our knowledge, no research has explored  “indie” platforms. 
%Mainstream platforms are designed with a top-down approach: a small group of centralized planners at the company make decisions about the design for end-users. Given their business model that aims for maximum market capture, this approach is logical as it allows them to design for the majority of people and situations by catering to the lowest common denominator. However, in food delivery edge cases that confound systems built for the lowest common denominator are common: traffic delays cause missed delivery timeframes, understaffed restaurants forget to communicate with delivery apps, orders arrive missing items. When breakdowns inevitably occur, drivers and restaurants often bear the brunt of the negative impacts \cite{joeguszkowskiFoodDeliveryMishaps, hobbsDoordashDriverWhy2017, pedancoWhatWhenThirdParty2018 }. Given the heavily automated nature of mainstream platforms, there is little room for restaurants and drivers to negotiate and plead their case with a human customer service agent. Seeking a more human-centric approach that understood the inherently unpredictable nature of food delivery, restaurants and drivers began turning to indie food delivery platforms. 
%Many restaurants now rely on mainstream platforms, such as UberEats, DoorDash, and Grubhub, for access to their large userbase. These platforms charge commission rates of around 30\% per order, which puts pressure on restaurants' already thin profit margins \cite{DeliveryAppsGrubhub2021, thompsonHiddenCostFood2020}. Restaurants must decide whether to pass on these higher costs, and risk of losing price-conscious customers, or subsume the costs themselves, reducing their already-thin profit margins. %Some restaurants attempt to pass on these higher costs to consumers, but doing so could result in losing price-sensitive customers. Because restaurants are reliant on mainstream platforms for their large userbase, they have limited ability to contest prohibitively high commission fees. 

LR SCRAP
Food delivery has been around since the 1890s: dabbawala, a food delivery system that emerged in colonial India was among the first instances of this~\cite{gentUnsurpassed125yearoldNetwork}. Food delivery platforms are a much more recent phenomena. 

\subsubsection{Critical infrastructuring to repair breakdowns in the platform economy}
When infrastructural breakdowns occur, users often engage in acts of \textit{critical infrastructuring}: simultaneously critiquing and patching existing infrastructures with supplemental support systems~\cite{britton2019mothers}. Britton and colleagues illustrate this process in their analysis of how new mothers in the U.S, facing a lack of infrastructural support after birth, piece together disparate pieces of existing infrastructures including Facebook, local mom support groups, and available medical care to construct a cohesive support system~\cite{britton2019mothers}. Gig workers engage in acts of critical infrastructuring as well: they develop and use gray-market mobile applications---unofficial mobile applications that enable order filtering and location spoofing---to facilitate the delivery process and build community-run e-bike charging stations~\cite{dziezaRevoltDeliveryWorkers2021, qadriPlatformWorkersInfrastructures2021, qadriWhatNetworkInfrastructures2021}. In developing these bottom-up support structures, gig workers "become the hidden scaffolding of the platform"~\cite[pg.33]{qadriPlatformWorkersInfrastructures2021} and can counter the infrastructural breakdowns that occur in platform labor. In some cases, people create entire parallel infrastructures to compensate for chronic breakdowns in existing infrastructure~\cite{semaanTechnologymediatedSocialArrangements2011}. 

BLAH BLAH THESE PLATFORMS ARE RISKY & TECHNOLOGICALLY INFERIOR SO WHY DO PEOPLE JOIN THEM? 
WHEN THEY JOIN THEM HOW DO THIS MAKE THIS TECH WORK?

\subsection{What is Infrastructure?}
Infrastructure refers to the foundation that underpins any-large scale system; society is dependent upon these systems to conduct everyday activities~\cite{edwards2003infrastructure}. For example, roads are infrastructures that people rely upon to conduct their everyday routines like getting groceries. While infrastructure is typically conceived as physical (\textit{e.g.}, roads), information communication technologies are also infrastructures~\cite{hanseth2010design}. These information infrastructures are comprised of digital platforms that allow users and communities to engage with the information systems~\cite{hanseth2010design}.
Information infrastructures have become integral to how people communicate with each other and obtain goods and services in the modern economy. Infrastructures are socio-technical systems, they shape and are shaped by social practices ~\cite{edwards2003infrastructure}.  They are also value-laden imbued with the values of their designers~\cite{star1996steps}.  
Langdon Winner famously demonstrated how roads can be imbued with the politics of their designers: he highlighted the design of tunnels on the highway to the coast that were just tall enough to allow cars to pass through but not city buses which were primarily used by people of color~\cite{winnerArtifactsHavePolitics1980}. When the values of designers do not align with the values of users, friction occurs that can result in breakdowns. Examining when infrastructural breakdowns occur allow us to surface the values of designers and users.  

\subsubsection{When infrastructures breakdown, people repair them}
When infrastructures fail to operate in a given context, \textit{infrastrutural breakdowns} occur~\cite{star1996steps}. Studying moments of breakdown is key to understanding the infrastructure at hand and the values which are embedded in them: infrastructures and the values of their designers become visible when breakdowns occur~\cite{star1996steps}. The source of infrastructural breakdowns can often be traced to the values embedded within the infrastructure itself; the underlying values of infrastructures serve to privilege some users above others~\cite{bowker1994information, Semaan2019}. For example, Britton and colleagues identify how maternity healthcare infrastructures break down after delivery of the baby because social and medicare resources are centered around the needs of the baby and not those of the mother. In the face of this breakdown, mothers engaged in repair work: they developed \textit{ad hoc} social and informational support networks to meet their needs~\cite{britton2019mothers}. Repair work is typically invisible, unseen by those who are unaffected by the breakdown. However, it is critical to examine these acts of repair to understand when and why the original infrastructures failed in order to inform design recommendations for improvement.% We build upon infrastructure literature in our paper in two ways: First, we demonstrate that food delivery platforms are imbued with the values of their designers and that value misalignment between designers and users drives the adoption of new, alternative platforms. Second, we identify how the essential repair work done by users makes a strong case for designing these platforms in ways that value, not penalize, human intervention. 


% In recent years, a cottage industry providing the modular building blocks needed to ``\textbf{unbundle}'' the platform economy and build independent platforms from the bottom up has emerged (see Figure~\ref{fig:unbundling} below)~\cite{wangCommissionfreeOnlineOrders2020}. This cottage industry provides tools such as website building and hosting services, point of sales (POS), white label ordering software, order aggregation, and delivery~\cite{wangArmingRebelsFood2021}. Indie platforms are an example of infrastructures built from the bottom-up in the platform economy; stakeholders unhappy with existing top-down designed platforms piece together the necessary building blocks to build a platform that conforms to their needs and values and offers an alternative to mainstream platforms. In contrast, mainstream platforms use a vertical integration model for their technology: they provide the customer interface, take and transmit orders to the provider, handle transaction processing, facilitate delivery, and adjudicate disputes. However, a vertically integrated and centralized model may not offer the same opportunities for localized human intervention to address breakdowns. The piecemeal nature of technical infrastructures that indie platform build necessitates human intervention because, sometimes, the individual pieces of software cannot "talk" to each other and a human must serve as a mediator.  



%Roads are infrastructures that are typically designed by city planners who dictate what neighborhoods will be serviced and what types of vehicles can traverse them. While roads may seem like a value-neutral system,
%\input{table.tex}
% Restaurants 
%   Dispatchers via phone for dispute resolution; much less frustrating than being routed through the corporate version of customer care with mainstream platforms because they get to talk to someone local who understands their problems 
%   Drivers in person, they are familiar with & comfortable with drivers - they know who some of them are & they form a bond/community with them 
% Dispatchers
%   Restaurants via phone to give them tailored assistance, discuss wait times & delays, troubleshoot problems - novel because there are no (known) human dispatchers at mainstream platforms, an algorithm can only offer up to a certain degree of help 
%   Drivers via phone & chat to help them troubleshoot, start the day off with a “how are you”, “Are you ready to work” - humanizes the interaction 
%   Customers via phone to update them when an order is late/delayed or something goes wrong; asks them “what would make this right for you”
% Customers
%   Dispatchers: dispute resolution
%    Drivers: check-in with orders, give directions 
% Drivers  
%    Dispatchers: troubleshooting, check-ins 
%    Restaurants: verify if orders are ready for pick up  
%   Customers: check in with them via phone & chat “my customers”/ “my regulars”  
%   Drivers: helping other drivers, giving tips, watercooler chat 

%restaurants interact with platform via telephone - enables rich communication & preserves human-to-human interaction
%drivers interact with dispatchers through the chat & via telephone - still talking human-to-human allows them to transmit concerns, get dynamic feedback, exert agency 
%customers interact with platform via telephone - helps them feel human connection & like a valued customer

%R6 communication on the phone...collaborative versus 
%what are they using ...foster sense of community ,, what interactions

% Rapid problem solving based on pre-established relationship: 
% R6: For Nosh, it's it's the, I can tell you that the best things about Nosh, that I love the most is their their message and the fact when I pick up the phone and I call, because I have a problem I get an answer from somebody here locally and they know my business they most often because of my relationship at Nosh, they know me. So I can problem solve very efficiently.

% Quality human services (hospitable attitude)
% R6 [speaking about his driving experiences]: you're one call away from a local person picking up and giving you answers you know, “oh no the House is downstream a little bit further, the addresses are out of order.” It's crazy how good and effective they are and how knowledgeable and friendly and what wonderful staff they put together.
% P4: When when they call us as someone who's locally, as someone who's got a caring voice and actually care about what just happened to their order and what's wrong with their frustrations, are they will fix it on the phone with you in that moment. That is just unheard of from the other delivery services.

% Quality human service (thorough problem-solving, identifying where in the delivery chain the error occurred and resolving it judiciously among actors involved )
% R6: I can, I can think of you know, a handful of situations, you know as a driver and as an operator where let's say we [the restaurant] miss part of the meal for a delivery. Well then we should pay for that and [Nosh will] let us know, hey i'm sorry, but you missed the salad in this meal so we're deducting this off of your sales for the week.” If it's something in the respect that maybe their driver got lost or did something incorrectly and that meal didn't get delivered or got delivered very late, but I [the restaurant] had done everything right because they can see when the meals were picked up and stuff like that, I'll never hear from them. They'll send the guest a gift card to Nosh for a free meal or free delivery or something like that, so they really dissect the problem. If I have those same two problems with grub hub or doordash, they will typically most of time expense the entire meal off and charge me for it on both case. There's no discussion.


\subsection{What tools do stakeholders use and what are the affordances and challenges that these tools present?}
% multiple software, frictions...drivers use phone, tablets (humans need to keep watch) 
% R6: Our technology has to improve. Without better technology, that's that's really the only thing getting in our way you know it's it's too hard too difficult to operate and grow the business from our staff side because they're managing technology, one of the credos that I speak in my restaurants, is, I want to clear away all of that stuff that they manage and just really put them with guests, you know I want them managing staff and guess I don't want them managing all the other pieces that happen. I don't want them managing with delivery service on our side. I want them to be able to turn it on, know that it works. And let it do its job, so they can go do their job, which is creating guests connections delivering fantastic food to our guests, and I want Nosh to be able to do the same thing.


% Pricing difficulty: R6: An update of my pricing with nosh, but I have to do that… i'll have to involve two parties, I have to call Nosh, make all my changes to my menu so somebody at Nosh will input those changes into the website. And then I have to call Chowdy and have them take that information and upload it into their system, so it matches the Nosh website. Even if you're off by one character in a sentence, it will not match, and it will not load. It's very… it's a cumbersome process, so my pricing right now is actually lower on my delivery service than it is in my restaurants, because of how many hours it's going to take me to work on this and, as you know, restaurants tours our time is gold.

% platform operators: multiple notifications arriving at too centralized a place, necessitating human delegation 
% P4: ...whoever can figure out how to streamline notifications is going to be very, very rich. I mean, just for example, for my calendar, I get emails coming to my phone all day. I need to see 25% of them, but I get every single email. To get a little more direct with your question, being able to integrate all these different notifications: driver applications, incoming orders, restaurant applications, being able to integrate them into one website application and streamline them to different people through the workflow would be incredible...There's a lot of time I spend in passing information along to the correct people, delegating projects, setting things up, that's part of my job, but I will admit it does take a lot of time.

% \subsection{Local Food Delivery is Built on a Patchwork of Technology}
% Food delivery is a logistically complex operation that requires the synthesis of three primary components: the placement of the order by a customer, the reception and fulfillment of the order by a restaurant, and the delivery of the order by a driver. National food delivery platforms, such as DoorDash, have sophisticated in-house microservice architectures that manage these three facets of delivery relatively seamlessly \cite{celozziHowDoorDashTransitioned2020}. However, such architectures are resource intensive and require teams of software engineers to build and maintain. Local food delivery services, like Nosh, face resource and financial constraints and thus turn to available white-label\footnote{software packages developed by a separate company that another company can license and apply its brand name to} software to piece together the requisite parts of their intranet. 
% %do we want a figure of the Nosh intranet/system? 
% %pull quotes about technology ecosystem used by stakeholders
% %%each stakeholder has to use disparate pieces of technology and patch them together to make food delivery happen; this is frustrating and difficult but given resource constrains & commitments to local models, it is something stakeholders are willing to do
% %%patchwork of tech hampers ability to scale model because it is so dependent on human intervention & local knowledge to compensate for its failings
% Food delivery requires Local food delivery platforms rely on an agglomeration of white label technologies and administrative software.  
% \subsection{Human Intervention is Critical in Local Food Delivery Model}
% Local food delivery models are lacking in technological sophistication and are often using pieces of software that breakdown on them and frustrate stakeholders. In order to patch over gaps that occur, Nosh has to rely on human intervention from all stakeholders. We find that each stakeholder intervenes in the system in unique ways that make this model of food delivery viable. 


% %discuss how each stakeholder performs their human intervention & what that does for the food delivery process as a whole --> restaurants calling & manually updating their menus, dispatchers 
% Dispatchers are the nucleus of the operation, overseeing the complete cycle of an order and solving issues along the way. While Nosh's dispatching algorithm assigns orders and routes automatically, they are rudimentary '''' and dispatchers often intervene in certain situations to assist drivers. 

% For example, the algorithm has issues with determining the lineup of delivery orders within a "stack" and as a result, provide inefficient routes for drivers. In these instances, dispatchers can intervene to rearrange the orders to streamline the routes for drivers and cut down the waiting time for customers. Their deftness imbues Nosh's rudimentary algorithm with the flexibility and reasoning to accomplish more complicated tasks. 

% D5 illustrates what an efficient route designed by human dispatchers would look like: "And they will try to create a route that you know, will create a loop, so that you can...go from the restaurant to customer A, B, C D and E restaurants back again. Or you know, just a route that makes sense, like you might be picking up from three restaurants, but you'll be like pick up restaurant A, pick up restaurant B, drop off restaurant A, pickup restaurant C, drop off restaurant B."

% This '''' is built into Nosh's delivery systems. Some drivers catch on to the algorithm's shortcomings and supplement it with requests to the dispatcher. 

% %check this quote so as to not undermine --> D5: um I do think the algorithm sometimes make stupid choices..but again, that is because it is not a human...So I think for some drivers they might perceive that the AI as being very stupid...They don't realize that we assume that they're going to tell us that it's doing something stupid and then a human can fix it.

% %D5: So again, human intervention and they know that I can handle stacks that other drivers can't.

% Drivers also compensate for technological shortcomings 
% -by contacting restaurants to ensure the order is received 
 %D3: As far as like stressful, just the way the Apps integrated. It's just not not very well like managed or designs and so even like I just find myself calling restaurant, a lot when i'm driving which, like stresses me out because then I have to focus on talking to them and driving in traffic and stuff and. So that’s kind of a little stressful yeah.




% -by contacting customers directly using their personal number to inform of issues or to confirm pickup
% -


% Customers compensate by going to the restaurants and looking at the dishes bc nosh has no pictures
% Restaurants calling & manually updating their menus

% P1: In my role you're constantly putting out little  fires everywhere



% %P4: When they call us as someone who's locally, as someone who's got a caring voice and actually care about what just happened to their order and what's wrong with their frustrations, are they will fix it on the phone with you in that moment. That is just unheard of from the other delivery services.

% %R6: You know, delivered later did something wrong, whereas Nosh, you know they they solve the problem you know they'll help the guest work through it and it's sometimes it's a you know it's a it's not always just comping the meal, it's doing something else for them, you know, a free delivery on their next time you know they really research, the problem and seek to be better.

% %P3:  would say that that set us apart from them in terms of our customer services local they can talk  to people we've got boots on the ground here that's where we're  different but. 


% %%human intervention smooths over seams in technological patchwork
% %%human intervention increases trust in system
% %%human intervention is critical differentiating factor between national gig platforms & local food delivery model
% %%communication is key --> need to be able to communicate with humans to solve problems
% \subsection{Investment in and Accountability to the Community}
% %%Local models differentiate themselves by grounding their values in a community
% %%Community investment holds the platform liable to those stakeholders meaning that it will be liable to the community 
% %%hiring local sets Nosh apart

%R7 And then grub hub is the opposite there's no human that's been in regular contact with us and it's just like I think there's somebody assigned to a group, but that role changes and it's just like a new email person.

%In the on-demand delivery economy, participation in mainstream platforms comes at the cost of anonymity; a loss of an actual stake in how the process unfolds 
% Mainstream platforms are designed in a top-down manner; engineers, managers, and designers at corporate offices dictate how the platforms are built. As infrastructures, mainstream platforms are imbued with the values of their designers \cite{star1996steps}. This can result in friction when users do not have the same values as designers. For example, mainstream platforms are designed to operate at economies of scale, meaning that they optimize for the lowest common denominator. This manifests in the form of generalized, de-personalized customer service for both consumers and restaurants as well inflexible algorithmic dispatching models for drivers. For restaurants participating in mainstream food delivery platforms, they are simply one of many faceless food suppliers that the platforms contract with and as such are treated in a de-personalized manner. R1 articulated this feeling of de-personalization as evidence that mainstream platforms did not care about their restuarant partners as individuals saying: "I firmly believe that [mainstream platforms] don't have the  restaurants' best interests at heart, so they were not incentivized in  any way to help us". R1 went on to explain that their experience with restaurant support services at GrubHub, a mainstream food delivery platform, indicated to him that despite messaging from platforms that they valued their restaurant partners their actions said otherwise. 

% \begin{quote}
%     [GrubHub's] restaurant success team is speaks in  generalities and platitudes and garbage nonsense that I just can't  handle.  We're waiting on a on a month long payment, a month long deposit, that never got sent to us back in March and I've been in  contact with them, since May to try to get \$5,000...payout from one store.  And, just like a constantly...revolving door yeah of customer support. I've never...been able  to have a support structure that's longer than two  interactions with any one account manager. So that's been a nightmare. (R1)
% \end{quote}

% Similarly, R6 described their experience working with GrubHub and DoorDash's restaurant partner helpline as being non-responsive to the concerns they articulated.  
% \begin{quote}
%     "doordash and grub hub, it's really all service related, you know if you don't call within certain hours of the day, you get routed to a call center with somebody who can’t help your question. Instead of them solving problems for guests, they don't ever solve a problem for a guest, other than just take money off the bill which affects my bottom line, even if it's their mistake their driver delivered later did something wrong."
% \end{quote}
% Mainstream platforms, valuing economies of scale, are unable to address every edge-case by design; the help they are able to offer is generic by necessity. In food delivery, where variability and uncertainty are endemic (e.g. traffic delays an order, an item is forgotten in a customer's meal, etc.), such generalized solutions do little to actually address the problems at hand.


%R1: yeah and it's like Okay, this is, you are, you are  outclassed in a huge way.yeah and you can't convert there's no way you can  take revenue really substantial amounts of market share away from  these companies that are effectively tech companies that you know. they're advertising companies that have a tech arm  that also happened to facilitate food delivery. 
% R2: They [the customers] don't know that the restaurant is paying a 30% Commission to be on the platform to be found yeah those are huge fees and the consumer is misled. 
% D6: nosh started out, they have like this crazy awesome story that started out as a small…The guy who started it started out someone who worked for grub club. yeah like Grubhub was like taking over and screw people over in town or something, and he, like made his own grubhub, which was nosh.
% R6: More of what I like to see you know more level playing field against companies that are just so big and i'd like to see you know more local opportunity for people to to win."
% R2: You know the restaurant partners' success is their [Nosh's] own success. 
% D6 [talking about Ubereats] "tips [were] going missing"
% R6: doordash and grub hub, it's really all service related, you know if you don't call within certain hours of the day, you get routed to a call center with somebody who can’t help your question. Instead of them solving problems for guests, they don't ever solve a problem for a guest, other than just take money off the bill which affects my bottom line, even if it's their mistake their driver delivered later did something wrong. Whereas Nosh, you know, they solve the problem, they'll help the guest work through it, and it's sometimes it's not always just copying the meal, it's doing something else for them, you know, a free delivery on their next time. You know, they really research the problem and seek to be better.
%P3:  think they've stuck with us because they like the Community  aspect of it. Just the local, especially in Fort Collins people  really think local here I don't know that it's carried into some of  the other cities, but here, where I live, it's just sort of a  mentality that people adopt 
%locality
% R6: Of course Nosh, their messages great. You know, local restaurants that's something that we believe in being a local restaurant group as well.

%Across all stakeholder groups a common theme emerged around wanting to ground the food delivery process in the local community. 

%the code for this table is also in the table.tex file. You can delete this code and insert the table anywhere you want in the paper. You can also use the command "\input{table.tex}" to insert the table directly from that file.

% main theme here is that communication w/mainstream platforms is overly formatted & too technologically mediated - this does away with a lot of the richness that human-to-human interaction has and that is important for something as dynamic & involved as food delivery
% On  

% Indie platforms are an example of infrastructures built from the bottom-up in the platform economy; stakeholders unhappy with existing platform options develop, assemble, and piece together requisite parts of the platform to create their own alternatives that better meet their needs & values; these platforms rely on an ecosystem of white label software and community support to function. They differ from mainstream platforms in that they are not monolithcally designed; they are built from "lego blocks" that allow for more flexibility (financial & service wise)
%There are downsides to Indie platforms; nonetheless they have grown in popularity & prevalence
%These downsides to indie platforms & the underlying concept of indie platforms as a whole has been studied in other contexts in CSCW/HCI (postcolonial computing, OSS); we borrow from these research areas to better understand the phenomena of indie platforms and extend the literature in these spaces by deploying these theories & learnings within a new context  




%missing something about the independent platform space & show that there is not much academic research on indie-platforms & show that hey there is something here & it needs to be researched more --> review Elizabeth's hand holding sentence comment 
%confusion about postcolonial computing section --> might make paper overly broad
%bricolage could be part around emergence of indepedent platforms; make section on independnt platforms 
%existing lit reviews do not focus on how community contribute to gig economy; because this is a gap that exists in the lit we try to address this gap (most lit talks about problems & solutions from worker perspectives)
%try to introduce RQs in lit review 

%%%%DUMP
% \subsection{Addressing infrastructural breakdowns in food delivery through bricolage}
% When faced with infrastructural breakdowns, users engage intentional, bottom-up construction of supplemental support systems to meet their needs \cite{star1996ecology}. This construction of supplemental systems, referred to as \textit{bricolage} in design literature, occurs when users piece together multiple disparate pieces of existing infrastructures to create a patchwork system that meets users needs \cite{EriksonJarrahi2016, erickson2014more, vallgaarda2015interaction, jackson2014RethinkingRepair}. Britton et. al illustrate this process of bricolage in their analysis of how new mothers in the U.S, facing a lack of infrastructural support after birth, piece together disparate pieces of existing infrastructures including Facebook, local mom support groups, and available medical care to construct a cohesive support system \cite{britton2019mothers}. Gig workers engage in acts of bricolage as well through their development and use of gray-market mobile applications that facilitate the delivery process and the creation of community run e-bike charging stations \cite{dziezaRevoltDeliveryWorkers2021, qadriPlatformWorkersInfrastructures2021, qadriWhatNetworkInfrastructures2021}. In developing these bottom-up support structures, gig workers "become the hidden scaffolding of the platform" \cite[pg.33]{qadriPlatformWorkersInfrastructures2021} and are able to counter the infrastructural breakdowns that occur in platform labor. Thus when gig workers engage in acts bricolage they are able to achieve "fleeting, nonstable, even ephemeral moments of alignment" \cite[~p.277]{vertesi2014seamful}.

% However, acts of bricolage are typically done after the fact, when the harm perpetrated by an infrastructural breakdown has already been realized by users. Due to the top-down, centrally designed and administrated nature of food delivery platforms, breakdowns are bound to occur when these technologies are deployed in contexts different from those in which they were developed \cite{qadriPlatformWorkersInfrastructures2021}. As a remedy to the brittle nature of top-down designed infrastructures, critical design scholars have proposed new paradigms of bottom-up infrastructuring that allows for users to co-construct systems alongside designers and imbue local values and knowledge that support \textit{situated action} in localized contexts \cite{suchman1987plans, irani2010postcolonial}. 

% \subsection{Postcolonial computing as a guiding paradigm for designing gig work platforms}
% Technology is is rarely bounded by geographic borders, it is often transplanted into contexts in which it was not designed \cite{irani2010postcolonial, qadriPlatformWorkersInfrastructures2021}. Incongruencies between values of designers and users of technology are bound to occur \cite{das2021jol}. Postcolonial computing scholars ... 
% During the COVID-19 pandemic, gig work platforms provided vital infrastructure for restaurants to continue their business even as brick and mortar locations closed \cite{mckinsey}. Restaurants became reliant on platforms like DoorDash, GrubHub, and UberEats as they shifted their business models to take-out only to cope with shutdowns brought on by the pandemic [\cite{mckinsey}, \cite{sharmaConvenienceDeliveryApps2021}]. Food delivery platforms provide the means for restaurants to reach and expand their customer base, coordinate delivery with drivers, and process payments. In exchange, these food delivery platforms extract a commission, reported to be between 15\%-30\%, for each order placed through their service  [\cite{follmerDeliveryAppDilemma},\cite{DeliveryAppsGrubhub2021}, \cite{ProductsPartnershipPlans}]. High commission rates exert pressure on restaurants' already thin profit margins, however, restaurants feel beholden to food delivery platforms as they are entirely reliant upon their infrastructures to facilitate the delivery aspect of their business model \cite{sharmaConvenienceDeliveryApps2021}. In addition to squeezing restaurants with high commission rates, food delivery platforms engender precarity for delivery workers     
%food delivery platforms are an example of how gig work platforms provide essential infrastructure, especially in light of the covid-19 pandemic 
% Layout: The problems with gig platforms are x, y, z. People have addressed these problems by doing by a, b, c. In this paper we study D, a novel way of dealing with problems x, y, z.

% % \subsection{Gig Platforms and Their Problems}
% % What is gig work? gig work has been studied in CHI in these ways) – here try and focus on some papers that reveal the central problems of gig work you discuss in the next section
% % a. Leading question: what are the potential problems of gig work?
% % \begin{itemize}
% %     \item They engender precarity via \begin{itemize}
% %         \item Low levels of control that workers have over wages and working conditions (due to algorithmic control)
% %         \item Lack of regulation (due to worker classification)
% %         \item High employment insecurity (due to worker classification)
% %     \end{itemize}
% %     \item They breakdown in real-world contexts (they depend on algorithms to function whose assumptions don’t always hold when unanticipated events occur) \begin{itemize}
% %         \item Make assumptions about information necessary for tasks (Ghost Work Mary L Gray)
% %         \item Give incomplete information/information that doesn’t fit actual situation at hand (difficulty with delivering to apartments w/inaccurate geolocation data) 
% %         \item Don’t allow for edge cases/variation in the labor process (penalization for delays caused by traffic)
% %         \item Leading question: What are the ways that people work to solve some of these problems?
% %     \end{itemize}
% % \end{itemize}

% \subsection{Gig work is associated with precarious labor conditions}
% In recent years, gig work has achieved mainstream visibility through ride-hailing services like Uber and Lyft, as well as platform-based food delivery services like Grubhub and UberEats (Hajal & Rowson 2021). These work arrangements are often temporary, based on project-to-project compensation, and are flexible in work hours, location, and work continuity (Watson et al. 2021). 

% The COVID-19 pandemic has accelerated the global digital gig platforms industry, which has seen a five-fold growth in the last decade. However, the crisis has also revealed the human consequences of the systemic precarities within gig work (Ravenelle, Kowalski & Janko 2021, Bellon & Balu 2020). These included limited health and social benefits, low job security, inadequate regulatory protections, and workers’ inability to control wages, hours, and working conditions \cite{Vosko2006}.

% During the health crises, many app-based companies failed to provide their gig drivers with adequate protective and sanitation equipment despite the high exposure rate of their front-line occupation (Beckman et. al 2021). 

% These health risks are exacerbated by the absence of a social safety net for workers. In the 2017 U.S. Bureau of Labor Statistics Census, all independent contractors needed to seek forms of insurance outside of their gig work provider, and many who cited gig work as their primary source of income lacked retirement plans. 

% Job insecurity, or the perception of a volatile working relationship, also features prominently in the gig economy, as workers are unable to anticipate declines in the amount of work offered to them (Vosko 2006). When demand for rideshare services dropped during the COVID-19 pandemic, gig drivers struggled to generate income (Hossain 2021). Their classification as “independent contractors” also barred them from receiving unemployment benefits, forcing many to continue to work for long hours in unsafe conditions (Thorbecke 2020).  This can lead to increased risk of housing loss, food insecurity, as well as increased psychological tolls (Glavin & Schieman 2022). 

% Wage precarity is also inherent within the model (Ravenelle 2019). In recent months, rising gas prices as an indirect result of the 2022 Russian invasion of Ukraine presented a financial burden to many gig drivers (Browning 2022). 

% %% Do we want to make more clear that these precarities vary among gig professions (drivers vs renters) as well as those that are using this as their primary source of income vs not (in Glavin & Schieman 2022)
 
 
% \subsection{Reactions to Problems Endemic to Gig Platforms}
% One thing less explored in this context is smaller, independent platforms. Indie platforms are defined as a, b, c. They’ve been studied in these contexts, however less is understood about how stakeholders interact with and use the affordances of these smaller platforms. In this paper, we draw on these studies to address these research questions

% Infrastructures
% Scholarship centering bottom-up infrastructuring often points to the sociotechnical nature of infrastructure, namely the fact that infrastructure is imbued with the values of those who co-construct it. Thus, when communities engage in bottom-up infrastructuring, they are able to imbue this infrastructure with values that reflect community values and norms. This makes bottom-up infrastructures potentially more resilient, flexible, and appropriate for communities in which norms and values are not static. \par

% \begin{itemize}
%     \item People draw upon other tools to help them do their jobs and improve their working conditions (e.g. critical infrastructuring) \begin{itemize}
%         \item Building networks to share information & support (Ghost Work)
%         \item Building physical infrastructure to provide necessary support (building bike charging stations)
%         \item Building & using third party applications to address breakdowns in gig applications (gray market apps built & used by delivery drivers in Indonesia to spoof GPS locations, queue orders more sensibly etc.) 
%         \item Building & contributing to data collectives to combat information asymmetries 
%         \item Using available white label softwares to make their own applications (The Drivers Co-op, for example) 
%     \end{itemize}
%     \item While academic and popular literature has discussed how workers attempt to patch-up gig platforms using ad-hoc tools, our study adds to this body of literature by examining how workers attempt to break out of existing gig platforms through creating their own “indie” platforms with other stakeholders.
% \end{itemize}
 

 
% Gig platforms, the digital intermediaries of the gig economy, have become sites of contention in both academic and popular discourse due to their association with conditions of precarity, exploitation, and discrimination (\cite{watkinsTookPicGot2020}, \cite{iraniDifferenceDependenceDigital2015}, \cite{kumarUberBangladeshTangled2018}, \cite{dillahuntUncoveringValuesConstraints2017}, \cite{caloTAKINGECONOMYUBER2017}, \cite{DoorDashProofHow}). Gig platforms propagate precarity by positioning themselves as neutral market-making intermediaries, thereby evading employer responsibilities (\cite{griffithFAIRLABORSTANDARDS}, \cite{UberPostmatesSue}). They foster exploitation through practices of predatory inclusion and algorithmic control and surveillance (\cite{mcmillancottomWherePlatformCapitalism2020}, \cite{dziezaRevoltDeliveryWorkers2021a}). Finally, they engage in discriminatory practices through amplifying existing racial and gender biases in their rating practices (\cite{edelmanDigitalDiscriminationCase2014}, \cite{hannakBiasOnlineFreelance2017}). Gig platforms do not create conditions of precarity, exploitation, and discrimination; saying so would be technodeterministic. Rather, they build upon existing mechanisms in the labor market that fosters these conditions and amplify them through the use of technology. 

% Gig platforms claim that they simply act as marketplaces where independent contractors, seeking to provide a service can be matched with consumers for their services \cite{UberPostmatesSue}. As independent contractors in the United States, most gig workers are exempt from minimum wage protections and unemployment insurance, making them vulnerable to income uncertainty \cite{kallebergGoodJobsBad}. Additionally, independent contractors are exempt from the right to unionize which complicates gig workers' efforts to collectively organize and bargain with platforms for better working conditions \cite{griffithFAIRLABORSTANDARDS}. 

% In the on-demand service economy that gig platforms participate in, consumers expect faster, friction-less service at a low cost; gig workers bear the brunt of these expectations. Gig platforms utilize algorithmic management to breakdown, speed up, and scale the labor process in ways that are untenable for workers in order to meet consumer expectations \cite{kelloggAlgorithmsWorkNew2020}. One of the key ways that gig platforms utilize algorithmic management is by measuring workers against a constantly moving goalpost based on data that is continually harvested from workers \cite{doornPlatformCapitalismHidden2020}. For example, food delivery workers in dense metropolitan areas use bikes to navigate congested traffic when making deliveries. When e-bike models, like the Arrow, a motorized mountain bike that can attain speeds up to 28 mph, hit the marketplace some delivery drivers purchased them and began to make deliveries faster than they did previously \cite{dziezaRevoltDeliveryWorkers2021a}. The platforms instaneously updated their algorithms with this new data showing that deliveries can now be completed faster than before, pushing all its other drivers to meet this new standard and penalizing those who didn't \cite{dziezaRevoltDeliveryWorkers2021a}.  When workers try to push back against these practices, they face difficulty in collectively organizing due to the informationally isolated nature of their work and a lack of protections, under U.S labor law, to form a union \cite{kerrPostmatesDriversHave}. 

% Gig workers, by design, operate in environments that are both geographically and informationally isolated \cite{kerrPostmatesDriversHave} \cite{yaoTogetherAloneAtomization}. Unlike traditional workers who can call on formal and informal social and technical infrastructures, like an IT help desk or an HR rep, to manage breakdowns in their work, gig workers develop their own infrastructures for managing algorithmic breakdowns with scant support from the algorithmic managers or their coworkers.

% \subsection{Responses to Problems Endemic to Gig Platforms}

%infrastructuring work that workers do to address labor on incomplete platforms + recognition of this labor & the need to support it (Sutherland & Jarrahi + Irani)
%rise of collective action & mutual aid networks among gig workers (more on infrastructuring - Rida + Chinese workers paper + Los Deliveristos article) 
%movement towards worker/community control over means of production (e.g. co-operatives & white label software that enables communities to establish their own platforms) --> similar to mainstream vs. indie movement that occurred with FSF 
%end with question about how do stakeholders use bits of white-label software to construct indie platforms that are grounded in local communities? We explore this in our paper 


%According to Vosko, a job is considered precarious if it meets at least two of the following four conditions: low wages; high employment insecurity; low levels of employee control over wages, hours, and working conditions; and a lack of regulatory protection.

%While gig platforms amplify precarity, they do not create it from scratch Gig platforms amplify existing precarity through three key mechanisms: positioning themselves as neutral market-making intermediaries to evade employer responsibilities, implementing algorithmic control over the labor process, and devaluing work through rendering it invisible (\cite{griffithFAIRLABORSTANDARDS}, \cite{mcmillancottomWherePlatformCapitalism2020}). 

%For example, Uber's webpage markets its platform to potential drivers by saying "Looking for full-time or part-time driver jobs? Instead, give Uber a try. Get paid to drive or deliver when you want, on the platform with the largest network of active riders."; Notably no mention is made of the well documented lack of control Uber drivers experience as a result of the algorithmic management and information asymmetries endemic to gig platforms \cite{}.
% \subsection{Mainstream vs. Indie Platforms}
% %roots in Linux & open source movement (e.g. top-down vs. bottom-up) 
% %how this manifests in the context of gig platforms & food delivery in particular - e.g. as a push back against dominating top-down designed & run mainstream platforms
% %availability of white-label software (sort of a derivative of FSF) enabling bottom-up designed platforms & allowing stakeholders to build their own systems
% %How do stakeholders use bits of white-label software to construct bottom-up food service platforms?
% \subsection{Bricolage and Indie Platforms}
% %when does bricolage occur --> when stitching together disparate pieces of technology to address an unmet need (e.g. piecing together bits of white label technology to build an indie model of food delivery
% %bricolage enables the development of infrastructures that suit the builders' needs; these infrastructures are sociotechnical systems, they shape and are shaped by the interactions that occur within them 
% %bricolage comes from a tradition of building in low-resource environments, it demonstrates creativity in the face of limited resources however, the act of bricolage requires additional labor to stitch together disparate pieces of technology 
% \subsection{Limitations of Indie Platforms}
%lack of access to extensive capital & technical resources pushes indie platforms to engage in bricolage to stitch together disparate pieces of technology however, there are issues with compatibility across disparate pieces of software 
%point to literature on the benefits of fully integrated software environments (could use some pointers on where to find this) 
%Given that stakeholders in indie platforms experience financial and technical constraints, how can the HCI community develop tools to (1) support this platform model and (2) enable smoother integration of disparate pieces of technology?  

% \subsection{What is Infrastructure?}
% %top down
% %bottom up
% %breakages & invisible labor
% Infrastructures are the underlying foundations to large-scale systems \cite{edwards2003infrastructure}.   
% \subsection{Gig Platforms as Infrastructure}
% %gig platform and infrastructure literature (sawyer & jarrahi) --> information infrastructure & infrastructuring that actors engage in to supplement platform's IT capabilities 
% %focus on gig platforms & infrastructure 
% \subsection{Critical Infrastructuring and Food Delivery}
% %brief history of food delivery & overview of platform food delivery lit --> why is food delivery esp important now (during Covid)
% %models of food delivery (national vs local) --> implications for context in design 
% \cite{begole_working_2015}
% \cite{gregoryDeliveringEdinburghUncovering2020}
% %%need to weave in top-down vs. bottom up infrastructure & imbrication theory for discussion
% %%need to also weave in local expertise, human infrastructure, bricolage, for findings 

%%prior work on critical infrastructure has explored ABC but this discussion hasn't been applied to food delivery 
% no lit on socio-technical systems of food delivery
% a lot of work on gig work platforms and that includes paper that are on the critical infrastructure (Dillahunt) but none in food delivery 
%% map out gig work --> uber (task/service platforms) --> food delivery 



%start with literature grounding mainstream vs. indie in context of software dev literature 
%discuss platforms and sociomateriality/context
%indie platforms & postcolonia design 
%focus on platform co-operatives & socio-materiality/context literature 
%postcolonial platform design? 
%platform co-op principles (accountability to community) 
%context & localization in platform co-operatives --> why does it matter + tie to larger literature in CSCW/HCI with ubicomp & context + sociomateriality
%definitions of context & relationship to socio-materiality --> how context is actively constructed; why should sociomateriality matter for gig platform design 
%The broad principle that these examples illustrate is that users, not designers, determine the meaning of the technologies that they use, through the ways in which they incorporate them into practice. Accordingly, the focus of the design is not simply ‘‘how can people get their work done,’’ but ‘‘how can people create their own meanings and uses for the system in use’’; and in turn, this suggests an open approach in which users are active participants in the emergence of ways of working. - Dourish 2004
%Web localization, understood by scholars as a complex communicative, cognitive, textual and technological process by which interactive digital texts are modified to be used in different linguistic and sociocultural contexts, is guided by the expectations of the target audience and the specifications requested by initiators - Vasquez 2014

% For example, ridehailing platforms, like Uber, utilize facial recognition technology to verify its drivers. However, when drivers face difficulty in submitting biometric data to the platform, they can be deactivated at a moments notice without explanation, losing access to their ability to make a livelihood (\cite{watkinsTookPicGot2020}, \cite{UberPressureFacial}). Ridehailing platforms classify their workers as independent contractors, stating that their role as a platform is to be a marketplace that matches demand to rides with a supply of self-employed, independent drivres \cite{UberPostmatesSue}. As independent contractors, it is significantly more difficult to take legal action against ridehailing companies for possible wrongful termination due to the limited rights and affordances given to independent contractors under U.S law. Thus, gig platforms, such as ridehailing service, build upon existing systems of precarity in employment law through utilizing technology that is opaque and difficult for workers to contest. 

% In the on-demand service economy that gig platforms participate in, consumers expect faster, friction-less service at a low cost; gig workers bear the brunt of these expectations. Gig platforms utilize algorithmic management to breakdown, speed up, and scale the labor process in ways that are untenable for workers \cite{kelloggAlgorithmsWorkNew2020}. One of the key ways that gig platforms utilize algorithmic management is by measuring workers against a constantly moving goalpost. Platforms continually accelerate the rate of work by incentivizing faster times for task fulfillment, then incorporating those faster times into the standards against which workers are measured and penalizing those who fail to meet the now faster standard \cite{dziezaRevoltDeliveryWorkers2021a}. Platforms have little incentive to support what they view as a fungible labor source  \cite{scholzUberworkedUnderpaidHow2017}. Therefore, platforms continue to build upon and accelerate existing systems of precarity in legal, social, and economic infrastructures leaving workers to deal with the consequences. 

% Gig platforms build upon and amplify conditions of precarity, exploitation, and discrimination in the labor market through three key mechanisms: the evasion of worker protections by positioning themselves as neutral intermediaries, the use of opaque algorithmic management, and the devaluation of work (\cite{caloTAKINGECONOMYUBER2017}, \cite{dubalWinningBattleLosing2017}, \cite{fuchsDigitalLabourKarl2013}, \cite{scholzUberworkedUnderpaidHow2017}). However, gig platforms do not themselves create these conditions, rather they build upon existing weaknesses in social, legal, and economic infrastructures and amplify these through technology.

%Uber is successful, but there are cracks - e.g. in non-Western contexts you have local companies that dominate the market; on the surface it seems sustainable & it works for the platform when it works but it hurts the stakeholders 
%so alternative of indie platforms is promising but there are a lot of difficulties --> opportunities for HCI platforms
%argue for componetized models and for this paper to serve as a call to action
%make discussion more of a call to action; argue for bottom up infra & PC computing even though it is p crappy rn & it needs more support 
%input future work section  
%tension between human labor & personal touch & scale 
\subsection{The Instability of Bottom-up Infrastructures: Tenuous arrangements of actors and technologies in "Indie" platforms}
\subsection{When is Bottom-up Platform Infrastructure Appropriate?: Supporting situated action with "Indie" platforms}
Mainstream platforms, valuing economies of scale, are unable to address every edge-case by design; the help they are able to offer is generic by necessity. In food delivery, where variability and uncertainty are endemic (e.g. traffic delays an order, missing items, etc.), such generalized solutions do little to actually address the problems at hand.
\subsection{Drawing on Postcolonial Computing to Make Bottom-up Platform Infrastructures More Resilient}
%design as culturally specific
\subsubsection{Technical limitations of third-party software constrain Nosh's ability to scale up operations}
%focused more on technical components of food delivery
%difficulty with integration of tech for restaurants 
%difficulty on the back-end with having a cohesive platform 
%difficulty with reliability of tech for drivers; app always shutting down 
%difficulty with customization & attraction for customers 
%need human intervention to smooth over these difficulties 
%open case for HCI researchers to explore integration of building blocks + create open source solutions 
%To compensate for a lack of technical affordances in the third-party software, P2 has built out an extensive Google Data Studios dashboard and formula sheets. However, the solutions that P2 developed are, by their own acknowledgement birttle: "I just wouldn't [expand operations] with data dreamers at the moment because it's just too unstable, you  know." (P2)
%%DUMP
% In this section we expand upon our findings and discuss how stakeholders in local models of food delivery are constantly engaged with supplementing insufficient technology with human intervention that requires intensive, but often invisible, labor that is not sustainable at scale. We frame these discussion points around a central paradox: the resilience of local models is sustained by a tenuous arrangement of actors and technology. To illustrate this, we utilize the concept of critical infrastructuring, which highlights how stakeholders' essential efforts to maintaining the local food delivery ecosystem are often uncompensated and invisible to other actors. This enables us to construct a critique of the broader social system and arrangements in food delivery, where we discuss the open-question of whether  ....
% \subsection{Critical Infrastructuring and Local Models of Food Delivery}
% %%how humans make patchwork of technology seamless 
% %%the human actors & their material resources are interwoven in food delivery; when material resources exert constraints on food delivery model, human actors make work-arounds 
% %%D5: Part of the way that we have a notch have dealt with, that is, I, Again this is me I could before I joined nosh I collected and created apartment maps. Okay, to find units quickly. And I contribute to beans I don't know if you're familiar with beans.  it's an APP that it's like the last hundred feet, so it collects and shows apartment map so like if you're going to this apartment community, whereas unit one day. it'll show it so we share those amongst each other, I keep them all on my phone, so I places very fast, which I think helps me to have more regulars.
% \subsection{Invisible Labor Underpins Local Models of Food Delivery}
% %%Human intervention is often invisible labor that goes on behind the scenes, stakeholders rarely have visibility into the labor that each of them puts in to maintain food delivery 
% \subsection{Context and Gig Platform Design}
% %%maybe move to discussion?? could map to the community findings? 
% %%plurality --> food delivery is hyperlocal, communities want to support themselves & understand themselves a local model of food delivery that keeps THINGS (logistics, staffing, and participation) small actually works really well %% why go for a monistic model of food delivery when you could have a pluralistic one? 
% %%organizational ecology
% %%enables personal connection and engenders trust between stakeholders 
% %insert R6 quote: I say doordash and grub hub are fantastic technology companies that deliver food...nosh is a fantastic food delivery company that has some technology.

% \subsection{Decolonizing the future of work }
% Top-down platform design doesn't capture nuances and complexities 

==> table.tex <==
%you can input this table anywhere in the manuscript with the command "\input{table.tex}" Documentation for this code can be found here: https://ctan.math.illinois.edu/macros/latex/contrib/tabularray/tabularray.pdf

\SetTblrInner{colsep=3pt}
\begin{tblr}{hlines,vlines}
{Stakeholder\\Group} &
    Have Control &
    {Treated\\with Respect} &
    Financial &
    {Investment\\in Community} \\
Restaurant & 
    {Restaurants are\\investors in Nosh.\\They get a say\\in how delivery\\operations are run} & 
    {Treated as equal\\partners in\\dispute resolution} & 
    {Charged a lower\\commission rate with\\Nosh than with\\mainstream platforms} & 
    {Nosh provides an\\opportunity for\\locals to win\\When restaurants\\do well, Nosh\\does well due\\to investment\\structure} \\
{Platform\\Dispatcher} &
  {Ability to intervene\\in dispatching\\algorithm as they\\see fit} &
  {Treated as valuable\\team members by\\platform executives} &
  {Ability to make\\a living while\\working remotely.\\Especially important\\during COVID} &
  {Dispatchers are all\\locals, Nosh helps\\to keep jobs local} \\
Customer &
  {Ability to call\\platform dispatcher\\and get relevant\\information about\\order and\\delivery time} &
  {Able to talk to\\a person during\\dispute resolution,\\asked what would\\make things right\\for them} &
  {Able to meet\\desire to put\\money to local\\economy by\\using Nosh} &
  {Nosh helps\\community members\\support local\\businesses} \\
Driver &
  {Ability to set\\schedule and benefit\\from flexibly\\available shifts} &
  {Feel like expertise,\\feedback, and\\opinions are\\listened to by\\dispatchers and\\platform execs} &
  {Get financial security\\from floor pay.\\Tips tend to be\\higher with Nosh\\compared to\\mainstream platforms} &
  {Drivers are all\\locals, Nosh helps\\to keep jobs local}
\end{tblr}
